Progress in Computer-Assisted Inductive Theorem Proving by Human-Orientedness and Descente Infinie?

In this short position paper we briefly review the development history of automated inductive theorem proving and computer-assisted mathematical induction. We think that the current low expectations on progress in this field result from a faulty narrow-scope historical projection. Our main motivation is to explain--on an abstract but hopefully sufficiently descriptive level--why we believe that future progress in the field is to result from human-orientedness and descente infinie.

==> headerhot.tex <==
\def\subsubsubsection{\paragraph}
\catcode`\@=11
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\font\sixsf  = cmss10 scaled 600
\font\fvesf  = cmss10 scaled 500
%\font\sevsf  = cmss10 scaled 700
\font\egtsf  = cmss10 scaled 800
%\font\twfvit  = cmti10   \@magscale5 % text italic

\def\xiipt{\textfont\z@\twlrm 
  \scriptfont\z@\egtrm \scriptscriptfont\z@\sixrm
\textfont\@ne\twlmi \scriptfont\@ne\egtmi \scriptscriptfont\@ne\sixmi
\textfont\tw@\twlsy \scriptfont\tw@\egtsy \scriptscriptfont\tw@\sixsy
\textfont\thr@@\tenex \scriptfont\thr@@\tenex \scriptscriptfont\thr@@\tenex
\def\unboldmath{\everymath{}\everydisplay{}\@nomath\unboldmath
          \textfont\@ne\twlmi 
          \textfont\tw@\twlsy \textfont\lyfam\twlly
          \@boldfalse}\@boldfalse
\def\boldmath{\@ifundefined{twlmib}{\global\font\twlmib\@mbi\@magscale1\global
        \font\twlsyb\@mbsy \@magscale1\global\font
         \twllyb\@lasyb\@magscale1\relax\@addfontinfo\@xiipt
              {\def\boldmath{\everymath
                {\mit}\everydisplay{\mit}\@prtct\@nomathbold
                \textfont\@ne\twlmib \textfont\tw@\twlsyb 
                \textfont\lyfam\twllyb\@prtct\@boldtrue}}}{}\@xiipt\boldmath}%
\def\prm{\fam\z@\twlrm}%
\def\pit{\fam\itfam\twlit}\textfont\itfam\twlit \scriptfont\itfam\egtit
   \scriptscriptfont\itfam\sevit
\def\psl{\fam\slfam\twlsl}\textfont\slfam\twlsl 
     \scriptfont\slfam\tensl \scriptscriptfont\slfam\tensl
\def\pbf{\fam\bffam\twlbf}\textfont\bffam\twlbf 
   \scriptfont\bffam\ninbf \scriptscriptfont\bffam\ninbf 
\def\ptt{\fam\ttfam\twltt}\textfont\ttfam\twltt
   \scriptfont\ttfam\nintt \scriptscriptfont\ttfam\nintt 
\def\psf{\fam\sffam\twlsf}\textfont\sffam\twlsf
    \scriptfont\sffam\egtsf \scriptscriptfont\sffam\sixsf
\def\psc{\@getfont\psc\scfam\@xiipt{\@mcsc\@magscale1}}%
\def\ly{\fam\lyfam\twlly}\textfont\lyfam\twlly 
   \scriptfont\lyfam\egtly \scriptscriptfont\lyfam\sixly
 \@setstrut \rm}

\def\xxvpt{\textfont\z@\twfvrm 
  \scriptfont\z@\twtyrm \scriptscriptfont\z@\svtnrm
\textfont\@ne\twtymi \scriptfont\@ne\twtymi \scriptscriptfont\@ne\svtnmi
\textfont\tw@\twtysy \scriptfont\tw@\twtysy \scriptscriptfont\tw@\svtnsy
\textfont\thr@@\tenex \scriptfont\thr@@\tenex \scriptscriptfont\thr@@\tenex
\def\unboldmath{\everymath{}\everydisplay{}\@nomath\unboldmath
        \textfont\@ne\twtymi \textfont\tw@\twtysy \textfont\lyfam\twtyly
        \@boldfalse}\@boldfalse
\def\boldmath{\@subfont\boldmath\unboldmath}%
\def\prm{\fam\z@\twfvrm}%
\def\pit{\fam\z@\twfvit}%
\def\psl{\@subfont\sl\rm}%
\def\pbf{\@getfont\pbf\bffam\@xxvpt{cmbx10\@magscale5}}%
\def\ptt{\@subfont\tt\rm}%
\def\psf{\@subfont\sf\rm}%
\def\psc{\@subfont\sc\rm}%
\def\ly{\fam\lyfam\twtyly}\textfont\lyfam\twtyly 
   \scriptfont\lyfam\twtyly \scriptscriptfont\lyfam\svtnly 
\@setstrut \rm}

\catcode`\@=12


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SUPERCOMMANDS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% The following redefines the latex macro \math not because 
% \math makes trouble but rather because I dont like it
\long\def\math#1{\relax\ifmmode{#1}\else$#1 $\fi}
%                                          ^ 
% This blank is necessary because otherwise \math{} may expand to $$
% which is different from $ $ insofar as it starts a displaymath environment 
\long\def\nomath#1{\relax\ifmmode\mbox{#1}\else{#1}\fi}
\newcommand\nlbmath[1]{\nolinebreak\math{#1}}
\newcommand\maths[2]{\math{#1#2}}
\newcommand\nlbmaths[2]{\nolinebreak\math{#1#2}}
%The fol. defines \mathcommand to work like \newcommand with the exception of 
%switching to math-mode iff the command is not called in math-mode.
%\remathcommand is like \renewcommand.

\catcode`\@=11

\long\def\@reargdefmath#1[#2]#3{\@reargdef#1[#2]{\math{#3}}}

\long\def\@argdefmath#1[#2]#3{\@ifdefinable #1{\@reargdefmath#1[#2]{#3}}}

\def\mathcommand#1{\@ifnextchar [{\@argdefmath#1}{\@argdefmath#1[0]}}

\def\remathcommand#1{\edef\@tempa{\expandafter\@cdr\string
  #1\@nil}\@ifundefined{\@tempa}{\@latexerr{\string#1\space undefined}\@ehc
    }{}\@ifnextchar [{\@reargdefmath#1}{\@reargdefmath#1[0]}}

\catcode`\@=12

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\mathapplycommand      
#1#2{\mathcommand{#1}[1]{{#2}({##1})}}
\def\mathdoubleapplycommand
#1#2{\mathcommand{#1}[2]{{#2}({##1},{##2})}}
\def\mathtripleapplycommand
#1#2{\mathcommand{#1}[3]{{#2}({##1},{##2},{##3})}}
%example: \mathapplycommand\foo{\rm rubbish}
%         \foo{x} 
%produces:
%         rubbish(x)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\mathoverline=\overline
\remathcommand\overline[1]{\mathoverline{#1}}
% This makes \overline more intelligent, namely switching into math-mode
% if use in text-mode

\newcommand\mycomment[1]{{\iffalse{#1}\fi}}
% The argument of \comment is completely ignored

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Typesetting basics (lengths, struts) %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \setlength{\parindent}{2.0em}
\newlength{\disp}
\setlength{\disp}{\textwidth}
\addtolength{\disp}{-2.0\parindent}

\newlength{\textwidthminustwomm}
\setlength{\textwidthminustwomm}{\textwidth}
\addtolength{\textwidthminustwomm}{-0.2cm}

\newlength{\textwidthminushalfcm}
\setlength{\textwidthminushalfcm}{\textwidth}
\addtolength{\textwidthminushalfcm}{-0.5cm}

\newlength{\textwidthminusonecm}
\setlength{\textwidthminusonecm}{\textwidth}
\addtolength{\textwidthminusonecm}{-1.0cm}

\newlength{\textwidthminustwocm}
\setlength{\textwidthminustwocm}{\textwidth}
\addtolength{\textwidthminustwocm}{-2.0cm}

\newlength{\textwidthminusfourcm}
\setlength{\textwidthminusfourcm}{\textwidthminustwocm}
\addtolength{\textwidthminusfourcm}{-2.0cm}

\newlength{\textwidthminussixcm}
\setlength{\textwidthminussixcm}{\textwidth}
\addtolength{\textwidthminussixcm}{-6.0cm}

\newcommand\notop   {\vspace{-1.0\topsep}}
\newcommand\yestop  {\vspace{\topsep}}
\newcommand\halftop {\vspace{0.5\topsep}}
\newcommand\ohyestop{\vspace*{\topsep}}
\newcommand\noitem  {\vspace{-1.0\itemsep}}
\newcommand\yesitem {\vspace{\itemsep}}

\newcommand\schweinerei{
\topsep 4pt plus 1pt minus 2pt
\partopsep 2pt plus 1pt minus 1pt
\renewcommand{\baselinestretch}{0.96}
\hfuzz=4pt}



\newcommand\bigmath[1]{\ \math{#1}\ }
\newcommand\bigmaths[2]{\ \math{#1}#2\ }
\newcommand\bigmathnlb[2]{\ \mbox{\math{#1}#2}\ }
\newcommand\nlmath{$\hfill\mbox{}\\\mbox{}\hfill$}
\newcommand\nlnomath{\hfill\mbox{}\\\mbox{}\hfill}

%Dont include spaces for pretty print here
\newcommand\linemath[1]{\mbox{}\hfill$#1$\hfill\mbox{}\\}  
\newcommand\linemaths[2]{\mbox{}\hfill$#1$#2\hfill\mbox{}\\}  
\newcommand\linenomath[1]{\mbox{}\hfill{#1}\hfill\mbox{}\\}  
%Dont include spaces for pretty print here
\newcommand\LINEmath[1]{\mbox{}\hfill$#1$\hfill\mbox{}}
\newcommand\LINEmaths[2]{\mbox{}\hfill$#1$#2\hfill\mbox{}}
\newcommand\LINEnomath[1]{\mbox{}\hfill{#1}\hfill\mbox{}}
%Dont include spaces for pretty print here

\newcommand\mysection
[1]{\noindent{\Large\bf#1}\addcontentsline{toc}{section}{#1}}
\newcommand\mysubsection
[1]{\noindent{\Large\bf#1}\addcontentsline{toc}{subsection}{#1}}
\newcommand\mysubsubsection
[1]{\noindent{\bf#1}\addcontentsline{toc}{subsubsection}{#1}}

\newcommand\knuthquotation[2]
{{\footnotesize\begin{flushright}{\sl#1\par}{\noindent\sc--- #2}\end
{flushright}}}

% The fol. \par\noindent\initial{A} writes an initial letter A 
% Note that it was designed to have the bottom line exactly on
% the bottom line of the line it starts. So it works well with
%   \initial{\underline{\underline{\underline{\underline{First case:}}}}}
%   In the first case we have the following...
% The two texts "first case" share their bottom. The underline extends
% below it.
% If you do not want your intials to get the bottom line
% from the bottom line of the first but of the second line
% you must design another macro or use \initial{\raisebox{-3.5ex}{...}}

\newbox\yinibox
\def\initial#1{\par
\noindent
\setbox\yinibox\hbox{#1}%
\setbox\yinibox\vbox to \ht\yinibox{\offinterlineskip\hbox{{#1}~~}\vss}%
\leavevmode
\hangindent=\wd\yinibox
\hangafter=-2
\hbox to0pt{\hskip-\hangindent\box\yinibox\hfill}\ignorespaces}
   
%%% Parentheses: %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\mathcommand\inparentheses[1]{\left(\begin{array}[c]{l}#1\end{array}\right)}
\mathcommand\inparenthesestight
[1]{\left(\begin{array}{@{}l@{}}#1\end{array}\right)}
\mathcommand\inparenthesesinline[1]{(\ #1\ )}
\mathcommand\inpit[1]{(#1)}
\mathcommand\inparenthesesinlinetight[1]{\inpit{#1}}
\newcommand\mathinparenthesesinlinetight[1]{(#1)}%allows line breaking
\mathcommand\noparenthesesoplist[1]
{{\begin{array}{ll}\relax&#1\\\end{array}}}
\mathcommand\inparenthesesoplist[1]
{{\left(\noparenthesesoplist{#1}\right)}}
\newcommand\oplistund        {\\\tightund        &}
\newcommand\oplistoder       {\\\tightoder       &}
\newcommand\oplistcup        {\\\tightcup        &}
\newcommand\oplistuplus      {\\\tightuplus      &}
\newcommand\oplistequivalent {\\\tightequivalent &}
\newcommand\oplistimplies    {\\\tightimplies    &}
\newcommand\oplistcirc       {\\\tightcirc       &}
\newcommand\oplistantiimplies{\\\tightantiimplies&}
\newcommand\oplistnl         {\\                 &}

\newcommand\opta{{\rm[}}
\newcommand\opte{{\rm]}}
\newcommand\opt[1]{\opta#1\/\opte}
\mathcommand\displayopt
[1]{\left[\begin{array}[t]{@{\,}c@{\,}}#1\end{array}\right]}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MATH NOTATION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\stopq{\math{.}\penalty-1\relax\,\,} %\penalty-10 is too low
\mathcommand\hastype[2]{{#1}:{#2}}
\mathcommand\tighthastype[2]{{#1}\tight:{#2}}
\mathcommand\typed[3]{#1\hastype{#2}{#3}\stopq}
\mathcommand\comma{,\ \ }
\mathcommand\setwithstart{\{\ }
\newcommand\setwithmark{~\math|\penalty-9\relax\,\ } 
%\penalty-10 is too low, \penalty-1 is too high
\mathcommand\setwithmarkq[1] {\ |_{#1}\ }
\mathcommand\setwithstop     {\ \}}
\newcommand\setwith
[2]{\math{\setwithstart#1}\setwithmark\math{#2\setwithstop}}
%should not be mathcommand for enabling \penalty-1
\mathcommand\displaysetwith
[2]{{\left\{\begin{array}{@{\ \ }l@{\ \ }|@{\ \ }l@{\ \ }}#1&#2\\\end
{array}\right\}}}
\mathcommand\displayset
[1]{{\left\{\begin{array}{@{\ \ }l@{\ \ }}#1\\\end{array}\right\}}}

\newcommand\tight[1]{\math{#1}}
\newcommand\tightsubseteq   {\tight\subseteq  }
\newcommand\tightnotsubseteq{\tight\nsubseteq }
\newcommand\tightsuperseteq {\tight\superseteq}
\newcommand\tightsetminus   {\tight\setminus  }
\newcommand\tightplus       {\tight+          }
\newcommand\tighttimes      {\tight\times     }
\newcommand\tightcap        {\tight\cap       }
\newcommand\tightcup        {\tight\cup       }
\newcommand\tightuplus      {\tight\uplus     }
\newcommand\tightcirc       {\tight\circ      }
\newcommand\tightin         {\tight{\,\in\,}  }
\newcommand\tightnotin      {\tight{\,\not\in\,}  }
\newcommand\tightni         {\tight{\,\ni\,}  }
\newcommand\tightnotni      {\tight{\,\not\ni\,}  }
\newcommand\tightequal      {\tight{\,=\,}\penalty-1\relax}
\newcommand\tightnotequal   {\tight{\,\not=\,}}
\newcommand\tightpreceq     {\tight{\,\preceq\,}}
\newcommand\tightprec       {\tight{\,\prec\,}}
\newcommand\tightnotprec    {\tight{\,\nprec\,}}
\newcommand\tightsucceq     {\tight{\,\succeq\,}}
\newcommand\tightsucc       {\tight{\,\succ\,}}
\newcommand\tightgtr        {\tight{\,>\,}}
\newcommand\tightless       {\tight{\,<\,}}
\newcommand\tightleq        {\tight{\,\leq\,}}
\newcommand\tightgeq        {\tight{\,\geq\,}}

\newcommand\boldequal  {\tight=}
\newcommand\boldunequal{\tight{\not=}}
\newcommand\boldless   {\tight<}
\newcommand\boldnotless{\tight{\not<}}
\newcommand\boldimplies{\tight\Rightarrow}
\newcommand\Defnombox{{\rm Def}}
\newcommand\Def{\mbox{\Defnombox}}
\mathcommand\DEF{\Defnombox\:}

\mathcommand\tightimplies    {\Rightarrow}
\mathcommand\tightantiimplies{\Leftarrow}
\mathcommand\tightequivalent {\Leftrightarrow}
\mathcommand\tightund        {\wedge}
\mathcommand\tightoder       {\vee}
\mathcommand\tightshefferstroke{|}
\newcommand\implies      {\ \tightimplies      \penalty-2\relax\ }
\newcommand\und          {\ \tightund          \penalty-2\relax\ }
\newcommand\oder         {\ \tightoder         \penalty-2\relax\ }
\newcommand\antiimplies  {\ \tightantiimplies  \penalty-2\relax\ }
\newcommand\equivalent   {\ \tightequivalent   \penalty-2\relax\ }
\newcommand\shefferstroke{\ \tightshefferstroke\penalty-2\relax\ }

\newcommand \id          {{\rm id}}
\mathcommand\allall      {\mathcal{V}}
\mathcommand\allsets     {\POWER\allall}
\mathcommand\allfinitesets{\FINITE\allall}
\mathcommand\urelements  {\mathcal{U}}
\mathcommand\algebra     {\mathcal{A}}
\mathcommand\balgebra    {\mathcal{B}}
\mathcommand\calgebra    {\mathcal{C}}
\mathcommand\dalgebra    {\mathcal{D}}
\mathcommand\ialgebra    {\mathcal{I}}
\mathcommand\salgebra    {\mathcal{S}}
\mathcommand\walgebra    {\mathcal{W}}
\mathcommand\ralgebra    {\mathcal{R}}
\mathcommand\algebraprime{\mathcal{A}'}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mathapplycommand\FLD        {\rm field}
\mathapplycommand\DOM        {\rm dom}
\mathapplycommand\RAN        {\rm ran}
\mathapplycommand\kernel     {\rm ker}
% \mathapplycommand\FINITE     {\mbox{\fraknomath P}_\N}%for \frak from german
% \mathapplycommand\POWER      {\mbox{\fraknomath P}}
% \mathapplycommand\posfinPOWER{\mbox{\fraknomath P}_\posN\!}
\mathapplycommand\FINITE     {{\mathfrak P}_{\scriptscriptstyle\N}}%for \frak from amssymb
\mathcommand\POWERSYM        {{\mathfrak P}}
\mathapplycommand\POWER      {\POWERSYM}
\mathapplycommand\posfinPOWER{\POWERSYM_{\scriptscriptstyle\posN\!}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mathcommand\CARD[1]         {\,|{#1}|\,}
\mathcommand\FLOOR[1]        {\ \lfloor#1\rfloor\ }
\mathcommand\CEIL[1]         {\ \lceil#1\rceil\ }
\mathcommand\reverserelation[1]{{#1}^{-1}}
%\mathcommand\restrictedto[1]{|_{#1}}
\mathcommand\domres[2]{{_{#2}\tight\upharpoonleft#1}}
\mathcommand\ranres[2]{{#1\tight\upharpoonright_{#2}}}
\mathcommand\funarg[1]{(#1)}
\mathcommand\app[2]{#1(#2)}
\mathcommand\displayapp[2]{#1\inparentheses{#2}}
\mathcommand\apptotuple[2]{#1#2}
\mathcommand\relapp[2]{\langle#2\rangle#1}
\mathcommand\displayrelapp
[2]{\left\langle\begin{array}{@{}l@{}}#2\end{array}\right\rangle\!#1}
\mathcommand\relappsin[2]{\relapp{#1}{\!\{#2\}\!}}
\mathcommand\revrelapp[2]{#1\langle#2\rangle}
\mathcommand\displayrevrelapp
[2]{#1\!\left\langle\begin{array}{@{}l@{}}#2\end{array}\right\rangle}
\mathcommand\revrelappsin[2]{\revrelapp{#1}{\!\{#2\}\!}}
\mathcommand\pair[2]{(#1,#2)}
\mathcommand\displaypair[2]{\inparentheses{#1,\ \ #2}}
\mathcommand\trip[3]{(#1,#2,#3)}
\mathcommand\displaytrip[3]{\inparentheses{#1,\ \ #2,\ \ #3}}
\mathcommand\superdisplaytrip[3]{\left(\begin
{array}{l}#1,\\#2,\\#3,\\\end{array}\right)}
\mathcommand\quar[4]{(#1,#2,#3,#4)}
\mathcommand\displayquar[4]{\inparentheses{#1,\ \ #2,\ \ #3,\ \ #4}}
\mathcommand\superdisplayquar[4]{\left(\begin
{array}{l}#1,\\#2,\\#3,\\#4\\\end{array}\right)}
\mathcommand\quin[5]{(#1,#2,#3,#4,#5)}
\mathcommand\displayquin[5]{\inparentheses{#1,\ \ #2,\ \ #3,\ \ #4,\ \ #5}}
\mathcommand\sext[6]{(#1,#2,#3,#4,#5,#6)}
\mathcommand\sept[7]{(#1,#2,#3,#4,#5,#6,#7)}
\mathcommand\oct[8]{(#1,#2,#3,#4,#5,#6,#7,#8)}
\mathcommand\ninetuple[9]{(#1,#2,#3,#4,#5,#6,#7,#8,#9)}
\newcommand\tentuple[9]{(#1,#2,#3,#4,#5,#6,#7,#8,#9,\singletonrest}
\newcommand\singletonrest[1]{#1)}
\newcommand\elev[9]{(#1,#2,#3,#4,#5,#6,#7,#8,#9,\pairrest}
\newcommand\pairrest[2]{#1,#2)}
\mathcommand\setwithq[3]     {\setwithstart#2\setwithmarkq{#1}#3\setwithstop}
\mathcommand\setofwords[1]{#1^{\textstyle\ast}}
\mathcommand\setofwordsscriptstyle[1]{#1^{\ast}}
\mathcommand\setofnonemptywords[1]{#1^+}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mathcommand\FUNSET   [2]{{#1}\rightarrow{#2}}
\mathcommand\PARFUNSET[2]{{#1}\leadsto   {#2}}
\mathcommand\FUNDEF   [3]{\hastype{#1}{\FUNSET   {#2}{#3}}}
\mathcommand\PARFUNDEF[3]{\hastype{#1}{\PARFUNSET{#2}{#3}}}
%categories
\mathcommand\morphcolon{::}
\mathcommand\morpharrow{\rightarrow}
\mathcommand\morph  [3]{{#1}\morphcolon{#2}\morpharrow{#3}}
\newcommand\Idname{{\rm Id}}
\mathcommand\Id[1]{{\Idname_{#1}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mathcommand\equiclass[2]{{#1}{[\{{#2}\}]}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mathcommand\aritysugarsymbol{\rightarrow}
\mathcommand\aritysugar{\ \aritysugarsymbol\ }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mathcommand\monus{\mathchoice
{\raisebox{-.4ex}{$\dot{\raisebox{.4ex}[0ex]{$-$}}$}}%     display-style
{\raisebox{-.4ex}{$\dot{\raisebox{.4ex}[0ex]{$-$}}$}}%     text-style
{\raisebox{-.3ex}{$\scriptstyle\dot{\raisebox{.3ex}[0ex]
{$\scriptstyle-$}}$}}                                %     scriptstyle
{\raisebox{-.2ex}{$\scriptscriptstyle\dot{\raisebox{.2ex}[0ex]
{$\scriptscriptstyle-$}}$}}                          %scriptscriptstyle
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\mathcommand\yields{\;\vdash\;}
\mathcommand\antiyields{\;\dashv\;}
\mathcommand\tightyields{\vdash}
\mathcommand\tightantiyields{\dashv}
\mathcommand\notyields{\;\nvdash\;}
\mathcommand\refltransyields{\hspace{0.5em}\raisebox{1.3ex}{\math{\scriptstyle
  \ast}}\hspace{-1.0em}\yields}
\mathcommand\transyields
{\hspace{0.5em}\raisebox{1.3ex}{$\scriptscriptstyle%\oplus
+$}\hspace
{-1.0em}\yields\hspace{0.3em}}
\mathcommand\notmodels{\:\not\!\models}

\newcommand\EVALSYM{{\rm eval}}
\mathapplycommand\EVAL{\EVALSYM}
\mathcommand\V{{\rm V}}
\mathcommand\X{{\rm X}}
\newcommand\nottight{\bigmath}
\mathcommand\refltransclosureinline[1]{{#1}^\ast}
\mathcommand\VARSYM {\mathcal{V}}
\mathapplycommand\VAR{\VARSYM}
\mathcommand\VARnoparentheses[1]{\VARSYM #1}
\mathcommand\VARsingleindex[1]{\VARSYM\!_{{#1}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ZAHLENMENGEN %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \N        Set of natural numbers
% \posN     Set of positive natural numbers
% \ordclass Proper class of ordinal numbers
% \ZZ       Set of integers
% \Q        Set of rationals
% \RE       Set of real numbers
% \posRE    Set of positive real numbers
% \nonnegRE Set of non-negative real numbers
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \mathcommand\N{{\rm
% %\rm must be out here because on rare occursions does not work
% %infront of the I\hskip....
% %\ifmmode%  Sind wir im Mathemodus ?
% \mathchoice{{I\hskip -2pt   N}}% display-style
%            {{I\hskip -2pt   N}}% text-style
%            {{I\hskip -1.5pt N}}% scriptstyle
%            {{I\hskip -1pt   N}}% scriptscriptstyle
% %\else\math{\rm I\hskip-2pt N}\fi
% }}
% \newcommand\ZZ{{\rm\ifmmode\mathchoice{{Z\hskip -4pt Z}}{{Z\hskip -4pt Z}}
% {{Z\hskip -3pt Z}}{{Z\hskip -3pt Z}}\else\mbox{\tenrm Z\hskip-4pt Z}\fi}}
\mathcommand\N{{\bf N}}
\mathcommand\posN{\N_{\:\!\!\mbox{\sixsf+}}}
\mathcommand\ZZ{{\bf Z}}
\mathcommand\Q{{\bf Q}}
\mathcommand\ordclass{\mathcal{O}}
%\newcommand\RE{{\rm\ifmmode\mathchoice{{I\hskip -2pt R}}{{I\hskip -2pt R}}
%{{I\hskip -1.5pt R}}{{I\hskip -1pt R}}\else{\tenrm I\hskip-2pt R}\fi}}
\mathcommand\RE{{\bf R}}
\mathcommand\posRE{\RE_{\scriptscriptstyle +}}
\mathcommand\nonnegRE{\RE_{\scriptscriptstyle\succeq0}}

\mathcommand\Qzero{{\cal Q}_0}
\newcommand\squaredot{\,\rule{0.4ex}{0.4ex}\,}

%Transitive closures
\mathcommand\transclosure[1]{\stackrel{\scriptscriptstyle+}{#1}}
\mathcommand\transclosureinline[1]{{#1}^{\scriptscriptstyle+}}

%_____________________________________________________________________________
%Signatures
\mathcommand\sigarity{\alpha}
\newcommand\sig{{\rm sig}}
\mathcommand\sigsorts  {{\mathbb S}}
\mathcommand\sigfunsym {{\mathbb F}}
\mathcommand\consfunsym{{\mathbb C}\,} 
% \, cures strange dvips bugg
\mathcommand\deffunsym {{\mathbb N}}
\mathcommand\Ax{\mathcal{AX}}

%from header.tex
%_____________________________________________________________________________
%Reduction relation

%\red...
%\notred
%\redpara
%\revpara
%\simpara
%\unired
\mathcommand\unired{\Longrightarrow}
\mathcommand\redsimple{\longrightarrow}
\mathcommand\redindex[1]{\redsimple_{_{\!#1}}}
\mathcommand\notredindex[1]{\,\,\,\not\!\!\!\!\redsimple_{_{\!#1}}}
\newcommand\redsub             {\redindex{\R ,\X        }}
\newcommand\redsubprime        {\redindex{\R',\X'       }}
\newcommand\redshortsub        {\redindex{\R ,\V        }}
\newcommand\redshortsubprime   {\redindex{\R',\V'       }}
\newcommand\redsubY            {\redindex{\R ,\Y        }}
\newcommand\redsubemptyset     {\redindex{\R ,\emptyset }}
\newcommand\redsubprimeemptyset{\redindex{\R',\emptyset }}
\newcommand\redsubVsig         {\smallfootroom\redindex{\R ,\Vsig     }}
\newcommand\redsubVsigprime    {\smallfootroom\redindex{\R',\Vsigprime}}
\mathcommand\redindexn[2]{\stackrel{#1}\redsimple_{_{\!#2}}}
\mathcommand\redparaindex[1]{\redpara_{\hskip-1.5pt\scriptscriptstyle#1}}
\mathcommand\revparaindex[1]{\revpara_{\hskip-1.5pt\scriptscriptstyle#1}}
\mathcommand\simparaindex[1]{\simpara_{\hskip-1.5pt\scriptscriptstyle#1}}
\mathcommand\uniredindex[1]{\unired_{\hskip-1.5pt\scriptscriptstyle#1}}

%\antired...
%\notantired..
%\antiredpara...
%\antirevpara...
%\antiunired...
\mathcommand\antiunired{\Longleftarrow}
\mathcommand\antired{\longleftarrow}
\mathcommand\antiuniredindex[1]{\antiunired_{_{\!#1}}}
\mathcommand\antiredindex[1]{\antired_{_{\!#1}}}
\mathcommand\notantiredindex[1]{\,\,\,\not\!\!\!\!\antired_{_{\!#1}}}
\newcommand\antiredsub          {\antiredindex{\R ,\X }}
\newcommand\antiredshortsub     {\antiredindex{\R ,\V }}
\newcommand\antiredshortsubprime{\antiredindex{\R',\V'}}
\newcommand\antiredsubVsig      {\smallfootroom\antiredindex{\R',\Vsig}}
\mathcommand\antiredindexn[2]{\stackrel{#1}\antired_{_{\!#2}}}
\mathcommand\antiredparaindex
[1]{\antiredpara_{\hskip-1.25pt\scriptscriptstyle#1}}
\mathcommand\antirevparaindex[1]
{\antirevpara_{\hskip-1.25pt\scriptscriptstyle#1}}

%\sym...
\mathcommand\sym{\longleftrightarrow}
\mathcommand\symindex[1]{\sym_{_{\!#1}}}
\mathcommand\symindexn[2]{\stackrel{#1}{\sym_{_{\!#2}}}}
\newcommand\symsub     {\symindex{\R,\X}}
\newcommand\symshortsub{\symindex{\R,\V}}
\newcommand\symsubVsig {\smallfootroom\symindex{\R,\Vsig}}

%Reflexive transitive closures
%Congruences
%\congru...
%\footnotecongru...
%\notcongru...
\mathcommand\refltransclosure[1]{\stackrel{\scriptstyle\ast}{#1}}
%{\mathop{#1}^{\scriptstyle\ast}}
\mathcommand\congru{\refltransclosure\sym}
\mathcommand\congruindex[1]{\congru_{_{\!#1}}}
\newcommand\congrusub             {\congruindex{\R ,\X            }}
\newcommand\congrushortsub        {\congruindex{\R ,\V            }}
\newcommand\congrusubVsig         {\smallfootroom\congruindex{\R ,\Vsig     }}
\newcommand\congrusubVsigprime    {\smallfootroom\congruindex{\R',\Vsigprime}}
\newcommand\congrusubemptyset     {\congruindex{\R ,\emptyset     }}
\newcommand\congrusubprimeemptyset{\congruindex{\R',\emptyset     }}
\mathcommand\footnotecongru%{\stackrel\footnoteoast\sym}
{\congru}
\mathcommand\footnotecongruindex[1]{\footnotecongru_{_{#1}}}
\mathcommand\notcongru{\hspace{0.6em}\not\hspace{-0.85em}\refltransclosure\sym}
\mathcommand\notcongruindex[1]{\notcongru_{_{\!#1}}}
\newcommand\notcongrusub        {\notcongruindex{\R,\X       }}
\newcommand\notcongrusubemptyset{\notcongruindex{\R,\emptyset}}

%Transitive closures
%\trans...
%\antitrans...
\mathcommand\trans{\transclosure\redsimple}
\mathcommand\transindex[1]{\trans_{_{\!#1}}}
\newcommand \transsub        {\transindex{\R,\X}}
\newcommand \transshortsub   {\transindex{\R,\V}}
\newcommand \transsubVsig    {\smallfootroom\transindex{\R,\Vsig}}
\newcommand \transsubemptyset{\transindex{\R,\emptyset}}
\mathcommand\antitrans{\transclosure\antired}
\mathcommand\antitransindex[1]{\antitrans_{_{\!#1}}}
\newcommand \antitranssub     {\antitransindex{\R,\X}}
\newcommand \antitransshortsub{\antitransindex{\R,\V}}
\newcommand \antitranssubVsig {\smallfootroom\antitransindex{\R,\Vsig}}

%Reflexive and transitive closures
%\refltrans...
%\footnoterefltrans...
%\notrefltrans...
%\antirefltrans...
%\footnoteantirefltrans...
\mathcommand\refltrans{\refltransclosure\redsimple}
\mathcommand\refltransindex[1]{\refltrans_{_{\!#1}}}
\newcommand \refltranssub          {\refltransindex{\R ,\X }}
\newcommand \refltranssubemptyset  {\refltransindex{\R ,\emptyset}}
\newcommand \refltranssubprime     {\refltransindex{\R',\X'}}
\newcommand \refltransshortsub     {\refltransindex{\R ,\V }}
\newcommand \refltransshortsubprime{\refltransindex{\R',\V'}}
\newcommand \refltranssubVsig      {\smallfootroom\refltransindex{\R ,\Vsig}}
\mathcommand\footnoterefltrans%{\stackrel\footnoteoast\redsimple}
{\refltrans}
\mathcommand\footnoterefltransindex[1]{\footnoterefltrans_{_{#1}}}
\newcommand \footnoterefltranssub     {\footnoterefltransindex{\R,\X}}
\newcommand \footnoterefltransshortsub{\footnoterefltransindex{\R,\V}}
\mathcommand\notrefltrans
            {\hspace{0.6em}\not\hspace{-0.85em}\refltransclosure\redsimple}
\mathcommand\antirefltrans{\refltransclosure\antired}
\mathcommand\antirefltransindex[1]{\antirefltrans_{_{\!#1}}}
\newcommand \antirefltranssub          {\antirefltransindex{\R ,\X }}
\newcommand \antirefltransshortsub     {\antirefltransindex{\R ,\V }} 
\newcommand \antirefltransshortsubprime{\antirefltransindex{\R',\V'}} 
\newcommand \antirefltranssubVsig      {\antirefltransindex{\R',\V'}} 
\mathcommand\footnoteantirefltrans%{\stackrel\footnoteoast\antired}
{\antirefltrans}
\mathcommand\footnoteantirefltransindex[1]{\footnoteantirefltrans_{_{#1}}}
\newcommand \footnoteantirefltranssub     {\footnoteantirefltransindex{\R,\X}}
\newcommand \footnoteantirefltransshortsub{\footnoteantirefltransindex{\R,\V}}

%joinability
\mathcommand\downarrowindex[1]{\downarrow_{_{#1}}}
\newcommand \downarrowsub        {\downarrowindex{\R ,\X       }}
\newcommand \downarrowsubemptyset{\downarrowindex{\R ,\emptyset}}
\newcommand \downarrowsubVsig    {\smallfootroom\downarrowindex{\R,\Vsig}}
\newcommand \downarrowsubprimeemptyset{\downarrowindex{\R',\emptyset}}
\mathcommand\notconfluindex[1]{\notconflu_{_{#1}}}
\newcommand \notconflusub        {\notconfluindex{\R,\X       }}
\newcommand \notconflusubemptyset{\notconfluindex{\R,\emptyset}}
\mathcommand\footnotenotconfluindex[1]{\footnotenotconflu_{_{#1}}}
\newcommand \footnotenotconflusub{\footnotenotconfluindex{\R,\X}}

%strong joinability
\mathcommand\downdownarrow        {\downdownarrows}
\mathcommand\downdownarrowindex[1]{\downdownarrow_{_{#1}}}
\newcommand \downdownarrowsub     {\downdownarrowindex{\R ,\X       }}

\mathcommand\reflclosure[1]{\stackrel
%{\raisebox{0.1em}{$\scriptscriptstyle\preceq$}{ 1}}
{\scriptscriptstyle=}
{#1}}
\mathcommand\reflclosureinline[1]{{#1}^{\scriptscriptstyle=}}
\mathcommand\onlyonce
%{{\displaystyle\mathop{\redsimple}^{{\leq}1}}}
{\reflclosure\redsimple}
\mathcommand\antionlyonce{\reflclosure\antired}
\mathcommand\onlyonceindex[1]{\onlyonce_{_{\!#1}}}
\mathcommand\antionlyonceindex[1]{\antionlyonce_{_{\!#1}}}

\mathapplycommand\nf{\rm NF}

\mathcommand\toconditiontermssub     {\twoheadrightarrow_{_{\R,\X}}}
\mathcommand\toconditiontermssubY    {\twoheadrightarrow_{_{\R,\Y}}}
\mathcommand\toconditiontermsshortsub{\twoheadrightarrow_{_{\R,\V}}}

%_____________________________________________________________________________
%Variables notation
\newcommand \U{{\rm U}}
\newcommand \Y{{\rm Y}}
\newcommand \Z{{\rm Z}}
\mathcommand\Xprime{{\rm X}'}
\mathcommand\Yprime{{\rm Y}'}
\mathcommand\Xprimeprime{{\rm X}''}
\newcommand \SIG     {{\rm SIG}}
\mathcommand\CONS    {\mathcal{C}}
\mathcommand\SIGsort     [1]{(\SIG     ,#1)}
\mathcommand\CONSsort    [1]{(\CONS    ,#1)}
\mathcommand\varsigmasort[1]{(\varsigma,#1)}
\mathcommand\SIGsortindex     [1]{_{\SIG ,#1}}
\mathcommand\CONSsortindex    [1]{_{\CONS,#1}}
\mathcommand\DUNNOsortindex   [1]{_{\DUNNO,#1}}
\mathcommand\varsigmasortindex[1]{_{\varsigma,#1}}
\mathcommand\Vsig      {\V \!_{\SIG }}
\mathcommand\Xsig      {\X   _{\SIG }}
\mathcommand\Vcons     {\V \!_{\CONS}}
\mathcommand\Sigmacons {\Sigmaoffont_{\CONS}}
\mathcommand\Xcons     {\X   _{\CONS}}
\mathcommand\Vconsprime{\V'\!_{\CONS}}
\mathcommand\Vsigprime {\V'\!_{\SIG }}
\mathcommand\sigV      {\Vsig\!\uplus\!\Vcons}
\mathcommand\sigVprime {\Vsigprime\!\uplus\!\Vconsprime}
\mathcommand\hiddenVindi     [2]{\V   \!_{{#1},{#2}}}
\mathcommand\hiddenXindi     [2]{\X     _{{#1},{#2}}}
\mathcommand\hiddenVprimeindi[2]{\V'\!\!_{{#1},{#2}}}
\newcommand \Vsigindex     [1]{\hiddenVindi\SIG     {#1}}
\newcommand \Xsigindex     [1]{\hiddenXindi\SIG     {#1}}
\newcommand \Vconsindex    [1]{\hiddenVindi\CONS    {#1}}
\newcommand \Xconsindex    [1]{\hiddenXindi\CONS    {#1}}
\newcommand \Vvarsigmaindex[1]{\hiddenVindi\varsigma{#1}}
\newcommand \Xvarsigmaindex[1]{\hiddenXindi\varsigma{#1}}
\mathapplycommand\VARCONS{\VARsingleindex\CONS}
\mathapplycommand\VARSIG {\VARsingleindex\SIG}
\mathapplycommand\VARord {\VARsingleindex\boldless}

%_____________________________________________________________________________
%Term notation
\mathcommand\vt{\mathcal{ T}}
\mathcommand\gt{\mathcal{GT}}
\mathcommand\hiddenvtindi[2]{\mathcal{ T}\!_{#1,#2}}
\mathcommand\hiddengtindi[2]{\mathcal{GT}\!_{#1,#2}}
\newcommand\vtsigindex     [1]{\hiddenvtindi{\SIG     }{#1}}
\newcommand\vtconsindex    [1]{\hiddenvtindi{\CONS    }{#1}}
\newcommand\vtvarsigmaindex[1]{\hiddenvtindi{\varsigma}{#1}}
\newcommand\gtsigindex     [1]{\hiddengtindi{\SIG     }{#1}}
\newcommand\gtconsindex    [1]{\hiddengtindi{\CONS    }{#1}}
\newcommand\gtvarsigmaindex[1]{\hiddengtindi{\varsigma}{#1}}
\mathapplycommand\hiddentv     {\mathcal{T}}
\mathapplycommand\hiddentg     {\mathcal{GT}}
\mathapplycommand\hiddentvprime{\mathcal{T}'}
%ground term sets
\newcommand\tgcons              {\hiddentg\cons }
\newcommand\tgsig               {\hiddentg\sig  }   
\newcommand\tgdunno             {\hiddentg\dunno}
\newcommand\tgconsprime         {\hiddentg{\cons'}}
\newcommand\tgsigprime          {\hiddentg{\sig' }}
\newcommand\tgunderlinecons     {\hiddentg{\underline{\underline{\cons }}}}
\newcommand\tgunderlineconsprime{\hiddentg{\underline{\underline{\cons'}}}}
%non-ground term sets
% variables from \Vsig or \Vsigprime
\newcommand\tsigV        {\hiddentv{\sig  ,\V}}
\newcommand\tsigVsig     {\hiddentv{\sig  ,\Vsig}}
\newcommand\tsigVsigprime{\hiddentv{\sig' ,\Vsigprime}}
% variables from \Vcons 
\newcommand\tcc{\hiddentv{\cons,\Vcons}}
% variables from \Vcons\cup\Vsig etc.
\newcommand\tss          {\hiddentv{\sig  ,\sigV     }}
\newcommand\tcs          {\hiddentv{\cons ,\sigV     }}
\newcommand\tcsprime     {\hiddentv{\cons',\sigVprime}}
% variables from \X or \X' etc.
\newcommand\tsigX        {\hiddentv{\sig ,\X }}
\newcommand\tconsX       {\hiddentv{\cons,\X }}
\newcommand\tsigXprime   {\hiddentv{\sig',\X'}}
\newcommand\tconsXprime  {\hiddentv{\cons',\X'}}
\newcommand\tconsVconsX  {\hiddentv{\cons,\Xcons}}
% variables from \Y
\newcommand\tsigY        {\hiddentv{\sig ,\Y }}
\newcommand\tconsY       {\hiddentv{\cons,\Y }}
%term algebras
\newcommand\tconsXalt {\app{{\mathcal T}_\CONS}\X}
\newcommand\tconsValt {\app{{\mathcal T}_\CONS}\V}
\newcommand\tX        {\hiddentv\X}
\newcommand\tXprime   {\hiddentv{\X'}}
\newcommand\tV        {\hiddentv\V}
\newcommand\tY        {\hiddentv\Y}
\newcommand\temptyset {\hiddentv\emptyset}
\newcommand\tVsig     {\hiddentv\Vsig}
\newcommand\tVsigprime{\hiddentvprime\Vsigprime}
% \newcommand{\gtc}{\hiddentg{\cons}}
%_____________________________________________________________________________
%substitutions
\mathcommand\SUBSYM{\mathcal{SU\hspace{-.08em}B}}
\mathdoubleapplycommand\SUBST{\SUBSYM}
\newcommand \Xsubst     {\SUBST\V\tX   }
\newcommand \Vsubst     {\SUBST\V\vt   }
\newcommand \Vsigsubst  {\SUBST\V\tVsig}
\newcommand \Gsubst     {\SUBST\V\gt   }
\mathcommand\Isubst     {{\rm CGSUB}(\V ,\cons )}
\mathcommand\Isubstprime{{\rm CGSUB}(\V',\cons')}
\mathcommand\GENSYM     {\mathcal{G\hspace{-.04em}E\hspace{-.09em}N}}
\mathcommand\GSSYM      {{\GENSYM\hspace{-.14em}}\SUBSYM}
\mathdoubleapplycommand\GS{\GSSYM}
\newcommand\VGS{\GS\V\vt}
\newcommand\XGS{\GS\V\tX}
\newcommand\VsigGS{\GS\V\tVsig}
%
\mathcommand\POSSYMBOL{\mathcal{P\hspace{-.08em}O\hspace{-.1em}S}}
\mathcommand\VPOSSYMBOL{\V\hspace{-.04em}\POSSYMBOL}
\mathcommand\FPOSSYMBOL{\sigfunsym\hspace{-.04em}\POSSYMBOL}
\mathapplycommand\TPOS{\POSSYMBOL}
%\mathapplycommand\POS{\POSSYMBOL} \POS is also used by xy. Use \TPOS instead!
\mathapplycommand\VPOS{\VPOSSYMBOL}
\mathapplycommand\FPOS{\FPOSSYMBOL}
%\mathcommand\OCCSYMBOL{\mathcal{O}}
%\mathapplycommand\OCC{\OCCSYMBOL}%obsolete but still in use
\mathcommand\neitherprefixsymbol{\parallel}
\mathcommand\neitherprefix[2]{{#1}\,\neitherprefixsymbol\,{#2}}
\mathcommand\replsuffix   [2]{[\,#1\leftarrow#2\,]}      %use \repl if possible
\mathcommand\replparsuffix[3]{\replsuffix{#1}{#2\ |\ #3}}%use \replpar
\mathcommand\repl         [3]{#1\penalty-1\replsuffix{#2}{#3}}
\mathcommand\replpar      [4]{#1\penalty-1\replparsuffix{#2}{#3}{#4}}
\mathcommand\eqvariablessig[1]{\mbox{\rm Eq}(\sig,{#1})}
\newcommand\eqvsig{\eqvariablessig{\sigV}}
\mathcommand\eqgsig{\mbox{\rm GEq}(\sig)}
\mathcommand\direqv[1]{\mbox{\rm DEq}(#1)}
\newcommand\direqvariablessig[1]{\direqv{\sig,{#1}}}
\newcommand\direqvsig{\direqv{\sig,\sigV}}
\mathapplycommand\MGU{\rm Mgu}
\mathdoubleapplycommand\minmgu{\rm mgu}
\mathdoubleapplycommand\sep{\rm Sep}
\mathdoubleapplycommand\minsep{\rm sep}
\mathapplycommand\depth{\rm depth}
\mathapplycommand\size{\rm size}
\newcommand\monotonic           {\tsigX-mono\-tonic}
\newcommand\Vmonotonic          {\vt-mono\-tonic}
%\newcommand\amonotonic          {an \X-mono\-tonic}
\newcommand\emptysetmonotonic   {\gt-mono\-tonic}
\newcommand\monotonicity        {\tsigX-mono\-toni\-city}
\newcommand\Vmonotonicity       {\vt-mono\-toni\-city}
%\newcommand\Monotonicity        {\X-mono\-toni\-city}
\newcommand\stable              {\X-stable}
\newcommand\Vstable             {\V-stable}
\newcommand\Ystable             {\Y-stable}
\newcommand\emptysetstable      {\mbox{$\emptyset$}-stable}
\newcommand\stability           {\X-stabi\-lity}
\newcommand\Stability           {\X-stabi\-lity}
\newcommand\Vstability          {\V-stabi\-lity}
\newcommand\VStability          {\V-stabi\-lity}
\newcommand\compatible          {\X-compa\-tible}
\newcommand\RXcompatible        {\RX-compa\-tible}
\newcommand\Vcompatible         {\V-compa\-tible}
\newcommand\Ycompatible         {\Y-compa\-tible}
\newcommand\leftrightcompatible {\X-left-right-compa\-tible}
\newcommand\Vleftrightcompatible{\V-left-right-compa\-tible}
\newcommand\dontcarecompatible  {\X-don't-care-compa\-tible}
\newcommand\aleftrightcompatible{an \X-left-right-compa\-tible}
\newcommand\adontcarecompatible {an \X-don't-care-compa\-tible}
\newcommand\compatibility       {\X-compa\-ti\-bility}
\newcommand\dontcarecompatibility{\X-don't-care-compa\-ti\-bility}
\newcommand\Vdontcarecompatible {\V-don't-care-compa\-tible}
\newcommand\Safety              {Safeness}
\newcommand\safety              {safeness}
\newcommand\safe                {safe}
\newcommand\Safe                {Safe}
\newcommand\unsafe              {unsafe}
\newcommand\safely              {safely}
\newcommand\constructorminimal{con\-struc\-tor-mini\-mal}
\newcommand\ConstructorMinimal{Con\-struc\-tor-Mini\-mal}
\newcommand\constructorminimality{con\-struc\-tor-mini\-mal\-ity}
\newcommand\constructorminimum{con\-struc\-tor-mini\-mum}
\newcommand\constructorpreserving{con\-struc\-tor-pre\-serving}
\newcommand\constructorpreservation{con\-struc\-tor-pre\-serva\-tion}
\newcommand\constructorbased{con\-struc\-tor-based}
\newcommand\Constructorbased{Con\-struc\-tor-based}
\newcommand\terminationpair{termi\-na\-tion-pair}
\newcommand\TerminationPair{Termi\-na\-tion-Pair}
\newcommand\inductivesubstitution{constructor ground substitution}
\newcommand\aninductivesubstitution{a constructor ground substitution}
\newcommand\Inductivesubstitution{Constructor ground substitution}
\newcommand\InductiveSubstitution{Constructor Ground Substitution}
\newcommand\inductiveinstance{constructor ground instance}

%Subterm
\newcommand\hiddensubST{_{_{\rm ST}}}
\mathcommand\superterm   {\rhd\hiddensubST}
\mathcommand\notsuperterm{\ntriangleright\hiddensubST}
\mathcommand\subterm     {\lhd\hiddensubST}
\mathcommand\notsubterm  {\ntriangleleft\hiddensubST}
\mathcommand\supertermeq {\trianglerighteq\hiddensubST}
\mathcommand\subtermeq   {\trianglelefteq\hiddensubST}

\mathcommand\sugarregel{l\boldequal r\rulesugar C}
\mathcommand\sugarregelindex[1]{l_{#1}\boldequal r_{#1}\rulesugar C_{#1}}
\mathcommand\sugaruncondregelindex[1]{l_{#1}\boldequal r_{#1}}
\mathcommand\ndrulewithassumption[3]{{{{\scriptstyle\lbrack}#1{\scriptstyle
\rbrack}}\atop\scriptstyle #2}\over #3}

%_____________________________________________________________________________
%Rules
\def\R{{\rm R}}
\mathcommand\RCONS{\R_\CONS}
\mathcommand\Rprime{{\rm R}'}
\mathcommand\RX{\R,\X}
\mathcommand\RCONSX{\RCONS,\X}
\mathcommand\DEFUNSYM{\mathcal{DEFUN}}
\mathapplycommand\DEFUN{\DEFUNSYM}
\newcommand\defsort{{\rm def}}
\mathcommand\ATSYM  {\mathcal{A\hspace{-.02em}T}}
\mathdoubleapplycommand\atomsof{\ATSYM}
\newcommand\atoms      {\atomsof\sig\V}
\newcommand\Xatoms     {\atomsof\sig\X}
\newcommand\Yatoms     {\atomsof\sig\Y}
\newcommand\scatoms    {\atomsof\sig\Vcons}
\mathcommand\GENATSYM  {\GENSYM\hspace{-.18em}\ATSYM}
\mathdoubleapplycommand\genatomsof{\GENATSYM}
\newcommand\genatoms      {\genatomsof\sig\V}
\newcommand\Xgenatoms     {\genatomsof\sig\X}
\newcommand\Ygenatoms     {\genatomsof\sig\Y}
\mathcommand\CONDSYM  {\mathcal{C\hspace{-.1em}O\hspace{-.12em}N\hspace{-.12em}D}}
\mathcommand\LITSYM   {\mathcal{LI\hspace{-.04em}T}}
\mathcommand\CONDLITSYM{\CONDSYM\hspace{-.04em}\LITSYM}
\mathapplycommand\condlitwitharg{\CONDLITSYM}
\newcommand\condlit {\condlitwitharg{\sig,\V}}
\newcommand\Xcondlit{\condlitwitharg{\sig,\X}}
\newcommand\Ycondlit{\condlitwitharg{\sig,\Y}}
\mathdoubleapplycommand\literals{\LITSYM}
\newcommand \lit        {\literals\sig\V}
\newcommand \Xlit       {\literals\sig\X}
\newcommand \Ylit       {\literals\sig\Y}
\mathcommand\GENLITSYM{\GENSYM\hspace{-.08em}\LITSYM}
\mathdoubleapplycommand\genliterals{\GENLITSYM}
\newcommand \genlit        {\genliterals\sig\V}
\newcommand \Xgenlit       {\genliterals\sig\X}
\newcommand \Ygenlit       {\genliterals\sig\Y}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% END %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> headernamesrest.tex <==
% FILE: headernamesrest.tex
% CONTENTS: CP's standard file for including world knowledge,
%           such as names, language, characters, life times.
%
% This file must be loadable as the first file of any latex file!
% So do not use any extensions which are not contained in it,
% such as \mathcommand
%
% Moreover, \emph must not be used here!

\usepackage{amssymb}

\input specialfonts

\newcommand\namefont{}

\hyphenation{
ab-ge-leitete
ab-ge-leitetem
ab-ge-leiteten
ab-ge-leiteter
ab-ge-leitetes
ab-weicht
accord-ing
actual
actual-ly
aktiv
aktive
aktivem
aktiven
aktiver
aktives
although
analysis
an-ge-mie-te-ten
ante-cedent
ante-cedents
appli-ca-tion
appli-ca-tions
area
areas
aspect
asser-tion
asser-tions
assump-tion
assump-tions
Aus-wahl-funktion
Aus-spra-che
author
authors
auto-ma-ted
auto-ma-tion
auto-ma-tisch
auto-ma-ti-sche
auto-ma-ti-schem
auto-ma-ti-schen
auto-ma-ti-scher
auto-ma-ti-sches
Autoren
axio-ma-tics
axiom
Axiome
axioms
basic
basis
be-ein-flusst
be-endet
beharr-lich
be-kannte
be-kanntem
be-kannten
be-kannter
be-kanntes
be-rech-tig-te
Bereich
Be-rei-chen
be-zeich-net
Be-zeich-nung
bis-heri-gen
certain
che-mi-sche
che-mi-schem
che-mi-schen
che-mi-sches
che-mi-scher
com-pati-bi-lity
concept
con-struc-tor
co-rol-lary
counter-example
creati-vity
custom-ary
Dag-stuhl
define
defi-niert
defi-nierte
defi-niertem
defi-nierten
defi-nierter
defi-niertes
defi-nit
defi-nite
defi-nitem
defi-niten
defi-niter
defi-nites
defi-ni-tion
defi-ni-tions
de-monstra-tion
der-arti-ge
der-arti-gen
der-arti-gem
der-arti-ger
der-arti-ges
De-signs
des-cente
descent
deter-mined
deutsche
deutschem
deutschen
deutscher
deutsches
develop-ing
diese
dis-equality
dis-equali-ties
durch-aus
Effi-zienz
effec-tive
ehren-amt-licher
ehren-amt-liches
ehren-amt-liche
ehren-amt-lichen
ehren-amt-lichem
eigent-lichen
Ein-arbei-tung
eine
einem
einen
einer
eines
either
elek-tro-ni-scher
elek-tro-ni-sches
elek-tro-ni-sche
elek-tro-ni-schen
elek-tro-ni-schem
element
elemen-tary
em-pfohlen
em-pfun-dener
em-pfun-denes
em-pfun-dene
em-pfun-denen
em-pfun-denem
eng-lisch
Engli-scher
Engli-sches
Engli-sche
Engli-schen
Engli-schem
englisch-sprachig
englisch-sprachi-ge
englisch-sprachi-gem
englisch-sprachi-gen
englisch-sprachi-ger
englisch-sprachi-ges
epsi-lon
equi-valent
equi-valence
essay
essays
estab-lish
evaluation
every
exist-ence
explain
explained
Ent-deckung
ent-schul-di-gen
Ent-wick-lung
Ent-wick-lun-gen
Ent-wurf
etab-lier-ter
etwas
every-where
ex-peri-ence
Ex-peri-mente
existen-tial
extra-pola-tion
fach-wissen-schaft-liche
fach-wissen-schaft-lichen
Fach-be-reich
Fahr-zeu-gen
Falsi-fi-ka-tion
father
final
finally
finite
finitis-tic
forma-tion
founda-tions
frequent
frequent-ly
further-more
general
ge-sicher-te
ge-sicher-tem
ge-sicher-ten
ge-sicher-ter
ge-sicher-tes
Ge-werk-schaft
glei-chen
Glei-chung
Glei-chun-gen
geo-metry
Gesamt-komplex
Gestalt
grie-chi-sche
grie-chi-schem
grie-chi-schen
grie-chi-scher
grie-chi-sches
groun-ded-ness
glo-bal-ly 
Grund-lage
Grund-lagen
Grund-lagen-wissen-schaft 
Grund-lagen-wissen-schaf-ten 
guaran-tee-ing
Haltung
haupt-ver-ant-wort-lich
Haupt-ver-ant-wort-liche
Haupt-ver-ant-wort-lichem
Haupt-ver-ant-wort-lichen
Haupt-ver-ant-wort-licher
Haupt-ver-ant-wort-liches
have
hin-rei-chend
hin-rei-chen-de
hin-rei-chen-dem
hin-rei-chen-den
hin-rei-chen-der
hin-rei-chen-des
hyper-text
Hyper-texte
hypo-theses
hypo-thesis
hypo-the-size
hypo-the-sizing
idealis-ti-sche
idealis-ti-schem
idealis-ti-schen
idealis-ti-scher
idealis-ti-sches
ideali-za-tion
ihre
ihrem
ihren
ihrer
ihres
indeed
in-definite
Induk-tions-be-wei-ser
Induk-tions-ord-nun-gen
Inferenz-systeme
in-finie
in-finite
in-formatics
ins-ge-samt
irreflexive
Jahres-tref-fen
je-weils
Kai-sers-lau-tern
Kaplan
Kenn-zeichen
kenn-zeich-net
knowledge
knowledge-able
klassi-sche
klassi-schen
klassi-schem
klassi-scher
konnte
Kritik
kriti-sche
kriti-schen
kriti-schem
kriti-scher
kriti-sches
Kumu-la-tion
latter
leistet
lesen
little
logic
logics
logi-sche
logi-schen
logi-schem
logi-scher
logi-sches
magni-tude
mani-fold
mani-folds
mathe-ma-tica
mathe-ma-tical
mathe-ma-tician
mathe-ma-ticians
mathe-ma-tics
Mathe-ma-tik
mathe-ma-ti-sche
mathe-ma-ti-schem
mathe-ma-ti-schen
mathe-ma-ti-scher
mathe-ma-ti-sches
method
methods
metho-di-cal
methodo-logi-sche
methodo-logi-schen
methodo-logi-schem
methodo-logi-scher
methodo-logi-sches
Modell-klasse
modern
moder-ne
moder-nem
moder-nen
moder-ner
moder-nes
mono-toni-city
mora-lisch
mora-li-sche
mora-li-schen
mora-li-schem
mora-li-scher
mora-li-sches
Mieter-sache
Miet-vertrag
Miet-vertrages
mini-mum
mis-anthropic
mis-under-stood
mitt-lere
Musik
Nach-mieterin
natu-ral
Natur-wissen-schaft
Natur-wissen-schaf-ten
Neben-kosten
nega-tiv
nega-tive
neo-logism
never-the-less
Nomina-list
Nomina-listen
notable
nothing
notion
numeral
Ober-begriff
object
objects
Objekt
occur-rence
occur-ren-ces
ohne
onto-logisch
onto-logi-sche
onto-logi-schem
onto-logi-schen
onto-logi-scher
onto-logi-sches
operationali-zation
Origi-nal
Origi-nals
Origi-nal-zitate
organi-sa-to-risch
organi-sa-to-ri-sche
organi-sa-to-ri-schem
organi-sa-to-ri-schen
organi-sa-to-ri-scher
organi-sa-to-ri-sches
para-digm
Para-digma
Para-digmas
para-digms
Parallelen-axiom
para-meter
para-meters
parti-ci-pa-tion
philo-so-phisch
philo-so-phi-sche
philo-so-phi-schem
philo-so-phi-schen
philo-so-phi-scher
philo-so-phi-sches
parallel
poly-nomial
poly-nomials
posi-tiv
posi-tive
post-humously
product
pro-posi-tion
pro-posi-tions
ratio-nalis-mus
ratio-nalis-tisch 
ratio-nalis-tische 
ratio-nalis-tischem 
ratio-nalis-tischen 
ratio-nalis-tischer 
ratio-nalis-tisches 
really
Real-wissen-schaf-ten
recht-eckige
recht-eckigem
recht-eckigen
recht-eckiger
recht-eckiges
re-cog-nition
re-duci-bi-lity
Re-duk-tions-re-la-tion
regard-less
Regel
relation-ship
relation-ships
re-organi-za-tion
repeti-tion
replace
represent
represents
repre-sen-ta-tion
reso-lu-tion
Rhein-steig
Sammel-bezeich-nung 
schrift-lich
schwerere
Schwierig-keiten
second
seiten-gleich
seiten-gleiche
seiten-gleichem
seiten-gleichen
seiten-gleiches
seiten-gleicher
seman-tic
seman-tics
sequence
sequen-ces
several
sinn-voller
sitt-lich
sitt-liche
sitt-lichem
sitt-lichen
sitt-liches
sitt-licher
speaking
solu-tion
solu-tions
Spezi-fi-ka-tio-nen
Spezi-fi-ka-tions-sprache
Sko-lem-i-za-tion
simpli-fi-cation
speci-fi-ca-tion
speci-fi-ca-tions
speci-fier
speci-fied
stable
sub-sequent
sym-metrical
sym-metrical-ly
tauto-logy
taking
tertium
theorem
theorems
Theorie
Theorien
theory
theo-re-ti-sche
theo-re-ti-schen
theo-re-ti-schem
theo-re-ti-sches
theo-re-ti-scher
topo-logy
total
trans-cend
typischer-weise
un-bestimmt
un-bestimmte
un-bestimm-tem
un-bestimm-ten
un-bestimm-ter
un-bestimm-tes
under
under-stood
unless
Un-par-tei-lich-keit
unter-bewusst
unter-schied
ur-element
ur-elements
Ur-sache
values
ver-an-lasst
Ver-an-stal-tung
Ver-bin-dung
ver-brei-ter-tem
Ver-mie-terin
ver-pflich-te-te
viel-leicht
Vor-annahme
Vor-annahmen
vor-kom-men-den
vor-para-dig-ma-ti-schen
vor-para-dig-ma-ti-scher
Vor-schrif-ten
wahr-ge-nom-men
weder
wei-te-ren
Weni-ger-ver-brauchs
wesent-liche
wesent-lichem
wesent-lichen
wesent-liches
wesent-licher
Win-kel
Wissen-schaft
Wissen-schaften
Wissen-schaft-ler
Wissen-schaft-lern
wissen-schaft-liche
wissen-schaft-lichen
wissen-schaft-licher
wissen-schaft-liches
Wissen-schafts-ent-wick-lung
wurde
zahl-reiche
zahl-reichen
zahl-reichem
zahl-reicher
zahl-reiches
zu-neh-men-den
zu-gleich
zwei-sprachi-ge
zwei-sprachi-gem
zwei-sprachi-gen
zwei-sprachi-ger
zwei-sprachi-ges
Zweit-woh-nungs-steu-er
zwischen
}

\newcommand\majorfootroom{\raisebox{-1.9ex}{\rule{0ex}{.5ex}}}
\newcommand\mediumbigfootroom{\raisebox{-1.7ex}{\rule{0ex}{.5ex}}}
\newcommand\footroom{\raisebox{-1.5ex}{\rule{0ex}{.5ex}}}
\newcommand\mediumfootroom{\raisebox{-1.25ex}{\rule{0ex}{3ex}}}
\newcommand\smallfootroom{\raisebox{-1.0ex}{\rule{0ex}{3ex}}}

\newcommand\majorheadroom{\rule{0ex}{3.2ex}}
\newcommand\headroom{\rule{0ex}{2.8ex}}
\newcommand\mediumheadroom{\rule{0ex}{2.4ex}}
\newcommand\smallheadroom{\rule{0ex}{2.0ex}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% FIRST NAMES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\alan    {Alan}
\newcommand\albert  {Al\-bert}
\newcommand\alexander{Alex\-ander}
\newcommand\alfred  {Alfred}
\newcommand\andreas {An\-dre\-a\es}
\newcommand\andrew  {An\-drew}
\newcommand\bernd   {Bernd}
\newcommand\bernard {Bernard}
\newcommand\bernhard{Bern\-hard}
\newcommand\benjamin{Benjamin}
\newcommand\carl    {Carl}
\newcommand\carlos  {Car\-lo\es}
\newcommand\carsten {Car\esi ten}
\newcommand\catherine{Catherine}
\newcommand\charles {Charle\es}
\newcommand\charybdis{Charybdi\es}
\newcommand\christian{Christian}
\newcommand\christoph{Christoph}
\newcommand\claude  {Claude}
\newcommand\claus   {Clau\es}
\newcommand\david   {Da\-vid}
\newcommand\donald  {Do\-nald}
\newcommand\dieter  {Die\-ter}
\newcommand\dirk    {Dirk}
\newcommand\edmund  {\mbox{Edmund}}
\newcommand\edgar   {\mbox{Edgar}}
\newcommand\ernst   {Ernst}
\newcommand\ferdinand{Ferdinand}
\newcommand\francois{Fran\-\c coi\es}
\newcommand\friedrich{Fried\-rich}
\newcommand\frank   {Frank}
\newcommand\gabriel {Gabri\ewithtrema l}
\newcommand\gerhard {Ger\-hard}
\newcommand\georg   {Georg}
\newcommand\george  {George}
\newcommand\gerd    {Gerd}
\newcommand\gottlob {Gott\-lob}
\newcommand\gustav  {Gustav}
\newcommand\hans    {Han\es}
\newcommand\helmut  {Hel\-mut}
\newcommand\henk    {Henk}
\newcommand\heinrich{Hein\-rich}
\newcommand\herbert {Her\-bert}
\newcommand\hermann {Her\-mann}
\newcommand\horst   {Horst}
\newcommand\howard  {{\namefont Howard}}
\newcommand\hubert  {Hubert}
\newcommand\immanuel{Immanu\ewithtrema l}
\newcommand\irving  {Irving}
\newcommand\ismael  {Isma\ewithtrema l}
\newcommand\jacques {Jacque\es}
\newcommand\james   {Jame\es}
\newcommand\jan     {Jan}
\newcommand\joachim {Jo\-achim}
\newcommand\joerg   {J\oe rg}
\newcommand\johan   {Jo\-han}
\newcommand\jose    {Jos\'e}
\newcommand\joseph  {Joseph}
\newcommand\juergen {J\ue r\-gen}
\newcommand\jean    {Jean}
\newcommand\john    {John}
\newcommand\karl    {Karl}
\newcommand\klaus   {Klau\es}
\newcommand\konrad  {Kon\-rad}
\newcommand\kurt    {Kurt}
\newcommand\lawrence{Lawrence}
\newcommand\leopold {Leo\-pold}
\newcommand\ludwig  {Lud\-wig}
\newcommand\magdalena{Magda\-lena}
\newcommand\manfred {Man\-fred}
\newcommand\maxchristianname{Max} %% \max is already a tex command
\newcommand\markus  {Mar\-ku\es}
\newcommand\martin  {Mar\-tin}
\newcommand\matthias{Matthia\es}
\newcommand\michael {Micha\-\ewithtrema l}%{Mi\-cha\-\ewithtrema l}
\newcommand\michaelwithouttrema{Micha\-el}%{Mi\-cha\-el}
\newcommand\nicolaus{Ni\-co\-lau\es}
\newcommand\ottonoconflict{Ot\-to}
\newcommand\paolo   {Paolo}
\newcommand\paul    {Paul}
\newcommand\peter   {Peter}
\newcommand\pierre  {Pierre}
\newcommand\raymond {Raymond}
\newcommand\rene    {Ren\'e}
\newcommand\redcap  {Red\-cap}
\newcommand\richard {Ri\-chard}
\newcommand\robert  {Ro\-bert}
\newcommand\roland  {Ro\-land}
\newcommand\rudolf  {Ru\-dolf}
\newcommand\ruediger{R\ue\-di\-ger}
\newcommand\scylla  {Scylla}
\newcommand\sergey  {Ser\-gey}
\newcommand\stanislaw{Stanis\l aw}
\newcommand\stanley {Stan\-ley}
\newcommand\stephan {Ste\-phan}
\newcommand\thomas  {Tho\-ma\es}
\newcommand\tobias  {{\namefont To\-bi\-a\es}}
\newcommand\wolfgang{Wolf\-gang}
\newcommand\ulrich  {Ul\-rich}
\newcommand\ulysses {Ulysse\es}
\newcommand\uwe     {Uwe}
\newcommand\vladimir{Vla\-di\-mir}
\newcommand\volker  {Vol\-ker}
\newcommand\werner  {Wer\-ner}
\newcommand\wilfried{Wil\-fried}
\newcommand\wilhelm {Wil\-helm}
\newcommand\william {Will\-iam}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SCIENTISTS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\aanderaa        {Aanderaa}
\newcommand\aanderaaname    {St\aa l \aanderaa}
\newcommand\abel            {Abel}
\newcommand\abelname        {Niel\es\ Henrik \abel} % verified
\newcommand\abellifetime    {(1802--1829)} % verified
\newcommand\acerbi          {{\namefont Acerbi}}
\newcommand\acerbiname      {{\namefont Fabio \acerbi}}
\newcommand\ackermann       {{\namefont Acker\-mann}}
\newcommand\ackermannname   {{\namefont \wilhelm\ \ackermann}}
\newcommand\ackermannlifetime{(1896--1962)}
\newcommand\aczel           {{\namefont Aczel}}
\newcommand\aczelname       {{\namefont \peter\ \aczel}}
\newcommand\adorno          {Adorno}
\newcommand\adornoname      {Theodor W. \adorno}
\newcommand\ahrendt         {{\namefont Ahrendt}}
\newcommand\ahrendtname     {{\namefont\wolfgang\ \ahrendt}}
\newcommand\ajdukiewicz     {Ajdukiewicz}
\newcommand\ajdukiewiczname {Kazimierz \ajdukiewicz}
\newcommand\ajdukiewiczlifetime{(1890--1963)}
\newcommand\anellis         {{\namefont Anelli\es}}
\newcommand\anellisname     {{\namefont\irving\ H. \anellis}}
\newcommand\albertus        {{\namefont Albertu\es}}
\newcommand\albertusname    {{\namefont\albertus\ Magnu\es}}
\newcommand\albertuslifetime{(\ca\,1200--1280)}
\newcommand\anselm          {{\namefont Anselmu\es}}
\newcommand\anselmname      {{\namefont\anselm\ Cantuariensi\es}}
\newcommand\anselmlifetime  {(1033--1109)}
\newcommand\artin           {{\namefont Artin}}
\newcommand\artinname       {{\namefont Emil \artin}}
\newcommand\artinlifetime   {(1898--1962)}
\newcommand\aristotle       {{\namefont Ari\esi totle}}
\newcommand\aristotlename   {{\namefont\aristotle\ of Stagira}}
\newcommand\aristotlelifetime{(384--322\,\BC)}
\newcommand\aristotelian    {{\namefont Ari\esi totelian}}
\newcommand\aristotelisch   {{\namefont Ari\esi totelisch}}
\newcommand\aristoteles     {{\namefont Ari\esi toteles}}
\newcommand\aristotelesname {{\namefont Ari\esi toteles von Stagira}}
\newcommand\aristoteleslifetime{(384--322\,v.\,Chr.)}
\newcommand\armando         {Armando}
\newcommand\armandoname     {Alessandro \armando}
\newcommand\asser           {{\namefont Asser}}
\newcommand\assername       {{\namefont G\ue nter \asser}}
\newcommand\asserlifetime   {(born\,1926)}
\newcommand\andrews         {{\namefont An\-drew\es}}
\newcommand\andrewsname     {{\namefont\peter\ B. \andrews}}
\newcommand\augustinus      {{\namefont Augu\esi tinus}}
\newcommand\augustinusname  {{\namefont \augustinus\ Hipponensis}}
\newcommand\augustinuslifetime{(354--430)}
\newcommand\autexier        {{\namefont Autexier}}
\newcommand\autexiername    {{\namefont Serge \autexier}}
\newcommand\avenhaus        {{\namefont Aven\-hau\es}}
\newcommand\avenhausname    {{\namefont\juergen\ \avenhaus}}
\newcommand\avron           {{\namefont Avron}}
\newcommand\avronname       {{\namefont Arnon \avron}}
\newcommand\awodey          {{\namefont Awodey}}
\newcommand\awodeyname      {{\namefont Steve \awodey}}
\newcommand\baaz            {{\namefont Baaz}}
\newcommand\baazname        {{\namefont\matthias\ \baaz}}
\newcommand\babbage         {Babbage}
\newcommand\babbagename     {\charles\ \babbage}
\newcommand\babbagelifetime {(1792--1871)}
\newcommand\bach            {Bach}
\newcommand\bachname        {Emmon \bach}
\newcommand\bachet          {Bachet}
\newcommand\bachetname      {\claude\ Gaspard \bachet\ de M\'eziriac}
\newcommand\bachetlifetime  {(1581--1638)}
\newcommand\bachmair        {Bach\-mair}
\newcommand\bachmairname    {Leo \bachmair}
\newcommand\backhouse       {Backhouse}
\newcommand\backhousename   {\roland\ \backhouse}
\newcommand\bacon           {Bacon}
\newcommand\baconname       {Franci\es\ \bacon}
\newcommand\barendregt      {Barendregt}
\newcommand\barendregtname  {Hen(dri)k P. \barendregt}
\newcommand\barwise         {Barwise}
\newcommand\barwisename     {Jon \barwise}
\newcommand\basin           {{\namefont Basin}}
\newcommand\basinname       {{\namefont\david\ \basin}}
\newcommand\bauermengelberg {{\namefont Bauer-Mengelberg}}
\newcommand\bauermengelbergname{{\namefont Stefan \bauermengelberg}}
\newcommand\baumgartner     {Baum\-gart\-ner}
\newcommand\baumgartnername {\peter\ \baumgartner}
\newcommand\becker          {Becker}
\newcommand\beckername      {\klaus\ \becker}
\newcommand\beckert         {Beckert}
\newcommand\beckertname     {\bernhard\ \beckert}
\newcommand\bell            {Bell}
\newcommand\bellname        {\john\ Lane \bell}
\newcommand\beethoven       {Beethoven}
\newcommand\beethovenname   {\ludwig\ van \beethoven}
\newcommand\beethovenlifetime{(1770--1827)}
\newcommand\behmann         {{\namefont Behmann}}
\newcommand\behmannname     {{\namefont\heinrich\ \behmann}}
\newcommand\bendix          {Bendix}
\newcommand\bendixname      {P. B. \bendix}
\newcommand\benzmueller     {{\namefont Benz\-m\ue ller}}
\newcommand\benzmuellername {{\namefont\christoph\ \benzmueller}}
\newcommand\berghammer      {Berg\-hammer}
\newcommand\berghammername  {\rudolf\ \berghammer}
\newcommand\bergstra        {{\namefont Bergstra}}
\newcommand\bergstraname    {{\namefont\jan\ A. \bergstra}}
\newcommand\berkeley        {{\namefont Berkeley}}
\newcommand\berkeleyname    {{\namefont \george\ \berkeley}}
\newcommand\berkeleylifetime{(1685--1753)}
\newcommand\bernays         {{\namefont Ber\-nay\es}}
\newcommand\bernaysname     {{\namefont \paul\ \bernays}}
%                           {{\namefont \paul\ Isaak \bernays}}
\newcommand\bernaysschoenfinkel{\bernays--\schoenfinkel}
\newcommand\bernayslifetime {(1888--1977)}
\newcommand\bertling        {{\namefont Bertling}}
\newcommand\bertlingname    {{\namefont\hubert\ \bertling}}
\newcommand\bevers          {Bever\es}
\newcommand\beversname      {Eddy \bevers}
\newcommand\bibel           {Bi\-bel}
\newcommand\bibelname       {\wolfgang\ \bibel}
\newcommand\billy           {Billy}
\newcommand\billyname       {\jacques\ de \billy}
\newcommand\billylifetime   {(1602--1679)}
\newcommand\bohr            {Bohr}
\newcommand\bohrname        {Nil\es\ \bohr}
\newcommand\bookhade        {Bookhade}
\newcommand\bookhadename    {\robert\ \bookhade}
\newcommand\boole           {{\namefont Boole}}
\newcommand\boolename       {{\namefont\george\ \boole}}
\newcommand\boolelifetime   {(1815--1864)}
\newcommand\myboolean       {Boolean}
\newcommand\boolos          {{\namefont Boolos}}
\newcommand\boolosname      {{\namefont\george\ \boolos}}
\newcommand\booloslifetime  {(1940--1996)}
\newcommand\bouhoula        {Bou\-hou\-la}
\newcommand\bouhoulaname    {Adel \bouhoula}
\newcommand\bourbaki        {Bourbaki}
\newcommand\bourbakiname    {Nicola\es\ \bourbaki}
\newcommand\boyer           {{\namefont Boyer}}
\newcommand\boyername       {{\namefont\robert\ S. \boyer}}
\newcommand\brahe           {Brahe}
\newcommand\brahename       {Tyge \brahe}%{Tyge B. \brahe}
\newcommand\brahelifetime   {(1546--1601)}
\newcommand\brentano        {{\namefont Brentano}}
\newcommand\brentanopoetname{{\namefont Clemens \brentano}}
\newcommand\brentanopoetlifetime{(1778--1842)}
\newcommand\brentanophilosophername{{\namefont Franz \brentano}}
\newcommand\brentanophilosopherlifetime{(1838--1917)}
\newcommand\bronsard        {{\namefont Bronsard}}
\newcommand\bronsardname    {{\namefont\francois\ \bronsard}}
\newcommand\brotherston     {{\namefont Brotherston}}
\newcommand\brotherstonname {{\namefont\james\ \brotherston}}
\newcommand\brouwersecondname{Brouwer} % Not: Brouwers (as often written)
\newcommand\brouwerfirstname{L. E. J.}
%{Luitzen}
%{Luitzen E. J.}
%Parsons: Also, Brouwer always referred to himself in print as L. E. J. Brouwer; that is the way most other writers have referred to him.  I don't know if anyone called him Luitzen; from van Dalen's biography, it is clear that he was known familiarly as Bertus (after Egbertus, his second Christian name).
\newcommand\brouwerindex    {\brouwersecondname, \brouwerfirstname}
\newcommand\brouwer         {{\namefont \brouwersecondname}}
\newcommand\brouwername     {{\namefont \brouwerfirstname\ \brouwersecondname}}
\newcommand\brouwerlifetime {(1881--1966)}
\newcommand\brownchad       {{\namefont Brown}}
\newcommand\brownchadname   {{\namefont Chad E. \brownchad}}
\newcommand\broy            {Broy}
\newcommand\broyname        {\manfred\ \broy}
\newcommand\bruggaier       {Bruggaier}
\newcommand\bruggaiername   {Juliana \bruggaier}
\newcommand\bruijn          {Bruijn}
\newcommand\bruijnname      {Nicolaa\es\ Govert de \bruijn}
\newcommand\buchholz        {{\namefont Buch\-holz}}
\newcommand\buchholzname    {{\namefont\wilfried\ \buchholz}}
\newcommand\buerckert       {B\ue rckert}
\newcommand\buerckertname   {\hans-\juergen\ \buerckert}
\newcommand\buldt           {{\namefont Buldt}}
\newcommand\buldtname       {{\namefont \bernd\ \buldt}}
\newcommand\bundy           {{\namefont Bundy}}
\newcommand\bundyname       {{\namefont\alan\ \bundy}}
                          %{\alan\ R. \bundy}
\newcommand\burris          {Burri\es}
\newcommand\burrisname      {\stanley\ \burris}
\newcommand\bush            {Bush}
\newcommand\bushname        {Vannevar \bush}
\newcommand\bussotti        {{\namefont Bussotti}}
\newcommand\bussottiname    {{\namefont\paolo\ \bussotti}}
\newcommand\byrnes          {Byrne\es}
\newcommand\byrnesname      {\john\ \byrnes}
\newcommand\caferra         {{\namefont Caferra}}
\newcommand\caferraname     {{\namefont Ricardo \caferra}}
\newcommand\cantone         {Cantone}
\newcommand\cantonename     {Domenico \cantone}
\newcommand\cantor          {{\namefont Cantor}}
\newcommand\cantorname      {{\namefont\georg\ \cantor}}
\newcommand\cantorlifetime  {(1845--1918)}
\newcommand\carcavi         {{\namefont Carcavi}}
\newcommand\carcaviname     {{\namefont\pierre\ de \carcavi}}
\newcommand\carnap          {{\namefont Carnap}}
\newcommand\carnapname      {{\namefont\rudolf\ \carnap}}
\newcommand\carnaplifetime  {(1891--1970)}
\newcommand\carroll         {Carroll}
\newcommand\carrollname     {Lewi\es\ \carroll}
\newcommand\carrolltrue     {Dodgson}
\newcommand\carrolltruename {\charles\ Lutwidge \carrolltrue}
\newcommand\carrolllifetime {(1832--1898)}
\newcommand\cate            {Ten Cate}
\newcommand\catename        {Balder \cate}
\newcommand\cauchy          {{\namefont Cauchy}}
\newcommand\cauchyname      {{\namefont Augustin Louis \cauchy}}
\newcommand\cauchylifetime  {(1789-1857)}
\newcommand\cavaillesname   {Jean Cavaill\`e\es}
\newcommand\cavailleslifetime{(1903--1944)}
\newcommand\cerrito         {Cerrito}
\newcommand\cerritoname     {Serenella \cerrito}
\newcommand\lassaadsecondname{{\namefont Cheikh\-rou\-hou}}
\newcommand\lassaadname     {{\namefont Las\-saad \lassaadsecondname}}
\newcommand\chrysippos      {Chrysippu\es}
\newcommand\chrysipposname  {\chrysippos\ of Soloi (Asia Minor)}
\newcommand\chrysipposlifetime{(\nth 3\,century\,\BC)}
\newcommand\chrysippossentence{\chrysippos\ sentence}
\newcommand\chevalley       {Chevalley}
\newcommand\chevalleyname   {\claude\ \chevalley}
\newcommand\chevalleylifetime{(1909--1984)}
\newcommand\church          {{\namefont Church}}
\newcommand\churchname      {{\namefont Alonzo \church}}
\newcommand\churchlifetime  {(1903--1995)}
\newcommand\churchrosser    {\church--\rosser}
\newcommand\churchrossertheorem{\churchrosser\ Theorem}
\newcommand\cialdea         {Cialdea}
\newcommand\cialdeaname     {Marta \cialdea}
\newcommand\clausius        {{\namefont Clausius}}
\newcommand\clausiusname    {{\namefont\rudolf\ \clausius}}
\newcommand\cleanthes       {Cleanthe\es}
\newcommand\cleanthesname   {\cleanthes\ of Asso\es}
\newcommand\corcoran        {Corcoran}
\newcommand\corcoranname    {\john\ \corcoran}
\newcommand\comon           {{\namefont Comon}}
\newcommand\comonname       {{\namefont\hubert\ \comon}}
\newcommand\costa           {{\namefont Costa}}
\newcommand\costaname       {{\namefont Newton C. A. da \costa}}
\newcommand\courant         {Courant}
\newcommand\courantname     {\richard\ \courant}
\newcommand\courantlifetime {(1988--1972)}
\newcommand\craig           {Craig}
\newcommand\craigname       {\william\ \craig}
\newcommand\craigsinterpolationtheorem{\craig's Interpolation Theorem}
\newcommand\crelle          {Crelle}
\newcommand\crellename      {August \leopold\ \crelle}
\newcommand\crellelifetime  {(1780--1855)}
\newcommand\dalen           {Dalen}
\newcommand\dalenname       {\dirk\ van \dalen}
\newcommand\dalenlifetime   {(born\,1932)}
\newcommand\dalton          {Dalton}
\newcommand\daltonname      {\john\ \dalton}
\newcommand\daltonlifetime  {(1766--1844)}
\newcommand\davis           {Davis}
\newcommand\davisname       {\martin\ \davis}
\newcommand\davislifetime   {(born\,1928)}
\newcommand\dawson          {Dawson}
\newcommand\dawsonname      {\john\ W. \dawson\ \jr}
\newcommand\dieudonne       {Dieudonn\'e}
\newcommand\dieudonnename   {\jean\ \dieudonne}
\newcommand\dieudonnelifetime {(1906--1992)}
\newcommand\diophantus      {Dio\-phan\-tu\es}
\newcommand\diophantusname  {\diophantus\ of Alexandria}
\newcommand\diophantuslifetime{(\nth 3\,century?)}
\newcommand\dedekind        {{\namefont Dedekind}}
\newcommand\dedekindname    {{\namefont\richard\ \dedekind}}
                           %{J. W. \richard\ \dedekind}
\newcommand\dedekindlifetime{(1831--1916)}
\newcommand\degtyarev       {Degtyarev}
\newcommand\degtyarevname   {Anatoli \degtyarev}
\newcommand\demorgan        {De-Morgan}
\newcommand\demorganname    {Augustus \demorgan}
\newcommand\demorganlifetime{(1806--1871)}
\newcommand\denjoy          {Denjoy}
\newcommand\denjoyname      {Arnaud Denjoy}
\newcommand\denjoylifetime  {(1884--1974)} % verified
\newcommand\denton          {Denton}
\newcommand\dentonname      {\john\ \denton}
\newcommand\dershowitz      {Dersho\-witz}
\newcommand\dershowitzname  {Nachum \dershowitz}
\newcommand\descartes       {De\esi carte\es}
\newcommand\descartesname   {\rene\ \descartes}
\newcommand\descarteslifetime{(1596--1650)}
\newcommand\devidi          {DeVidi}
\newcommand\devidiname      {\david\ \devidi}
\newcommand\dietrich        {{\namefont Diet\-rich}}
\newcommand\dietrichname    {{\namefont Dominik \dietrich}}
\newcommand\dixnoconflict   {Dix}
\newcommand\dixname         {\juergen\ \dixnoconlflict}
\newcommand\dixon           {{\namefont Dixon}}
\newcommand\dixonname       {{\namefont Luca\es\ \dixon}}
\newcommand\doornbos        {Doornbo\es}
\newcommand\doornbosname    {\henk\ \doornbos}
\newcommand\dreben          {{\namefont Dreben}}
\newcommand\drebenname      {{\namefont Burton \dreben}}
\newcommand\drebenlifetime  {(1927--1999)}
\newcommand\dunsscotus      {{\namefont Duns-Scotus}}
\newcommand\dunsscotusname  {{\namefont Johannes \dunsscotus}}
\newcommand\dunsscotuslifetime{(1265?--1308)}
\newcommand\egli            {Egli}
\newcommand\egliname        {Ur\es\ \egli}
\newcommand\egly            {Egly}
\newcommand\eglyname        {\uwe\ \egly}
\newcommand\ehrenfels       {Ehrenfel\es}
\newcommand\ehrenfelsname   {\christian\ von \ehrenfels}
\newcommand\ehrenfelslifetime{(1859--1932)}
\newcommand\ehrig           {{\namefont Ehrig}}
\newcommand\ehrigname       {{\namefont Hartmut \ehrig}}
\newcommand\eijck           {{\namefont Eijck}}
\newcommand\eijckname       {{\namefont \jan\ van \eijck}}
\newcommand\elsenbroich     {{\namefont Elsenbroich}}
\newcommand\elsenbroichname {{\namefont Corinna \elsenbroich}}
\newcommand\einstein        {{\namefont Ein\-stein}}
\newcommand\einsteinname    {{\namefont\albert\ \einstein}}
\newcommand\einsteinlifetime{(1879--1955)}
\newcommand\eisenstein      {Eisenstein}
\newcommand\eisensteinname  {Gotthold \eisenstein}
%                           {\ferdinand\ Gotthold \max\ \eisenstein}
\newcommand\eisensteinlifetime{(1823--1852)}
\def       \enderton        {{\namefont Enderton}}
%newcommand has problems with \end..
\def       \endertonname    {{\namefont\herbert\ B. \enderton}}
\newcommand\engesser        {{\namefont Engesser}}
\newcommand\engessername    {{\namefont\kurt\ \engesser}}
\newcommand\eschbach        {Esch\-bach}
\newcommand\eschbachname    {\robert\ \eschbach}
\newcommand\euclid          {{\namefont Euclid}}
\newcommand\euclidname      {{\namefont\euclid\ of Alexandria}}
\newcommand\euclidlifetime  {(\ca\ 300\,\BC)}
\newcommand\euler           {{\namefont Euler}}
\newcommand\eulername       {{\namefont Leon\-hard \euler}}
\newcommand\eulerlifetime   {(1707--1783)}
\newcommand\faltings        {Faltings}
\newcommand\faltingsname    {{\namefont \gerd\ \faltings}}
\newcommand\faraday         {Faraday}
\newcommand\feferman        {{\namefont Feferman}}
\newcommand\fefermanname    {{\namefont Sol(omon) \feferman}}
\newcommand\fefermanlifetime{(*1928)}
\newcommand\fefermanshename {Anita Burdman \feferman}
\newcommand\fermat          {\mbox{\namefont Fermat}}
\newcommand\fermatname      {{\namefont \pierre\ \fermat}}
\newcommand\fermatnoblename {{\namefont\pierre\ {\em de} \fermat}}
\newcommand\fermatbirthyear {1607?}
\newcommand\fermatdeathyear {1665}
\newcommand\fermatlifetime  {(\fermatbirthyear--\fermatdeathyear)}
\newcommand\letterforhuygensyear{1659}
\newcommand\letterforhuygenstitle
              {Relation des nouvelles d\'ecouvertes en la science des
              nombres}
\newcommand\letterforhuygensproofcitation
                           {\cite{fermat-oeuvres}, \Vol\,1, \p\,431\f}
\newcommand\fermatsprofession{conseilleur au parlement de Toulouse%
%et commissaire aux requ\^etes
% Das ist nur die Anfaengerposition!!!
}
\newcommand\fermatstitle    {\'eculier}
\newcommand\fermatslasttheorem{\fermat's Last Theorem}
\newcommand\fermueller      {Fer\-m\ue ller}
\newcommand\fermuellername  {\christian\ G. \fermueller}
\newcommand\fettig          {Fet\-tig-Vogt}
\newcommand\fettigname      {\roland\ \fettig}
\newcommand\feyerabend      {Feyer\-abend}
\newcommand\feyerabendname  {\paul\ \feyerabend}%{\paul\ K. \feyerabend}
\newcommand\feyerabendlifetime{(1924--1994)}
\newcommand\fiedler         {{\namefont Fiedler}}
\newcommand\fiedlername     {{\namefont Armin \fiedler}}
\newcommand\fitting         {{\namefont Fitting}}
\newcommand\fittingname     {{\namefont Melvin       \fitting}}
%                           {{\namefont Melvin C.    \fitting}}
%                           {{\namefont Melvin Ch.   \fitting}}
%                           {{\namefont Melvin Chris \fitting}}
\newcommand\fleuriot        {{\namefont Fleuriot}}
\newcommand\fleuriotname    {{\namefont\jacques\ \fleuriot}}
\newcommand\foellesdal      {F\o llesdal}
\newcommand\foellesdalname  {Dagfinn \foellesdal}
\newcommand\fraenkel        {{\namefont Fraenkel}}
\newcommand\fraenkelname    {{\namefont Adolf Abraham \fraenkel}}
\newcommand\fraenkellifetime{(1891--1965)}
\newcommand\franke          {{\namefont Franke}}
\newcommand\frankename      {{\namefont\andreas\ \franke}}
\newcommand\fraus           {Frau\es}
\newcommand\frausname       {\ulrich\ \fraus}
\newcommand\frechet         {Fr\'echet}
\newcommand\frechetname     {Maurice Ren\'e Fr\'echet}
\newcommand\frechetlifetime {(1878--1973)} % verified
\newcommand\frege           {{\namefont Frege}}
\newcommand\fregename       {{\namefont \gottlob\ \frege}}
                               %{F. L. \gottlob\ \frege}
\newcommand\fregelifetime   {(1848--1925)} 
\newcommand\Begriffsschrift {Begriff\esi schrift}
\newcommand\frenicle        {{\namefont Fr\'enicle}}
\newcommand\freniclename    {{\namefont\bernard\ \frenicle\ de Bessy}}
\newcommand\freniclelifetime{(1602?--1675)} 
\newcommand\freud           {{\namefont Freud}}
\newcommand\freudname       {{\namefont Sigmund \freud}}
\newcommand\freudlifetime   {(1856--1939)} 
\newcommand\furbach         {Furbach}
\newcommand\furbachname     {\ulrich\ \furbach}
\newcommand\furtwaengler    {Furt\-w\ae ngler}
\newcommand\furtwaenglername{\wilhelm\ \furtwaengler}
\newcommand\furtwaenglerlifetime{(1886--1954)}
\newcommand\galilei         {{\namefont Gali\-lei}}
\newcommand\galileiname     {{\namefont Gali\-leo \galilei}}
\newcommand\galileilifetime {(1564--1642)}
\newcommand\gaillard        {{\namefont Gaillard}}
\newcommand\gaillardname    {{\namefont \francois\ \gaillard}}
\newcommand\galois          {Galoi\es}
\newcommand\galoisname      {Evariste \galois}
\newcommand\galoislifetime  {(1811--1832)}
\newcommand\gabbay          {{\namefont Gabbay}}
\newcommand\gabbayname      {{\namefont Dov \gabbay}}
%                           {{\namefont Dov M. \gabbay}}
\newcommand\jamiegabbayname {{\namefont Murdoch J. \gabbay}}
\newcommand\michaelgabbayname{{\namefont\michaelwithouttrema\ \gabbay}}
\newcommand\gallier         {Gallier}
\newcommand\galliername     {\jean\ \gallier}
\newcommand\ganzinger       {Gan\-zin\-ger}
\newcommand\ganzingername   {Harald \ganzinger}
\newcommand\gauss           {{\namefont Gau\sz}}
\newcommand\gaussname       {{\namefont\carl\ \friedrich\ \gauss}}
\newcommand\gausslifetime   {(1777--1855)}
\newcommand\gentzen         {{\namefont Gentzen}}
\newcommand\gentzenlifetime {(1909--1945)}
\newcommand\gentzenname     {{\namefont\gerhard\ \gentzen}}
\newcommand\gentzensHauptsatz{{\namefont\gentzen}'\es\ {\germanfont \Hauptsatz}}
\newcommand\gentzensverschaerfterHauptsatz
{{\namefont\gentzen}'\es\ {\germanfont\verschaerfterHauptsatz}}
\newcommand\gentzensverschaerfterHauptsatzfootnote
{{\namefont\gentzen}'\es\ {\germanfontfootnote\verschaerfterHauptsatz}}
\newcommand\verschaerfterHauptsatz{Ver\-sch\ae rf\-ter \Hauptsatz}
\newcommand\Hauptsatz{Haupt\-satz}
\newcommand\gerson          {Gerson}
\newcommand\gersonname      {Levi ben \gerson}
\newcommand\gersonlifetime  {(1288--1344)}
\newcommand\geurts          {Geurt\es}
\newcommand\geurtsname      {Bart \geurts}
\newcommand\geser           {Geser}
\newcommand\gesername       {Alfons \geser}
\newcommand\giese           {{\namefont Giese}}
\newcommand\giesename       {{\namefont\martin\ \giese}}
\newcommand\giesl           {Giesl}
\newcommand\gieslname       {\juergen\ \giesl}
\newcommand\gilmore         {Gilmore}
\newcommand\gilmorename     {\paul\ C. \gilmore}
\newcommand\gilmorelifetime {(born\,1925)}
\newcommand\goedel          {{\namefont G\oe del}}
\newcommand\goedelname      {{\namefont \kurt\ \goedel}}
\newcommand\goedellifetime  {(1906--1978)}
\newcommand\goedelssecondincompletenesstheorem
{\goedel'\es\ \secondincompletenesstheorem}
\newcommand\goedelssecondIncompletenessTheorem
{\goedel'\es\ \secondIncompletenessTheorem}
\newcommand\secondincompletenesstheorem{\nth 2 \incompletenesstheorem}
\newcommand\secondIncompletenessTheorem{\nth 2 \IncompletenessTheorem}
\newcommand\incompletenesstheorem{incompleteness theorem}
\newcommand\IncompletenessTheorem{Incompleteness Theorem}
\newcommand\goethe          {G\oe the}
\newcommand\goethename      {Johann \wolfgang\ von \goethe}
\newcommand\gogolla         {Gogolla}
\newcommand\gogollaname     {\martin\ \gogolla}
\newcommand\goguen          {{\namefont Goguen}}
\newcommand\goguenname      {{\namefont\joseph\ \goguen}}
\newcommand\goldbachname    {{\namefont\christian\ \goldbach}}
\newcommand\goldbach        {{\namefont Gold\-bach}}
\newcommand\goldbachlifetime{(1690--1764)}
\newcommand\goldbachsconjecture{\goldbach's Conjecture}
\newcommand\goldfarb        {{\namefont Gold\-farb}}
\newcommand\goldfarbname    {{\namefont Warren %D.
                              \goldfarb}}
\newcommand\goldstein       {Gold\-stein}
\newcommand\goldsteinname   {\catherine\ \goldstein}
\newcommand\gonseth         {{\namefont Gonseth}}
\newcommand\gonsethname     {{\namefont \ferdinand\ \gonseth}}
\newcommand\gow             {{\namefont Gow}}
\newcommand\gowname         {{\namefont Jeremy \gow}}
\newcommand\gramlich        {{\namefont Gram\-lich}}
\newcommand\gramlichname    {{\namefont\bernhard\ \gramlich}}
\newcommand\greensurname    {{\namefont Green}}
\newcommand\greenname       {{\namefont Ian \greensurname}}
\newcommand\grimm           {Grimm}
\newcommand\grimmjacobname  {Jacob \grimm}
\newcommand\grimmwilhelmname{\wilhelm\ \grimm}
\newcommand\guillaume       {{\namefont Guillaume}}
\newcommand\guillaumename   {{\namefont Marcel \guillaume}}
\newcommand\gurevich        {{\namefont Gurevich}}
\newcommand\gurevichname    {{\namefont Yuri \gurevich}}
\newcommand\hadamard        {{\namefont Hadamard}}
\newcommand\hadamardname    {{\namefont\jacques\ Salomon \hadamard}}
\newcommand\hadamardlifetime{(1865--1963)}
\newcommand\haehnle         {H\ae hnle}
\newcommand\haehnlename     {Reiner \haehnle}
\newcommand\haerdername     {Theo H\ae r\-der}
\newcommand\hahn            {{\namefont Hahn}}
\newcommand\hahnname        {{\namefont\ottonoconflict\ \hahn}}
\newcommand\hahnlifetime    {(1879--1968)}
\newcommand\hallmann        {{\namefont Hall\-mann}}
\newcommand\hallmannname    {{\namefont\andreas\ \hallmann}}
\newcommand\hailperin       {{\namefont Hailperin}}
\newcommand\hailperinname   {{\namefont Theodore \hailperin}}
\newcommand\hamilton        {{\namefont Hamilton}}
\newcommand\hamiltonname    {{\namefont Geoff \hamilton}}
\newcommand\hamoen          {Hamoen}
\newcommand\hamoenname      {Erik \hamoen}
\newcommand\hanus           {Hanu\es}
\newcommand\hanusname       {\michael\ \hanus}
\newcommand\harmelen        {{\namefont Harmelen}}
\newcommand\harmelenname    {{\namefont\frank\ van \harmelen}}
\newcommand\hartogs         {{\namefont Hartogs}}
\newcommand\hartogsname     {{\namefont\friedrich\ \hartogs}}
\newcommand\hartogslifetime {(1874--1943)}
\newcommand\hartogswellorderingtheorem{\hartogs' Ordinal Theorem}
\newcommand\hasenjaeger     {{\namefont Hasenjaeger}}
\newcommand\hasenjaegername {{\namefont Gisbert \hasenjaeger}}
\newcommand\hasse           {Hasse}
\newcommand\hassename       {\helmut\ \hasse}
\newcommand\hasselifetime   {(1898--1979)}
\newcommand\hecke           {{\namefont Hecke}}
\newcommand\heering         {Heering}
\newcommand\heeringname     {\jan\ \heering}
\newcommand\heidegger       {\mbox{\namefont Heidegger}}
\newcommand\heideggername   {{\namefont\martin\ \heidegger}}
\newcommand\heijenoort      {Hei\-jen\-oort}
\newcommand\heijenoortname  {{\namefont\jean\ %L. M. 
                              van \heijenoort}}
\newcommand\heijenoortdeathyear{1986}
\newcommand\heijenoortlifetime{(1912--\heijenoortdeathyear)}
\newcommand\heijenoortonherbrandunpublishedtitle
{On the relation between the Falsifiability Tree Method and the 
\herbrand\ Method in Quantification Theory}
\newcommand\helmholtz       {{\namefont Helm\-holtz}}
\newcommand\helmholtzname   {{\namefont \hermann\ von \helmholtz}}
\newcommand\helmholtzlifetime{(1821--1894)}
\newcommand\herbrand        {{\namefont Herbrand}}
\newcommand\herbrandname    {{\namefont \jacques\ \herbrand}}
\newcommand\herbrandlifetime{(1908--1931)}
\newcommand\herbrandbirthday{\Feb\,12, 1908}
\newcommand\herbranddeathday{\Jul\,27, 1931}
\newcommand\herbrandPhDtitle
{Recherches sur la th\'eorie de la d\'e\-mon\-stra\-tion}
\newcommand\herbrandPhDdefensedate{\Jun\,11, 1930}
\newcommand\herbrandPhDapprovedforpublicationdate{\Jun\,20, 1929}
\newcommand\herbrandPhDdating{\Apr\,14, 1929}
\newcommand\herbrandtogoedeldate{\Apr\,7, 1931}
\newcommand\herbrandsfundamentaltheorem{\herbrand'\es\ \fundamentaltheorem}
\newcommand\fundamentaltheorem{Fundamental Theorem}
\newcommand\herbrandribet   {\herbrand--\ribet}
\newcommand\heisenberg      {{\namefont Heisen\-berg}}
\newcommand\heisenbergname  {{\namefont\werner\ \heisenberg}}
\newcommand\heisenberglifetime{(1901--1976)}
\newcommand\hermes          {{\namefont Herme\es}}
\newcommand\hermesname      {{\namefont\hans\ \hermes}}
\newcommand\hertz           {{\namefont Hertz}}
\newcommand\hertzeinsname   {{\namefont\heinrich\ \hertz}}
\newcommand\hertzzweiname   {{\namefont\gustav  \ \hertz}}
\newcommand\hertzdreiname   {{\namefont\paul    \ \hertz}}
\newcommand\hertzeinslifetime{(1857--1894)}
\newcommand\hertzzweilifetime{(1887--1975)}
\newcommand\hertzdreiphysicistlifetime {(1881--1940)}
\newcommand\hertzdreipoliticianlifetime{(1888--1961)}
\newcommand\heusinger       {Heusinger}
\newcommand\heusingername   {\klaus\ von \heusinger}
\newcommand\heyting         {{\namefont Heyting}}
\newcommand\heytingname     {{\namefont Arend \heyting}}
\newcommand\heytinglifetime {(1898--1980)}
\newcommand\henkin          {{\namefont Henkin}}
\newcommand\henkinname      {{\namefont Leon \henkin}}
\newcommand\henkinlifetime  {(1921--2006)}
\newcommand\hilbert         {{\namefont Hil\-bert}}
\newcommand\hilbertname     {{\namefont \david\ \hilbert}}
\newcommand\hilbertlifetime {(1862--1943)}
\newcommand\hilbertsprogram {\hilbert'\es\ programme}
\newcommand\hilbertsProgram {\hilbert'\es\ Programme}
\newcommand\hilbertsepsilon {\hilbert'\es\ \nlbmath\varepsilon}
\newcommand\hilbertbernaysproject{{\namefont\hilbert\ \bernays\ Pro\-ject}}
\newcommand\hillenbrand     {{\namefont Hillenbrand}}
\newcommand\hillenbrandname {{\namefont\thomas\ \hillenbrand}}
\newcommand\hintermeier     {Hinter\-meier}
\newcommand\hintermeiername {\claus\ \hintermeier}
\newcommand\hintikka        {Hintikka}
\newcommand\hintikkaname    {Jaakko \hintikka}%{K. Jaakko J. \hintikka}
\newcommand\hippasos        {{\namefont Hippasu\es}}
\newcommand\hippasosname    {{\namefont\hippasos\ of Metapontum}}
\newcommand\hippasoslifetime{(\ca\ 550\,\BC)}
\newcommand\hippasosgerman  {{\namefont Hippaso\es}}
\newcommand\hippasosnamegerman{{\namefont\hippasosgerman\ von Metapont}}
\newcommand\hoare           {Hoare}
\newcommand\hoarename       {C. A. R. \hoare}
\newcommand\hobbs           {Hobb\es}
\newcommand\hobbsname       {Jerry R. \hobbs}
\newcommand\hoeven          {Hoeven}
\newcommand\hoevenname      {Jori\es\ van der \hoeven}
\newcommand\hogger          {{\namefont Hogger}}
\newcommand\hoggername      {{\namefont Christopher \john\ \hogger}}
\newcommand\horacek         {{\namefont Horacek}}
\newcommand\horacekname     {{\namefont\helmut\ \horacek}}
\newcommand\howardname      {{\namefont\paul\ \howard}}
\newcommand\huebner         {H\ue bner}
\newcommand\huebnername     {Malte \huebner}
\newcommand\hudlak          {Hudlak}
\newcommand\hudlakname      {\paul\ \hudlak}
\newcommand\huet            {Huet}
\newcommand\huetname        {G\'erard \huet}
\newcommand\huff            {{\namefont Huff}}
\newcommand\huffname        {{\namefont\george\ \huff}}
\newcommand\hullot          {Hullot}
\newcommand\hullotname      {\jean-Marie \hullot}
\newcommand\humboldt        {{\namefont Hum\-boldt}}
\newcommand\humboldtname    {{\namefont Alexander von \humboldt}}
\newcommand\humboldtlifetime{(1769--1859)}
\newcommand\hume            {{\namefont Hume}}
\newcommand\humename        {{\namefont \david\ \hume}}
\newcommand\humelifetime    {(1711--1776)}
\newcommand\huntington      {{\namefont Huntington}}
\newcommand\huntingtonname  {{\namefont Edward V. \huntington}}
\newcommand\husserl         {{\namefont Husserl}}
\newcommand\husserlname     {{\namefont\edmund\ \husserl}}
\newcommand\husserllifetime {(1859--1938)}
\newcommand\hutter          {{\namefont Hutter}}
\newcommand\huttername      {{\namefont\dieter\ \hutter}}
\newcommand\huygens         {{\namefont Huygen\es}}
\newcommand\huygensname     {{\namefont Christiaan \huygens}}
\newcommand\huygenslifetime {(1629--1695)}
\newcommand\ireland         {{\namefont Ireland}}
\newcommand\irelandname     {{\namefont\andrew\ \ireland}}
\newcommand\jouannaud       {Jouannaud}
\newcommand\jouannaudname   {\jean-\pierre\ \jouannaud}
\newcommand\kahle           {{\namefont Kahle}}
\newcommand\kahlename       {{\namefont Rein\-hard \kahle}}
\newcommand\kalmar          {{\namefont Kalm\'ar}}
\newcommand\kalmarname      {{\namefont L\'aszl\'o \kalmar}}
\newcommand\kalmarlifetime  {(1905--1976)}
\newcommand\kamp            {Kamp}
\newcommand\kampname        {\hans\ \kamp}
\newcommand\kanger          {Kan\-ger}
\newcommand\kangername      {Stig \kanger}
\newcommand\kant            {{\namefont Kant}}
\newcommand\kantname        {{\namefont\immanuel\ \kant}}
\newcommand\kantdeathyear   {1804}
\newcommand\kantlifetime    {(1724--\kantdeathyear)}
\newcommand\kaplan          {Kaplan}
\newcommand\kaplanname      {St\'ephane \kaplan}
\newcommand\kapur           {Kapur}
\newcommand\kapurname       {Deepak \kapur}
\newcommand\kaufmann        {{\namefont Kaufmann}}
\newcommand\kaufmannname    {{\namefont Matt \kaufmann}}
\newcommand\kelley          {{\namefont Kelley}}
\newcommand\kelleyname      {{\namefont \john\ L. \kelley}}
\newcommand\kelleylifetime  {(1916--1999)}
\newcommand\kepler          {{\namefont Kepler}}
\newcommand\keplername      {{\namefont Johanne\es\ \kepler}}
\newcommand\keplerlifetime  {(1571--1630)}
\newcommand\kerber          {Kerber}
\newcommand\kerbername      {\manfred\ \kerber}
\newcommand\kernighan       {Kernighan}
\newcommand\kernighanname   {Brian W. \kernighan}
\newcommand\kleene          {Kleene}
\newcommand\kleenename      {Stephen C. \kleene}%{Stephen Cole \kleene}
\newcommand\klint           {Klint}
\newcommand\klintname       {\paul\ \klint}
\newcommand\klop            {Klop}
\newcommand\klopname        {\jan\ Willem \klop}
\newcommand\knuth           {Knuth}
\newcommand\knuthname       {\donald\ E. \knuth}
\newcommand\koenig          {K\oe nig}
\newcommand\koenigname      {\koenig}
\newcommand\koenigslemma    {\koenig's Lemma}
\newcommand\kohlhase        {{\namefont Kohl\-hase}}
\newcommand\kohlhasename    {{\namefont\michael\ \kohlhase}}
\newcommand\koller          {Koller}
\newcommand\kollername      {\alexander\ \koller}
\newcommand\kopernik        {Koper\-nik}% Das ist der einzige korrekte 
                                     % original polnische Name!
\newcommand\kopernikname    {Niko\-lau\es\ \kopernik}
\newcommand\koperniklifetime{(1473--1543)}
\newcommand\kopernikan      {\kopernik an}
\newcommand\kopernikanisch  {\kopernik a\-nisch}
\newcommand\kounalis        {Kounali\es}
\newcommand\kounalisname    {Emmanu\ewithtrema l \kounalis}
\newcommand\knaster         {{\namefont Knaster}}
\newcommand\knastername     {{\namefont Bronis\l aw \knaster}}
\newcommand\knasterlifetime {(1893--1990)}
\newcommand\knastertarski   {\knaster--\tarski}
\newcommand\kreisel         {{\namefont Kreisel}}
\newcommand\kreiselname     {{\namefont\georg\ \kreisel}}
\newcommand\kreisellifetime {(born\,1923)}
\newcommand\kreowski        {{\namefont Kreow\-ski}}
\newcommand\kreowskiname    {{\namefont\hans-\joerg\ \kreowski}}
\newcommand\kronecker       {{\namefont Kronecker}}
\newcommand\kroneckername   {{\namefont\leopold\ \kronecker}}
\newcommand\kroneckerlifetime{(1823--1891)}
\newcommand\kruskal         {Kruskal}
\newcommand\kruskalname     {\joseph\ B. \kruskal}
\newcommand\kuechlin        {K\ue ch\-lin}
\newcommand\kuechlinname    {\wolfgang\ \kuechlin}
\newcommand\kuehler         {{\namefont K\ue h\-ler}}
\newcommand\kuehlername     {{\namefont\ulrich\ \kuehler}}
\newcommand\kuhn            {{\namefont Kuhn}}
\newcommand\kuhnname        {{\namefont\thomas\ S. \kuhn}}
\newcommand\kuhnlifetime    {(1922--1996)}
\newcommand\kummer          {Kummer}
\newcommand\kummername      {\ernst\ Eduard \kummer}
\newcommand\kummerlifetime  {(1810--1893)}
\newcommand\kuratowski      {Kuratowski}
\newcommand\kuratowskiname  {Kazimierz \kuratowski}
\newcommand\kuratowskilifetime{(1896--1980)}
\newcommand\landau          {{\namefont\Landau}}
\newcommand\landauname      {{\namefont\edmund\ G. H. \landau}}
                           % G. H. = Georg Hermann
\newcommand\landaulifetime  {(1877--1938)}
\newcommand\lankford        {Lankford}
\newcommand\lankfordname    {Dalla\es\ S. \lankford}
\newcommand\laotse          {Lao\-zi}
\newcommand\laotsename      {\laotse}
\newcommand\taoteking       {Tao Te King}
\newcommand\lautman         {Laut\-man}
\newcommand\lautmanname     {\albert\ \lautman}
\newcommand\lautmanlifetime {(1908--1944)}
\newcommand\lavoisier       {La\-voi\-sier}
\newcommand\lavoisiername   {Antoine Laurent de \lavoisier}
\newcommand\lavoisierlifetime{(1743--1794)}
\newcommand\lee             {Lee}
\newcommand\leename         {\richard\ C.-T. \lee}
\newcommand\leeuwen         {Leeuwen}
\newcommand\leeuwenname     {\jan\ van \leeuwen}
\newcommand\lehmann         {{\namefont Lehmann}}
\newcommand\lehmannname     {{\namefont Daniel \lehmann}}
\newcommand\leibniz         {{\namefont Leibniz}}
\newcommand\leibnizname     {{\namefont Gottfried \wilhelm\ \leibniz}}
\newcommand\leibnizlifetime {(1646--1716)}
\newcommand\leisenring      {{\namefont Leisen\-ring}}
\newcommand\leisenringname  {{\namefont\leisenringfirstname\ \leisenring}}
\newcommand\leisenringfirstname
                            {\albert\ C.}
                            %{Al C.}
                            %{A. C.}
                            %{Al(bert) C.}
\newcommand\leisenringlifetime{(born\,1941?)}
\newcommand\leibowitz       {Leibowitz}
\newcommand\leibowitzname   {\rene\ \leibowitz}
\newcommand\leibowitzlifetime{(1913--1972)}
\newcommand\leitsch         {{\namefont Leitsch}}
\newcommand\leitschname     {{\namefont\alexander\ \leitsch}}
\newcommand\lenart          {{\namefont Lenart}}
\newcommand\lenartname      {{\namefont Mihaly \lenart}}
\newcommand\lesniewski      {{\namefont Le\'sniewski}}
\newcommand\lesniewskiname  {{\namefont\stanislaw\ \lesniewski}}
\newcommand\lesniewskilifetime{(1886--1939)}
\newcommand\letz            {Letz}
\newcommand\letzname        {Rein\-hold \letz}
\newcommand\levyname        {\jean-\jacques\ L\'evy}
\newcommand\lewi            {{\namefont Lewi}}
\newcommand\lewiname        {{\namefont\johan\ \lewi}}
\newcommand\lewis           {{\namefont Lewis}}
\newcommand\lewisname       {{\namefont Clarence \irving\ \lewis}}
\newcommand\lewislifetime   {(1883--1964)}
\newcommand\lewy            {{\namefont Lewy}}
\newcommand\lewyname        {{\namefont\hans\ \lewy}}
\newcommand\lewylifetime    {(1904--1980)}
\newcommand\lifschitz       {Lifschitz}
\newcommand\lifschitzname   {\vladimir\ A. \lifschitz}
\newcommand\lindner         {{\namefont Lindner}}
\newcommand\lindnername     {{\namefont\wolfgang\ \lindner}}
\newcommand\linne           {{\namefont Linn\'e}}
\newcommand\linnename       {{\namefont\carl\ von \linne}}
\newcommand\linnelifetime   {(1707--1778)}
\newcommand\loechner        {{\namefont L\oe chner}}
\newcommand\loechnername    {{\namefont\bernd\ \loechner}}
\newcommand\loewenheim      {{\namefont L\oe wen\-heim}}
\newcommand\loewenheimname  {{\namefont\leopold\ \loewenheim}}
\newcommand\loewenheimlifetime{(1878--1957)}
\newcommand\loewenheimskolem{\loewenheim--\skolem}
\newcommand\loewenheimskolemtheorem{\loewenheimskolem\ Theorem}
\newcommand\upwardloewenheimskolemtarskitheorem
{Upward \loewenheimskolem--\tarski\ Theorem}
\newcommand\loef            {{\namefont\martin-L\oe f}}
\newcommand\loefname        {{\namefont Per \loef}}
\newcommand\loria           {Lor\'\i a-S\'aenz}
\newcommand\lorianame       {\carlos\ A. \loria}
\newcommand\liouville       {Liouville}
\newcommand\liouvillename   {\joseph\ \liouville}
\newcommand\liouvillelifetime{(1809--1882)}
\newcommand\lukasiewicz     {{\namefont \L uka\-sie\-wicz}}
\newcommand\lukasiewiczname {{\namefont\jan\ \lukasiewicz}}
\newcommand\lukasiewiczlifetime{(1878--1956)}
\newcommand\titlelukasiewicztarski 
          {Unter\-suchungen \ue ber den Au\esi sagen\-kalk\ue l}
\newcommand\lunde           {Lunde}
\newcommand\lundename       {\ruediger\ \lunde}
\newcommand\luther          {{\namefont Luther}}
\newcommand\luthername      {{\namefont\martin\ \luther}}
\newcommand\lutherlifetime  {(1483--1546)}
\newcommand\macqueen        {MacQueen}
\newcommand\macqueenname    {\david\ B. \macqueen}
\newcommand\madlener        {Mad\-lener}
\newcommand\madlenername    {\klaus\ \madlener}
\newcommand\mahr            {Mahr}
\newcommand\mahrname        {\bernd\ \mahr}
\newcommand\makinson        {{\namefont Makinson}}
\newcommand\makinsonname    {{\namefont\david\ \makinson}}
\newcommand\mancosu         {{\namefont Mancosu}}
\newcommand\mancosuname     {{\namefont\paolo\ \mancosu}}
\newcommand\mann            {{\namefont Mann}}
\newcommand\mannname        {{\namefont\thomas\ \mann}}
\newcommand\mannlifetime    {(1875--1955)}
\newcommand\manna           {Manna}
\newcommand\mannaname       {Zohar \manna}
\newcommand\manolios        {{\namefont Manolio\es}}
\newcommand\manoliosname    {{\namefont Panagioti\es\ ``Pete'' \manolios}}
\newcommand\maslov          {Maslov}
\newcommand\maslovname      {\sergey\ Yu.\ \maslov}
\newcommand\mattick         {Mattick}
\newcommand\mattickname     {\volker\ \mattick}
\newcommand\maurolycus      {Maurolico}
\newcommand\maurolycuslatin {Maurolycu\es}
\newcommand\maurolycusname  {Francisco \maurolycus}
\newcommand\maurolycuslifeplace{Messina}
\newcommand\maurolycuslifetime{(1494--1575)}
\newcommand\meier           {{\namefont Meier}}
\newcommand\meiername       {{\namefont\andreas\ \meier}}
\newcommand\meinong         {Meinong}
\newcommand\meinongname     {Alexiu\es\ \meinong}
\newcommand\meinonglifetime {(1853--1920)}
\newcommand\Gegenstand      {Gegen\-stand}
\newcommand\Gegenstandstheorie{\Gegenstand\esi theo\-rie}
\newcommand\melis           {{\namefont Meli\es}}
\newcommand\melisname       {{\namefont Erica \melis}}
\newcommand\mendelssohn     {{\namefont Mendel\esi sohn}}
\newcommand\mendelssohnname {{\namefont Moses \mendelssohn}}
\newcommand\mendelssohnlifetime{(1729--1786)}
\newcommand\meseguer        {Meseguer}
\newcommand\meseguername    {\jose\ \meseguer}
\newcommand\meyerviol       {Meyer-Viol}
\newcommand\meyerviolname   {\wilfried\ P. M. \meyerviol}
\newcommand\middeldorp      {Middel\-dorp}
\newcommand\middeldorpname  {Aart \middeldorp}
\newcommand\miller          {{\namefont Mil\-ler}}
\newcommand\millername      {{\namefont Dale A. \miller}} 
% {Dale \miller} As his supervisor Peter Andrews
% cites him with middle initial, we had better do so, too
\newcommand\mints           {Mint\es}
\newcommand\mintsname       
{{\namefont Grigori    \mints}}
%{{\namefont Grigori E. \mints}}
\newcommand\mitchell        {Mitchell}
\newcommand\mitchellname    {Oscar \howard\ \mitchell} 
\newcommand\mitchelllifetime{(1851--1889)}
\newcommand\mitchelldeathdate{\Mar\,29, 1889}
\newcommand\mitchelldeathcourse{pneumonia}
% Lungenentzuendung, Quelle: Peirce, Chronological Edition, Vol. 6, p.lvi
\newcommand\montanari       {{\namefont Montanari}}
\newcommand\montanariname   {{\namefont Ugo \montanari}}
\newcommand\moore           {{\namefont Moore}}
\newcommand\moorename       {{\namefont J S.       \moore}}
%                           {{\namefont J Strother \moore}}
\newcommand\morse           {{\namefont Morse}}
\newcommand\morsename       {{\namefont Anthony P.    \morse}}
%                           {{\namefont Anthony Percy \morse}}
\newcommand\morselifetime   {(1911--1984)}
\newcommand\MKlong          {\morse--\kelley}
\newcommand\MKshort         {{\sc MK}}
\newcommand\moschner        {{\namefont Moschner}}
\newcommand\moschnername    {{\namefont\markus\ \moschner}}
\newcommand\moser           {{\namefont Moser}}
\newcommand\mosername       {{\namefont\georg\ Ch.\ \moser}}
\newcommand\moss            {Mo\ses}
\newcommand\mossname        {\lawrence\ \moss}
\newcommand\mostowski       {{\namefont Mostowski}}
\newcommand\mostowskiname   {{\namefont Andrzej \mostowski}}
\newcommand\mostowskilifetime{(1913--1975)}
\newcommand\mozart          {\mbox{\namefont Mozart}}
\newcommand\mozartname      {{\namefont\wolfgang\ Amadeus \mozart}}
\newcommand\mozartlifetime  {(1756--1791)}
\newcommand\mueller         {{\namefont M\ue ller}}
\newcommand\muellername     {{\namefont Gert H. \mueller}}
\newcommand\musser          {{\namefont Musser}}
\newcommand\mussername      {{\namefont\david\ R. \musser}}
\newcommand\narendran       {Narendran}
\newcommand\narendranname   {Paliath \narendran}
\newcommand\nebel           {Nebel}
\newcommand\nebelname       {\bernhard\ \nebel}
\newcommand\nicolosi        {Nicolosi-Asmundo}
\newcommand\nicolosiname    {Marianna \nicolosi}
\newcommand\neumann         {{\namefont Neumann}}
\newcommand\neumannname     
{{\namefont\john\    von \neumann}}
%{{\namefont\john\ L. von \neumann}}
\newcommand\neumannlifetime {(1903--1957)}
\newcommand\NBGlong         {\neumann--\bernays--\goedel}
\newcommand\NBGshort        {{\sc NBG}}
\newcommand\newman          {Newman}
\newcommand\newmanname      {M. H. A. \newman}
\newcommand\newmanlemma     {\newman\ Lemma}
\newcommand\newton          {{\namefont Newton}}
\newcommand\newtonname      {{\namefont Isaac \newton}}
\newcommand\newtonlifetime  {(1643--1727)}
\newcommand\nieuwenhuis     {Nieuwenhui\es}
\newcommand\nieuwenhuisname {\robert\ \nieuwenhuis}
\newcommand\nipkow          {{\namefont Nipkow}}
\newcommand\nipkowname      {{\namefont\tobias\ \nipkow}}
\newcommand\nicod           {{\namefont Nicod}}
\newcommand\nicodname       {{\namefont\jean\ \nicod}}
\newcommand\nicodlifetime   {(1893--1924)}
\newcommand\nicolauscusanus {\nicolaus}
\newcommand\nicolauscusanusname{\nicolauscusanus\ of Cu\ewithtrema\es}
\newcommand\nicolauscusanuslifetime{(1401--1464)}
\newcommand\noether         {{\namefont Noether}}
%                           {{\namefont N\oe ther}}
% Though ``N\oe ther'' is also definitely correct as a ligature and is also
% the version of the birth certificate of Emmy,
% in the old age Max and in her adult age Emmy never used the 
% umlaut
\newcommand\noethername     {{\namefont Emmy \noether}}
%                           {{\namefont A. Emmy \noether}}
\newcommand\noetherfathername{\maxchristianname\ \noether}
\newcommand\noetherbirthyear{1882}
\newcommand\noetherdeathyear{1935}
\newcommand\noetherlifetime {(\noetherbirthyear--\noetherdeathyear)}
\newcommand\noetherfatherlifetime {(1844--1921)}
\newcommand\noetherian      {\noether ian}
\newcommand\theoremofnoetherianinduction{Theorem of\/ \noetherian\ Induction}
\newcommand\axiomofstructuralinductionfirsthalf{Axiom}
\newcommand\axiomofstructuralinductionsecondhalf{of Structural Induction}
\newcommand\axiomofstructuralinduction{\axiomofstructuralinductionfirsthalf\ 
\axiomofstructuralinductionsecondhalf}
\newcommand\axiomofchoice   {Axiom of Choice}
\newcommand\axiomofcollection{Axiom of Collection}
\newcommand\nonnengart      {Nonnengart}
\newcommand\nonnengartname  {\andreas\ \nonnengart}
\newcommand\nourani         {Nourani}
\newcommand\nouraniname     {Cyru\es\ F. \nourani}
\newcommand\okadaname       {Mitsuhiro Okada} 
\newcommand\ockham          {{\namefont Ockham}}
\newcommand\ockhamname      {{\namefont \william\ of \ockham}}
\newcommand\ockhamlifetime  {(1285--1347)}
\newcommand\oostrom         {{\namefont Oostrom}}
\newcommand\oostromname     {{\namefont Vincent van \oostrom}}
\newcommand\orevkov         {Orevkov}
\newcommand\orevkovname     {\vladimir\ P. \orevkov}
\newcommand\ottoname        {\friedrich\ \ottonoconflict}
\newcommand\padawitz        {{\namefont Pada\-witz}}
\newcommand\padawitzname    {{\namefont\peter\ \padawitz}}
\newcommand\paley           {Paley}
\newcommand\paleyname       {\raymond\ \paley}
\newcommand\paleylifetime   {(1907--1933)}
\newcommand\pandora         {Pandora}
\newcommand\parsons         {{\namefont Parsons}}
\newcommand\parsonsname     {{\namefont\charles\ \parsons}}
\newcommand\pascal          {Pascal}
\newcommand\pascalname      {Blaise \pascal}
\newcommand\pascalbirthyear {1623}
\newcommand\pascaldeathyear {1662}
\newcommand\pascallifetime  {(\pascalbirthyear--\pascaldeathyear)}
\newcommand\pasztor         {Pasztor}
\newcommand\pasztorname     {Ana \pasztor}
\newcommand\paterson        {Paterson}
\newcommand\patersonname    {\michael\ S. \paterson}
\newcommand\paulson         {{\namefont Paulson}}
\newcommand\paulsonname     {{\namefont\lawrence\ C. \paulson}}
%                           {Larry C. \paulson}
% Larry will das so!
\newcommand\peano           {{\namefont Peano}}
\newcommand\peanoname       {{\namefont Guiseppe \peano}}
\newcommand\peanolifetime   {(1858--1932)}
\newcommand\peanoaxiom      {\dedekind--\peano\ axiom}
\newcommand\peckhaus        {{\namefont Peck\-haus}}
\newcommand\peckhausname    {{\namefont \volker\ \peckhaus}}
\newcommand\peirce          {{\namefont Peirce}}
\newcommand\peircename      {{\namefont \charles\ S. \peirce}}
                           %{\charles\ Sanders \peirce}
\newcommand\peircelifetime  {(1839--1914)}
\newcommand\peircefathername{\benjamin\ \peirce}
\newcommand\peircefatherlifetime{(1809--1880)}
\newcommand\peirceindex     {\index{Peirce!Charles S.}}
\newcommand\protectedpeirceindex{\protect\index{Peirce!Charles S.}}
\newcommand\peters          {Peter\es}
\newcommand\petersname      {\stanley\ \peters}
\newcommand\bachpeterssentence{\bach--\peters\ sentence}
\newcommand\bachpetersSentence{\bach--\peters\ Sentence}
\newcommand\peterson        {Peterson}
\newcommand\petersonname    {\john\ \peterson}
\newcommand\pieri           {{\namefont Pieri}}
\newcommand\pieriname       {{\namefont Mario \pieri}}
\newcommand\pierilifetime   {(1860--1913)}
\newcommand\pinkal          {Pinkal}
\newcommand\pinkalname      {\manfred\ \pinkal}
\newcommand\plaisted        {Plaisted}
\newcommand\plaistedname    {\david\ A. \plaisted}
\newcommand\planck          {Planck}
\newcommand\planckname      {\maxchristianname\ \planck}
\newcommand\plancklifetime  {(1858--1947)}
\newcommand\plato           {{\namefont Plato}}
\newcommand\platoname       {\plato} % Plato is a nickname ``the broad''.
\newcommand\platolifetime   {(427--347\,\BC)}
\newcommand\poincare        {{\namefont Poincar\'e}}
\newcommand\poincarename    {{\namefont Henri \poincare}}
\newcommand\poincarelifetime{(1854--1912)}
\newcommand\popper          {\mbox{Popper}}
\newcommand\poppername      {\karl\ \popper}%{\karl\ R. \popper} 
\newcommand\popperlifetime  {(1902--1994)}
\newcommand\pollet          {{\namefont Pollet}}
\newcommand\polletname      {{\namefont\martin\ \pollet}}
\newcommand\prause          {Prause}
\newcommand\prausename      {\gerhard\ \prause}
\newcommand\prawitz         {Pra\-witz}
\newcommand\prawitzname     {Dag \prawitz}
\newcommand\presburger      {Pre\esi burger} %actually: Prezburger
\newcommand\presburgername  {\mbox{Moj\zwithdot es{}z} \presburger}
\newcommand\presburgerlifetime{(1904--1943?)}
\newcommand\presburgerarithmetic{\presburger\ Arithmetic}
\newcommand\presburgertruename{Prez\-burger}
\newcommand\priestley       {Priestley}
\newcommand\priestleyname   {\joseph\ \priestley}
\newcommand\priestleylifetime{(1733--1804)}
\newcommand\prote           {Prote}
\newcommand\protename       {\horst\ \prote}
\newcommand\protzen         {{\namefont Protzen}}
\newcommand\protzenname     {{\namefont\martin\ \protzen}}
\newcommand\ptolemaios      {Ptole\-maio\es}
\newcommand\ptolemaiosname  {Klaudio\es\ \ptolemaios}
\newcommand\ptolemaioslifetime{(\ca\,100--\ca\,160)}
\newcommand\putnam          {Putnam}
\newcommand\putnamname      {Hilary \putnam}
\newcommand\putnamlifetime  {(born\,1926)}
\newcommand\pythagoras      {Pythagora\es}
\newcommand\pythagorasname  {\pythagoras}
%                           {\pythagoras\ of Samo\es}
% As the only other Pythagoras is also from Samos, what does ``of Samos'' help?
\newcommand\pythagoraslifetime{(\ca\,570--\ca\,500\BC)}
\newcommand\pythagorean     {{\namefont Pytha\-gorean}}
\newcommand\pythagoreans    {{\namefont\pythagorean s}}
\newcommand\quine           {{\namefont Quine}}
\newcommand\quinename       
{{\namefont Willard Van O.     \quine}}
%{{\namefont Willard Van %Orman \quine}}
\newcommand\quinelifetime   {(1908--2000)}
\newcommand\raamsdonk       {Raams\-donk}
\newcommand\raamsdonkname   {Femke van \raamsdonk}
\newcommand\readiname       {Rodrigo Readi-Nasser}
\newcommand\reddy           {Reddy}
\newcommand\reddyname       {Uday S. \reddy}
\newcommand\reichel         {Rei\-chel}
\newcommand\reichelname     {\horst\ \reichel}
\newcommand\reyle           {Reyle}
\newcommand\reylename       {\uwe\ \reyle}
\newcommand\rezaei          {{\namefont Rezaei}}
\newcommand\rezaeiname      {{\namefont Marianeh \rezaei}} 
\newcommand\ribet           {{\namefont Ribet}}
\newcommand\ribetname       {{\namefont Ken \ribet}} 
                           %{Kenneth A. \ribet}
\newcommand\riemann         {{\namefont Rie\-mann}}
\newcommand\riemannname     {{\namefont\bernhard\ \riemann}}
\newcommand\riemannlifetime {(1926--1966)}
\newcommand\ritchie         {Ritchie}
\newcommand\ritchiename     {Denni\es\ M. \ritchie}
\newcommand\robbins         {{\namefont Robbin\es}}
\newcommand\robbinsname     {{\namefont\herbert\ E. \robbins}}
\newcommand\robbinslifetime {(1922--2001)}
\newcommand\robbinsproblem  {\robbins\ Algebra problem}
\newcommand\robinson        {{\namefont Robinson}}
\newcommand\robinsonname    {{\namefont J. \alan\ \robinson}}
\newcommand\robinsonlifetime{(born\,1930)}
\newcommand\robinsontwoname {\peter\ J. \robinson}
\newcommand\roch            {{\namefont Roch}}
\newcommand\rochname        {{\namefont\gustav\ \roch}}
\newcommand\rochlifetime    {(1839--1866)}
\newcommand\roedding        {{\namefont R\oe dding}}
\newcommand\roeddingname    {{\namefont\dieter\ \roedding}}
\newcommand\rosu            {Ro\c su}
\newcommand\rosuname        {Grigore \rosu}
\newcommand\reinert         {Reinert}
\newcommand\reinertname     {Birgit \reinert}
\newcommand\roentgen        {R\oe ntgen}
\newcommand\roentgenname    {\wilhelm \ \roentgen}
\newcommand\roquette        {Roquette}
\newcommand\roquettename    {\peter\ \roquette}
\newcommand\rosser          {Rosser}
\newcommand\rossername      
{{\namefont    Barkley \rosser}}
%{{\namefont J. Barkley \rosser}}
\newcommand\rosserlifetime  {(1907-1989)}
\newcommand\rubin           {Rubin}
\newcommand\rubinhename     {Herman \rubin}
\newcommand\rubinshename    {\jean\ E. \rubin}
\newcommand\rusinowitch     {Rusino\-witch}
\newcommand\rusinowitchname {\michael\ \rusinowitch}
\newcommand\russell         {{\namefont Russell}}
\newcommand\russellname     {{\namefont Bertrand \russell}}
% {Bertrand A.\,W. \russell} % no space after A.
\newcommand\russelllifetime {(1872--1970)}
\newcommand\russellsparadox {\russell'\es\ Paradox}
\newcommand\sankappanavar   {Sankappanavar}
\newcommand\sankappanavarname{H. P. \sankappanavar}
\newcommand\sannella        {Sannella}
\newcommand\sannellaname    {\donald\ T. \sannella}
\newcommand\salzer          {{\namefont Salzer}}
\newcommand\salzername      {{\namefont Gernot \salzer}}
\newcommand\sartre          {{\namefont Sartre}}
\newcommand\sartrename      {{\namefont\jean\ \paul\ \sartre}}
\newcommand\sattler         {Sattler-Klein}
\newcommand\sattlername     {Andrea \sattler}
\newcommand\samoa           {{\namefont Schmidt-Sa\-moa}}
\newcommand\samoaname       {{\namefont\tobias\ \samoa}}
\newcommand\scanlon         {Scanlon}
\newcommand\scanlonname     {\thomas\ M. \scanlon\ \jr}
\newcommand\scanlonlifetime {(born\,1940)}
\newcommand\schiller        {Schiller}
\newcommand\schillername    {{\namefont\friedrich\ von \schiller}}
\newcommand\schillermarvinname{{\namefont Marvin \schiller}}
\newcommand\schlick         {{\namefont Schlick}}
\newcommand\schlickname     {{\namefont Moritz \schlick}}
\newcommand\schlicklifetime {(1882--1936)}
\newcommand\schmidt         {{\namefont Schmidt}}
\newcommand\fkschmidtname   {{\namefont\friedrich\ \karl\ \schmidt}}
\newcommand\arnoldschmidtname{{\namefont H. Arnold \schmidt}}
\newcommand\schmitt         {Schmitt}
\newcommand\schmittname     {\peter\ H. \schmitt}
\newcommand\schoenfinkel    {{\namefont Sch\oe n\-finkel}}
\newcommand\schoenfinkelname{{\namefont Mose\es\ \schoenfinkel}}
\newcommand\schoenfinkellifetime{(1889--1942)}
\newcommand\scholz          {{\namefont Scholz}}
\newcommand\scholzname      {{\namefont\heinrich\ \scholz}}
\newcommand\scholzlifetime  {(1884--1956)}
\newcommand\schroeder       {{\namefont Schr\oe der}}
\newcommand\schroedername   {{\namefont\ernst\ \schroeder}}
\newcommand\schroederlifetime{(1841--1902)}
\newcommand\schroedinger    {Schr\oe\-din\-ger}
\newcommand\schuermann      {{\namefont Sch\ue r\-mann}}
\newcommand\schuermannname  {{\namefont\carsten\ \schuermann}}
\newcommand\schuette        {{\namefont Sch\ue tte}}
\newcommand\schuettename    {{\namefont\kurt\ \schuette}}
\newcommand\schuettelifetime{(1909--1998)}
\newcommand\schulz          {Schulz}
\newcommand\schulzname      {\stephan\ \schulz}
\newcommand\schwaller       {{\namefont Schwaller de Lubicz}}
\newcommand\schwallername   {{\namefont \rene\ A. \schwaller}}
\newcommand\schwallerlifetime{(1887--1961)}
\newcommand\schweitzer      {{\namefont Schweitzer}}
\newcommand\schweitzername  {{\namefont\albert\ \schweitzer}}
\newcommand\schweitzerlifetime{(1875--1965)}
\newcommand\schweizer       {{\namefont Schweizer}}
\newcommand\schweizername   {{\namefont\stephan\ \schweizer}}
\newcommand\schwichtenberg  {Schwichten\-berg}
\newcommand\schwichtenbergname{\helmut\ \schwichtenberg}
\newcommand\sengler         {Sengler}
\newcommand\senglername     {\claus\ \sengler}
\newcommand\shakespeare     {Shakespeare}
\newcommand\shakespearename {\william\ \shakespeare}
\newcommand\shan            {{\namefont Shan}}
\newcommand\shanname        {{\namefont Chung-chieh \shan}}
\newcommand\sheffer         {{\namefont Sheffer}}
\newcommand\sheffername     {{\namefont Henry Maurice \sheffer}}
\newcommand\shefferstrokename{\sheffer\ stroke}
\newcommand\siefkes         {{\namefont Siefkes}}
\newcommand\siefkesname     {{\namefont\dirk\ \siefkes}}
\newcommand\sieg            {{\namefont Sieg}}
\newcommand\siegname        {{\namefont\wilfried\ \sieg}}
\newcommand\siekmann        {{\namefont Siek\-mann}}
\newcommand\siekmannname    {{\namefont \joerg\ \siekmann}}
% The true name is actually \hans-\joerg\ \siekmann.
% Thus, the often found \joerg\ H. \siekmann\ is rubbish.
\newcommand\simpson         {{\namefont Simpson}}
\newcommand\simpsonname     {{\namefont Alex \simpson}}
\newcommand\sivakumarname   {G. Sivakumar}
\newcommand\skolem          {{\namefont Skolem}}
\newcommand\skolemname      {{\namefont Thoralf \skolem}}% {Thoralf A. \skolem}
\newcommand\skolemlifetime  {(1887--1963)}
\newcommand\skolemizing     {\skolem izing}
\newcommand\skolemization   {\skolem ization}
\newcommand\skolemizedform  {\skolem ized form}   % for validity, this is
% to denote the form that results by getting all general (universal) 
% quantifiers to the top on the price of incrementing their order,
% as used in Loewenheim (1915) and Skolem (1928).
\newcommand\skolemnormalform{\skolem\ normal form}% for validity, this is 
% to denote the form that results by getting all restricted (existential)
% quantifiers to the top on the price of adding new relation symbols for the
% subformulas starting with general quantification
\newcommand\skolemsparadox  {\skolem's Paradox}
\newcommand\slind           {{\namefont Slind}}
\newcommand\slindname       {{\namefont\konrad\ \slind}}
\newcommand\smaill          {{\namefont Smaill}}
\newcommand\smaillname      {{\namefont\alan\ \smaill}}
\newcommand\smith           {Smith}
\newcommand\smithname       {\james\ T. \smith}
\newcommand\smolka          {Smolka}
\newcommand\smolkaname      {{\namefont \gerd\ \smolka}}
\newcommand\smullyan        {{\namefont Smullyan}}
\newcommand\smullyanname    {{\namefont\raymond\ M. \smullyan}}
\newcommand\snyder          {Snyder}
\newcommand\snydername      {Wayne \snyder}
\newcommand\sobocinski      {{\namefont Soboci\'nski}}
\newcommand\sobocinskiname  {{\namefont Boles\l aw \sobocinski}}
\newcommand\sobocinskilifetime{(1906--1990)}
\newcommand\sokrates        {{\namefont Sokrates}}
\newcommand\sokratesname    {{\namefont \sokrates\ the Older}}
\newcommand\sokrateslifetime{(469--399\BC)}
\newcommand\solon           {{\namefont Solon}}
\newcommand\solonname       {{\namefont \solon}}
\newcommand\solonlifetime   {(638?--after\,561\BC)}
\newcommand\sprenger        {Spren\-ger}
\newcommand\sprengername    {Christof \sprenger}
\newcommand\stanisfer       {Stanisfer}
\newcommand\stanisfername   {Ryan \stanisfer}
\newcommand\staples         {Staple\es}
\newcommand\staplesname     {\john\ \staples}
\newcommand\steele          {Steele}
\newcommand\steelename      {Guy L. \steele\ \jr}
\newcommand\steffenname     {\bernhard\ Steffen}
\newcommand\steinbach       {{\namefont Steinbach}}
\newcommand\steinbachname   {{\namefont\joachim\ \steinbach}}
\newcommand\stephansecondname{{\namefont Stephan}}
\newcommand\stephansecondnamename{{\namefont\werner\ \stephansecondname}}
\newcommand\stevens         {{\namefont Steven\es}}
\newcommand\stevensname     {{\namefont\andrew\ \stevens}}
\newcommand\stickel         {Stickel}
\newcommand\stickelname     {Mark E. \stickel}
\newcommand\stolzenburg     {Stol\-zen\-burg}
\newcommand\stolzenburgname {Frie\-der \stolzenburg}
\newcommand\stratulat       {Stratulat}
\newcommand\stratulatname   {Sorin \stratulat}
\newcommand\stuber          {Stu\-ber}
\newcommand\stubername      {\juergen\ \stuber}
\newcommand\sutcliffe       {Sutcliffe}
\newcommand\sutcliffename   {Geoff \sutcliffe}
\newcommand\suzuki          {Suzuki}
\newcommand\suzukiname      {Taro \suzuki}
\newcommand\szabo           {Szabo}
\newcommand\szaboname       {\manfred\ E. \szabo}
\newcommand\tait            {{\namefont Tait}}
\newcommand\taitname        {{\namefont William W. \tait}}
\newcommand\takagi          {Takagi}
\newcommand\takaginame      {Teiji \takagi}
\newcommand\takagilifetime  {(1875--1960)}
\newcommand\tapp            {{\namefont Tapp}}
\newcommand\tappname        {{\namefont\christian\ \tapp}}
\newcommand\tarski          {{\namefont Tar\-ski}}
\newcommand\tarskiname      {{\namefont\alfred\ \tarski}}
\newcommand\tarskilifetime  {(1901--1983)}
\newcommand\tarskigrothendieck{\tarski--Grothendieck}
\newcommand\thomasaquinas   {{\namefont\thomas}}
\newcommand\thomasaquinasname{{\namefont\thomasaquinas\ Aquina\es}}
\newcommand\thomasaquinaslifetime{(1225?--1274)}
\newcommand\thales          {{\namefont Thales}}
\newcommand\theiss          {{\namefont Theiss}}
\newcommand\theissname      {{\namefont\frank\ \theiss}}
\newcommand\thurber         {{\namefont Thurber}}
\newcommand\thurbername     {{\namefont\james\ \thurber}}
\newcommand\troelstra       {{\namefont Troelstra}}
\newcommand\troelstraname   {{\namefont Anne Sjerp \troelstra}}
%                           {{\namefont Anne S. \troelstra}}
\newcommand\toyama          {{\namefont Toyama}}
\newcommand\toyamaname      {{\namefont Yoshihito \toyama}}
\newcommand\turing          {Turing}
\newcommand\turingname      {\alan\ \turing}
\newcommand\turinglifetime  {(1912--1954)}
\newcommand\unguru          {{\namefont Unguru}}
\newcommand\unguruname      {{\namefont Sabetai \unguru}}
\newcommand\unruh           {{\namefont Unruh}}
\newcommand\unruhname       {{\namefont Fritz von \unruh}}
\newcommand\unruhlifetime   {(1885--1970)}
\newcommand\urysohn         {Urysohn}
\newcommand\urysohnname     {Pavel Samuilovich \urysohn}
\newcommand\urysohnlifetime {(1898--1924)}
\newcommand\vandeveire      {Van de Veire}
\newcommand\vandeveirename  {Ann \vandeveire}
\newcommand\veblen          {{\namefont Veblen}}
\newcommand\veblenname      {{\namefont Oswald \veblen}}
\newcommand\venn            {Venn}
\newcommand\vennname        {\john\ \venn}
\newcommand\vennlifetime    {(1834--1923)}
\newcommand\vessiot         {Vessiot}
\newcommand\vessiotname     {Ernest \vessiot}
\newcommand\vessiotlifetime {(1865--1952)}
\newcommand\viete           {{\namefont Vi\`ete}}
\newcommand\vietename       {{\namefont\francois\ \viete}}
\newcommand\vietelifetime   {(1540--1603)}
\newcommand\villon          {Villon}
\newcommand\villonname      {\francois\ \villon}
\newcommand\voigt           {{\namefont Voigt}}
\newcommand\voigtname       {{\namefont\andreas\ \heinrich\ \voigt}}
\newcommand\voigtlifetime   {(1860--1940)}
\newcommand\voronkov        {{\namefont Voron\-kov}}
\newcommand\voronkovname    {{\namefont Andrei \voronkov}}
\newcommand\wagner          {{\namefont Wag\-ner}}
\newcommand\wagnername      {{\namefont Marc \wagner}}
\newcommand\waerden         {{\namefont Waerden}}
\newcommand\waerdenname     {{\namefont Bartel Leendert van der \waerden}}
\newcommand\waerdenlifetime {(1903--1996)}
\newcommand\wajsberg        {{\namefont Waj\esi berg}}
\newcommand\wajsbergname    {{\namefont Morde\-chai \wajsberg}}
\newcommand\wajsberglifetime{(1902--1940?)}
\newcommand\waldmann        {Wald\-mann}
\newcommand\waldmanneinsname{\bernard\ \waldmann}
\newcommand\waldmannzweiname{\uwe\ \waldmann}
\newcommand\wallen          {{\namefont Wallen}}
\newcommand\wallenname      {{\namefont Lincoln A. \wallen}}
\newcommand\walsh           {{\namefont Walsh}}
\newcommand\walshname       {{\namefont Toby \walsh}}
\newcommand\walshtwoname    {C. M. \walsh}
\newcommand\walters         {Walter\es}
\newcommand\waltersname     {Humphrey \robert\ ``Pum'' \walters}
\newcommand\walther         {{\namefont Walther}}
\newcommand\walthername     {{\namefont\christoph\ \walther}} 
\newcommand\wang            {Wang} 
\newcommand\wangname        {Hao \wang} 
\newcommand\wedderburn      {Wedderburn}
\newcommand\wedderburnname  {\joseph\ H. M. \wedderburn}
                          %{\joseph\ \henry\ Maclagen \wedderburn}
\newcommand\wedderburnlifetime{(1882--1948)}
\newcommand\weber           {{\namefont Weber}}
\newcommand\webername       {{\namefont \heinrich\ \weber}}
\newcommand\weberlifetime   {(1842--1913)}
\newcommand\wegener         {Wegener} 
\newcommand\wegenername     {Ingo \wegener} 
\newcommand\wegman          {Wegman} 
\newcommand\wegmanname      {Mark N. \wegman} 
\newcommand\weidenbach      {{\namefont Weidenbach}}
\newcommand\weidenbachname  {{\namefont\christoph\ \weidenbach}}
\newcommand\weierstrass     {{\namefont Weierstra\sz}}
\newcommand\weierstrassname {{\namefont\karl\ \weierstrass}}
\newcommand\weierstrasslifetime{(1815--1897)}
\newcommand\weil            {Weil}
\newcommand\weilname        {Andr\'e \weil}
\newcommand\weillifetime    {(1906--1998)}
\newcommand\wertheimer      {Wertheimer}
\newcommand\wertheimername  {\maxchristianname\ \wertheimer}
\newcommand\wertheimerlifetime{(1880--1943)}
\newcommand\weyl            {{\namefont Weyl}}
\newcommand\weylname        {{\namefont\hermann\ \weyl}}
\newcommand\weyllifetime    {(1885--1955)}
\newcommand\whitehead       {{\namefont White\-head}}
\newcommand\whiteheadname   {{\namefont\alfred\ North \whitehead}}
\newcommand\whiteheadlifetime{(1861--1947)}
\newcommand\PM              {Principia Mathematica}
\newcommand\PMshort         {Principia}
\newcommand\principleofdependentchoice{Principle of Dependent Choice}
\newcommand\wiles           {{\namefont Wiles}}
\newcommand\wilesname       {{\namefont\andrew\ \wiles}}
\newcommand\wilhelmname     {{\namefont Rein\-hard \wilhelm}}
\newcommand\wirth           {{\namefont Wirth}}
\newcommand\wirthname       {{\namefont\claus-\peter\ \wirth}}
\newcommand\wirtz           {{\namefont Wirtz}}
\newcommand\wirtzname       {{\namefont Daniela \wirtz}}
\newcommand\wittgenstein    {{\namefont Wittgenstein}} 
\newcommand\wittgensteinname{{\namefont\ludwig\ \wittgenstein}} 
\newcommand\wittgensteinlifetime{(1889--1951)}
\newcommand\wolff           {{\namefont Wolff}} 
\newcommand\wolffname       {{\namefont\christian\ \wolff}} 
%                           {{\namefont\christian\ Freiherr von \wolff}} 
\newcommand\wolfflifetime   {(1679--1754)}
\newcommand\wolska          {Wol\-ska}
\newcommand\wolskaname      {\magdalena\ \wolska}%{\magdalena\ A. M. \wolska}
\newcommand\woods           {Wood\es}
\newcommand\woodsname       {\john\ \woods}
\newcommand\woudename       {Jaap van der Woude}
\newcommand\wrightson       {{\namefont Wright\-son}}
\newcommand\wrightsonname   {{\namefont Graham \wrightson}}
\newcommand\yamada          {Yamada}
\newcommand\yamadaname      {Toshiyuki \yamada}
\newcommand\zach            {{\namefont Zach}}
\newcommand\zachname        {{\namefont\richard\ \zach}}
\newcommand\zantema         {{\namefont Zantema}}
\newcommand\zantemaname     {{\namefont\hans\ \zantema}}
\newcommand\zaremba         {Zaremba}
\newcommand\zarembaname     {\stanislaw\ \zaremba}
\newcommand\zarembalifetime {(1863--1942)}
\newcommand\zeno            {{\namefont Zeno}} 
\newcommand\zenoeinsname    {{\namefont \zeno\ of Elea}}
                           % elatic school 
\newcommand\zenosparadox    {\zeno's Paradox}
                           % the paradox stems from \zenoeinsname 
\newcommand\zenozweiname    {{\namefont \zeno\ of Citium}}
                           % founder of stoic school
\newcommand\zenodreiname    {{\namefont \zeno\ of Sidon}}
                           % Epicurean school, induction
\newcommand\zenoeinslifetime{(\nth 5\,century\,\BC)}
\newcommand\zenozweilifetime{(\ca\,333--262\,\BC)}
\newcommand\zenodreilifetime{(\ca\,150--70\,\BC)}
\newcommand\zermelo         {{\namefont Zermelo}}
\newcommand\zermeloname     {{\namefont \ernst\ \zermelo}}
%                           {{\namefont \ernst\ F. E. \zermelo}}
\newcommand\zermelolifetime {(1871--1953)}
\newcommand\ZFlong          {\zermelo--\fraenkel}
\newcommand\ZFshort         {{\sc ZF}}
\newcommand\zhang           {{\namefont Zhang}}
\newcommand\zhangname       {{\namefont Han\-tao \zhang}}
\newcommand\zorn            {Zorn} 
\newcommand\zuse            {{\namefont Zuse}}
\newcommand\zusename        {{\namefont\konrad\ \zuse}}
%                           {{\namefont\konrad\ E. O. \zuse}}
\newcommand\zuselifetime    {(1910--1995)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ABBREVIATIONS and SPECIAL WORDS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%General:

\newcommand\am   {a.m.}
\newcommand\ASF  {ASF}
\newcommand\asfplus{\ASF\/\math{^+}}
\newcommand\afortiori{a fortiori}
\newcommand\Afortiori{A fortiori}
%\newcommand\Av   {\mbox{{A}\hspace{-.09em}{v}}}
\newcommand\appendixes{appendixes}
\newcommand\Apr  {April}
\newcommand\Aug  {Aug.}
\newcommand\ca   {ca.}
\newcommand\Ca   {Ca.}
\newcommand\ct   {c.t.}
\newcommand\fiance{fianc\'e}
\newcommand\FB   {FB}
\newcommand\FBinf{Fachbereich Informatik}
\newcommand\FBinfshort{\FB\ Informatik}
\newcommand\FR   {FR}
\newcommand\FRinf{Fachrichtung Informatik}
\newcommand\FRinfshort{\FR\ Informatik}
\newcommand\f    {\mbox{}{f.}}   %extra block blocks ligature to VI\f
\newcommand\ff   {\mbox{}{ff.}}  %extra block blocks ligature to VI\ff
\newcommand\Fa   {Fa.} % Modis
\newcommand\Feb  {Feb.}
\newcommand\FreeVariable{Free-\math\!Variable}
\newcommand\freevariable{free-variable}
\newcommand\freely{free}
\newcommand\defi {Definition} % note that this controls \litdefiref and \defiref
\newcommand\Dr   {Dr.}
\newcommand\Drrernat{Dr.\,\,rer.\,\,nat.}
\newcommand\EMAIL{E-mail}
\newcommand\eMAIL{e-mail}
\newcommand\Int  {Int.}
\newcommand\international{int.} % \int is the integral in math mode
\newcommand\Inc  {Inc.}
\newcommand\Inst {Inst.}
\newcommand\Jan  {Jan.}
\newcommand\jr   {Jr.}
\newcommand\Math {Math.}
\newcommand\mathe{math.}
\newcommand\MASlong{Mathematics Assistance System}
\newcommand\Maslong{Mathematics assistance system}
\newcommand\maslong{mathematics assistance system}
\newcommand\naiv {na\iwithtrema v}
\newcommand\naive{na\iwithtrema ve}
\newcommand\Naive{Na\iwithtrema ve}
\newcommand\Numero{No.}
\newcommand\Nov  {Nov.}
\newcommand\pmabbrev{p.m.} % \pm is already a command putting a +- in math
\newcommand\Prof {Prof.}
\newcommand\qedabbrev{q.e.d.}
\newcommand\qedhelp[1]{Q.e.d.~({#1})}
\newcommand\getittotheright[1]  
%puts argument flush right, if necessary on fol. line
{\hfill\mbox{}\penalty 100\mbox{\ \,}\nolinebreak
\hfill\hfill\hfill\nolinebreak\mbox{#1}\ignorespaces}
\newcommand\Qed      [1]{\underline{\qedhelp{#1}}}
\newcommand\Qeddouble[1]{\underline{\underline{\qedhelp{#1}}}}
\newcommand\Qedtriple[1]{\underline{\underline{\underline{\qedhelp{#1}}}}}
\newcommand\Qedbf    [1]{\mbox{\bf\qedhelp{#1}}}
\newcommand\QED      [1]{\getittotheright{\Qed      {#1}}}
\newcommand\QEDdouble[1]{\getittotheright{\Qeddouble{#1}}}
\newcommand\QEDtriple[1]{\getittotheright{\Qedtriple{#1}}}
\newcommand\QEDbf    [1]{\getittotheright{\Qedbf    {#1}}}
\newcommand\Role{R\^ole}
\newcommand\role{r\^ole}
\newcommand\Sep  {Sept.}
\newcommand\st   {s.t.}
% s.t. = sine tempore or such that
\newcommand\Tech {Tech.}
\newcommand\Tel  {Tel.}
\newcommand\theo {Theorem}
\newcommand\uni  {Uni\-ver\-si\-t\ae t}
\newcommand\Univ {Univ.}
\newcommand\Vol  {Vol.}
\newcommand\wintersemester{WS}%{Win\-ter-Semes\-ter}
\newcommand\WWW  {WWW}
\newcommand\www  {\url{http://www.ags.uni-sb.de/~cp}}
\newcommand\wwwhb{\url{http://www.dfki.de/hb}}
\newcommand\urlverbraucherpreise{\url{http://www.destatis.de/jetspeed/portal/cms/Sites/destatis/Internet/DE/Content/Statistiken/Zeitreihen/WirtschaftAktuell/Preise/Content100/kpre510bv4,templateId=renderPrint.psml}}

%Abbreviations: English or Latin:

\newcommand\AI   {Artificial Intelligence}
\newcommand\BC   {{\sc b.c.}} % Cf. Lyn Dupre, Bugs in Writing, Segment 21
\newcommand\Bull {Bull.}
\newcommand\Cf   {Cf.}
\newcommand\cf   {cf.}
\def\nlbcite{\nolinebreak\cite}
\newcommand\Cfnlb{\Cf\nolinebreak}
\newcommand\cfnlb{\cf\nolinebreak}
\newcommand\Co   {Co.}
\newcommand\Comm {Comm.}
\newcommand\Comp {Comp.}
\newcommand\Conf {Conf.}
\newcommand\contd{contd.}
\newcommand\ConstructorBased{Con\-struc\-tor-Based}
\newcommand\CS   {Computer \Sci}
\newcommand\Dec  {Dec.}
\newcommand\Dept {Dept.}
\newcommand\descenteinfinie{descente infinie}
\newcommand\Descenteinfinie{Descente infinie}
\newcommand\DescenteInfinie{Descente Infinie}
\newcommand\howdescenteinfiniegoes
{He starts with the conjecture and simplifies it by case analysis.
When he realizes that the current goal becomes 
similar to an instance of the conjecture, 
he applies the instantiated conjecture just like a lemma, 
but keeps in mind that he has actually applied an induction hypothesis. 
Finally, he searches for some \wellfounded\ ordering in which 
all the instances of the conjecture he has applied as induction hypotheses 
are smaller than the original conjecture.%
% itself.
}
\newcommand\howMethodofDescenteInfiniegoes{Show that for each 
assumed counterexample of \math\Gamma\
there is a smaller counter\-example of \math\Gamma\
\wrt\ a \wellfounded\ ordering \nlbmath<,
which does not depend on the counterexamples.}
\newcommand\theinnermostpartofW
{\math{\forall u\tight<v\stopq\app P  u}}
\newcommand\thelogicalpointofview
{At \fermat's time, natural language was still the predominant tool for 
expressing terms and equations in mathematical writing,
and it was too early for a formal axiomatization.
Moreover, note that an axiomatization captures only validity, but 
in general does neither induce a method of proof search
nor provide the data structures required to admit both
a formal treatment and a human-oriented proof search.
The formalizable logic part, however, of {\em\descenteinfinie}
can be expressed in what is called
the (\secondorder) {\em\theoremofnoetherianinduction} \nlbmath{(\ident{N})}, \ 
after \noethername\ \noetherlifetime. \ 
This is not to be confused with the {\em\axiomofstructuralinduction},
which is generically given for any inductively defined data structure, 
such as the {\em\axiomofstructuralinductionfirsthalf\ 
\nlbmath{(\ident{S})}
\axiomofstructuralinductionsecondhalf\ 
for the natural numbers inductively defined by the constructors
zero \nlbmath{\zeropp} and successor \nlbmath{\ssymbol}}. \
Moreover, we need the definition \nlbmath{(\Wellfpp{\tight<})}
of \wellfoundedness\ of a relation \nlbmath<\@.
\par\noindent\math{\begin{array}{@{}l@{\ \ \ }r@{\ }l@{}}
 (\Wellfpp{\tight<}) 
&\forall Q\stopq
&\,\inparentheses{\headroom\footroom
     \exists x\stopq\app Q x
   \nottight{\nottight{\nottight{\nottight\implies}}}
     \exists m\stopq\inparentheses{\app Q m\und
     \neg\exists w\tight<m\stopq\app Q w}}
 \footroom\\\headroom
 \inpit{\ident{N}}
&\forall P\stopq
&\inparentheses{\headroom
     \forall x\stopq\app P  x
   \nottight{\nottight{\nottight{\nottight\antiimplies}}}
     \exists\tight<\stopq\inparenthesesoplist{
      \forall v\stopq\inparentheses{
           \app P  v
         \nottight{\nottight\antiimplies}
           \theinnermostpartofW}
    \oplistund
       \Wellfpp <}}
 \footroom\\\headroom
 \inpit{\ident{S}}
&\forall P\stopq
&\,\inparentheses{\headroom\forall x\stopq\app P  x
   \nottight{\nottight{\nottight{\nottight\antiimplies}}}
   \app P \zeropp\nottight\und
   \forall y\stopq\inparentheses{\app P {\spp y}\antiimplies\app P  y}}
 \footroom\\\headroom
 (\nat 1)
&\forall\boundvari x{}\stopq
&\inparentheses{
     \boundvari x{}\tightequal\zeropp
   \nottight\oder
     \exists
     \boundvari y{}\stopq
     \boundvari x{}\tightequal\spp{\boundvari y{}}}
 \footroom\\\headroom
 (\nat 2)
 &
 \forall
 \boundvari x{}\stopq
 &
 \spp x\tightnotequal\zeropp
 \footroom\\\headroom
 (\nat 3)
 &\forall x,y\stopq
 &\inparentheses{\spp x\tightequal\spp y\nottight\implies x\tightequal y}
\\\end{array}}
\par\halftop\noindent
Let \Wellfpp\ssymbol\ denote 
\Wellfpp{\lambda x,y.\,\inpit{\spp x\tightequal y}},
which implies the \wellfoundedness\ of the ordering of the natural numbers. \ 
The natural numbers can be specified up to isomorphism
either by \math{(\ident{S})}, \nlbmath{(\nat 2)}, 
and \nlbmath{(\nat 3)}, \hskip.15em 
or else by \Wellfpp\ssymbol\ and \nlbmath{(\nat 1)}\@. \ 
The first alternative 
% is the traditional one, 
% following \dedekind\ and 
follows \dedekindname\ \dedekindlifetime\ and is 
named after \peanoname\ \peanolifetime. \ 
The second follows \pieriname\ \pierilifetime. \ 
As the instances for \math P and \nlbmath< in \nlbmath{\inpit{\ident{N}}}
are often still easy to find when the instances for \math P in 
\nlbmath{\inpit{\ident{S}}} are not, \hskip.15em 
the second alternative together with \nlbmath{\inpit{\ident{N}}}
is to be preferred in theorem proving for its usefulness and elegance. \ 
\Cfnlb\ \cite{wirthcardinal} for more on this.}
\newcommand\Diplomarbeit{Diplomarbeit (\Mastersthesis)}
\newcommand\Dissertation{Dissertation (\PhDthesis)}
\newcommand\EcoleNormaleSuperieure{\'Ecole Normale Sup\'erieure}
\newcommand\ed   {ed.}
\newcommand\Ed   {Ed.}
\newcommand\eds  {eds.}
\newcommand\eg   {e.g.}
\newcommand\Eg   {E.g.}
\newcommand\Esp  {Esp.}
\newcommand\esp  {esp.}
%\newcommand\etal{\&al.}%name already use by jsc style.
\newcommand\etalabbrev{{\namefont\&al.}}
\newcommand\etc  {\&c.}
\newcommand\exfalsoquodlibet{ex falso quodlibet}
\newcommand\extd {extd.}
\newcommand\Extd {Extd.}
\newcommand\sententialtautology{sentential tautology}
\newcommand\SententialTautology{Sentential Tautology}
\newcommand\sententialtautologies{sentential tautologies}
\newcommand\substitutionalsententialtautology
{substitutional sentential tautology}
\newcommand\substitutionalsententialtautologies
{substitutional sentential tautologies}
\newcommand\signatureenlarge     {enrich}
\newcommand\signatureenlarges    {enriches}
\newcommand\signatureenlarging   {enriching}
\newcommand\signatureenlarged    {enriched}
\newcommand\signatureenlargedby  {enriched with}
\newcommand\signatureenlargement {enrichment}
\newcommand\Signatureenlargement {Enrichment}
\newcommand\sr   {Sr.}
\newcommand\asignatureenlargement{an enrichment}
\newcommand\firstorder{first-order}
\newcommand\Firstorder{First-order}
\newcommand\FirstOrder{First-Order}
\newcommand\fol  {following}
\newcommand\ibid {ibid.} % ibidem, at the same place.
\newcommand\ie   {i.e.}
\newcommand\Ie   {I.e.}
\newcommand\incl {incl.}
\newcommand\uiff {\ iff\ }
\newcommand\udiff{\ if\ }
\newcommand\HumanOrientedInteractiveATP
{Human-Oriented Interactive Automated Theorem Proving}
\newcommand\ITP  {Inductive Theorem Proving}
\newcommand\Jun  {June}
\newcommand\Jul  {July}
% \newcommand\Log  {Log.}
\newcommand\LK   {{LK}}
\newcommand\LJ   {{LJ}}
\newcommand\Ltd  {Ltd.}
\newcommand\May  {May}
\newcommand\Mar  {March}
\newcommand\Mastersthesis{Master's thesis}
\newcommand\MSc  {M.Sc.}
\newcommand\MrUS {Mr.}
\newcommand\mutatismutandis{mutatis mutandis}
\newcommand\ND   {Natural Deduction}
% There is an alternative by \usepackage{proof} and 
% \infer*{#2}{[#1]} that does four nice dots in between.
\newcommand\nonpermutable{non-permu\-ta\-ble}
\newcommand\nonpermutability{non-permu\-ta\-bi\-lity}
\newcommand\NonPermutability{Non-Permu\-ta\-bi\-lity}
\newcommand\nonpermutabilities{non-permu\-ta\-bi\-li\-ties}
\newcommand\NonPermutabilities{Non-Permu\-ta\-bi\-li\-ties}
\newcommand\negbyfail{negation as failure}
\def\note{Note}
\newcommand\notes{Notes}
%note that \note determines \litnoteref and \noteref.
\newcommand\Oct  {Oct.}
\newcommand\p    {p.}
\newcommand\pp   {pp.}
\newcommand\PP[2]{\pp\,\ignorespaces#1--\ignorespaces#2}
% Like \pp but gets first and last page as arguments
\newcommand\PPcount[1]{#1\,\pp}
\newcommand\PhD  {PhD}%{Ph.D.}
\newcommand\PhDthesis{\PhD\ thesis}
\newcommand\PhDThesis{\PhD\ Thesis}
\newcommand\Proc {Proc.}
\newcommand\pnc  {posi\-tive/ne\-ga\-tive-condi\-tional}
\newcommand\Pnc  {Posi\-tive/ne\-ga\-tive-condi\-tional}
\newcommand\PNC  {Posi\-tive/Ne\-ga\-tive-Condi\-tional}
\newcommand\prep {prep.}
\newcommand\Publ {Publ.}
\newcommand\Quart{Quart.}
\newcommand\resp {resp.}
\newcommand\rev  {rev.}
\newcommand\Rev  {Rev.}
\newcommand\secondorder{second-order}
\newcommand\Secondorder{Second-Order}
\newcommand\sect {\myparagraphsymbol} 
%note that \sect determines \litsectref and \sectref.
\newcommand\sects{\myparagraphsymbol\myparagraphsymbol}
\newcommand\thissect{this \nolinebreak\sect}
\newcommand\Sci  {Sci.}
\newcommand\sic  {sic}
\newcommand\unary{singulary} % Following Quine's Mathematical Logic, p. 13:
% singulary, binary, ternary, quaternary, quinary
\newcommand\singulary{singulary}
\newcommand\Singulary{Singulary}
\newcommand\nullary  {nullary}
\newcommand\Soc  {Soc.}
\newcommand\substitutionlemma{{\sc Substitution \opt{Value} Lemma}}
\newcommand\explicitnesslemma{{\sc Explicitness Lemma}}
\newcommand\valuationlemma   {{\sc Valuation Lemma}}
\newcommand\foralllemma      {{\sc\math\forall-Lemma}}
\newcommand\existslemma      {{\sc\math\exists-Lemma}}
\newcommand\implieslemma     {{\sc\tightimplies-Lemma}}
\newcommand\vel  {vel}
\newcommand\vs   {vs.}
\newcommand\wellformed{well-formed}
\newcommand\wellformedness{well-formed\-ness}
\newcommand\wellfounded{well-founded}
\newcommand\WellFounded{Well-Founded}
\newcommand\nonwellfounded{non-well-founded}
\newcommand\wellfoundedness{well-founded\-ness}
\newcommand\Wellfoundedness{Well-founded\-ness}
\newcommand\wellordered{well-ordered}
\newcommand\wellorderedness{well-ordered\-ness}
\newcommand\wellordering{well-ordering}
\newcommand\Wellordering{Well-ordering}
\newcommand\WellOrdering{Well-Ordering}
\newcommand\WellOrderingTheorem{Well-Ordering Theorem}
\newcommand\wrog {w.l.o.g.} % My favorite misspelling. Moreover \wlog is
\newcommand\Wrog {W.l.o.g.} % already a latex command
\newcommand\wrt  {w.r.t.}
\newcommand\Wrt  {W.r.t.}
\newcommand\WWWhomepage{\WWW-home-page}
\newcommand\WYSIWYG{WYSIWYG}
\newcommand\zornslemma{\zorn's Lemma}

%Abbreviations: German
\newcommand\Abs{Abs.}
\newcommand\bzw{bzw\hskip-.08em.}
\newcommand\Dasheisst{D.\nolinebreak\,h.}
\newcommand\dasheisst{d.\nolinebreak\,h.}%\dh already defined
\newcommand\dasist{d.\nolinebreak\,i.}
\newcommand\Dez{Dez.}
\newcommand\exkl{exkl.}
\newcommand\ggf{ggf.}
\newcommand\geb{geb.}
\newcommand\Ing{Ing.}
\newcommand\inkl{inkl.}
\newcommand\Jh{Jh.}
\newcommand\lt{lt.}
\newcommand\Mae{M\ae rz}
\newcommand\Mai{Mai}
\newcommand\Juni{Juni}
\newcommand\MwSt{M\hskip-0.06emwSt.}
\newcommand\Nr{Nr.}
\newcommand\oa{o.\penalty100\,a.}
\newcommand\oViA{o.V.\penalty100\,i.\penalty100\,A.}
\newcommand\Okt{Okt.}
\newcommand\reell{re\unprotectedewithtrema ll}
\newcommand\so{s.o.}
\newcommand\St{St.}
\newcommand\Staatl{Staatl.}
\newcommand\Str{Str.}
\newcommand\ua{u.\penalty100\,a.} % und andere
\newcommand\usw{usw.}
\newcommand\vgl{vgl.}
\newcommand\Vgl{Vgl.}
\newcommand\vglnlb{\vgl\nolinebreak}
\newcommand\zB{z.\penalty100\,B.}
\newcommand\ZB{Z.\penalty100\,B.}
\newcommand\zT{z.\penalty100\,T.}
\newcommand\ZT{Z.\penalty100\,T.}
\newcommand\zHd{z.\penalty100\,H.}

\newcommand\pncgerman{posi\-tiv/ne\-ga\-tiv be\-dingt}
\newcommand\constructorbasedgerman{kon\-struk\-tor\-ba\-siert}
\newcommand\Inferenzsystem{In\-ferenz\-sy\esi tem}
\newcommand\Rahmeninferenzsystem{Rah\-men\-in\-ferenz\-sy\esi tem}
\newcommand\Inferenzregel{In\-ferenz\-re\-gel}
\newcommand\Termersetzungssystem{Term\-er\-setzung\esi sy\esi tem}
\newcommand\gegenueber{ge\-gen\-\ue ber}
\newcommand\Beweissteuerungskonzept{Be\-wei\esi steue\-rung\esi kon\-zept}

% references

\newcommand\Axioms{Axioms}
\newcommand\thewordand{and}
\newcommand\litspageref[1]{Page\,#1}
\newcommand\litspagerefs[2]{Pages #1 \nolinebreak \thewordand\ \nolinebreak #2}
\newcommand\litconjref[1]{Conjecture\,#1}
\newcommand\litfootref[1]{Footnote\,#1}
\newcommand\litrequref[1]{Requirement\,#1}
\newcommand\litnoteref[1]{\note\,#1}
\newcommand\litremaref[1]{Remark\,#1}
\newcommand\lititemref[1]{Item\,#1}
\newcommand\litfiguref[1]{Figure\,#1}
\newcommand\litslidref[1]{Slide\,#1}
\newcommand\litprobref[1]{Problem\,#1}
\newcommand\littheoref[1]{\theo\,#1}
\newcommand\litsectref[1]{\sect\,#1} %previously called \sectimm
\newcommand\litchapref[1]{Chapter\,#1} %{\sect\,#1}
\newcommand\litchapwithsectref[2]{Chapter\,#1, \sect\,#2}%{\sect\,#1.#2} 
\newcommand\litnotefromtoref[2]{\notes\,#1--#2}
\newcommand\litchapfromtoref[2]{Chapters\,#1--#2}
\newcommand\litsectfromtoref[2]{\sects\,#1--#2}%previously called \sectfromtoimm
\newcommand\lititemfromtoref[2]{Items #1 \nolinebreak to \nolinebreak #2}
\newcommand\litdefiref[1]{\defi\,#1}
\newcommand\Examplename{Ex\-am\-ple}
\newcommand\litexamref[1]{\Examplename\,#1}
\newcommand\litcoexref[1]{Counter\-ex\-am\-ple\,#1}
\newcommand\litlemmref[1]{Lem\-ma\,#1}
\newcommand\litaxioref[1]{Axiom\,#1}
\newcommand\litcororef[1]{Co\-rollary\,#1}
\newcommand\litpropref[1]{Pro\-po\-si\-tion\,#1}
\newcommand\litproprefs[2]
{Pro\-po\-si\-tions \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\litrequrefs
[2]{Require\-ments  \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\lititemrefs
[2]{Items           \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\litexamrefs[2]
{Examples        \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\litcoexrefs[2]
{Counterexamples \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\litlemmrefs[2]
{Lem\-mas        \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\litaxiorefs[2]
{\Axioms\        \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\litcororefs[2]
{Co\-rol\-laries \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\littheorefs[2]
{Theorems        \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\litnoterefs[2]
{\notes\         \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\litsectrefs[2]
{\sects\         \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\litchaprefs[2]
{Chapters        \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\litdefirefs[2]
{Definitions     \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\lititemrefss
[3]{Items \nolinebreak #1, #2, \thewordand\ \nolinebreak #3}
\newcommand\litdefirefss
[3]{Definitions \nolinebreak #1, #2, \thewordand\ \nolinebreak #3}
\newcommand\litexamrefss
[3]{Examples \nolinebreak #1, #2, \thewordand\ \nolinebreak #3}
\newcommand\litlemmrefss
[3]{Lemmas \nolinebreak #1, #2, \thewordand\ \nolinebreak #3}
\newcommand\litaxiorefss
[3]{\Axioms\ \nolinebreak #1, #2, \thewordand\ \nolinebreak #3}
\newcommand\litcororefss
[3]{Co\-rol\-laries \nolinebreak #1, #2, \thewordand\ \nolinebreak #3}
\newcommand\litnoterefss
[3]{\notes\ \nolinebreak #1, #2, \thewordand\ \nolinebreak #3}
\newcommand\litsectrefss
[3]{\sects\ \nolinebreak #1, #2, \thewordand\ \nolinebreak #3}
\newcommand\spageref[1]{\litspageref{\pageref{#1}}}
\newcommand\spagerefs[2]{\litspagerefs{\pageref{#1}}{\pageref{#2}}}
\newcommand\specref[1]{Spec.\,\ref{#1}}
\newcommand\requref[1]{\litrequref{\ref{#1}}}
\newcommand\conjref[1]{\litconjref{\ref{#1}}}
\newcommand\remaref[1]{\litremaref{\ref{#1}}}
\newcommand\slidref[1]{\litslidref{\ref{#1}}}
\newcommand\probref[1]{\litprobref{\ref{#1}}}
\newcommand\cororef[1]{\litcororef{\ref{#1}}}
\newcommand\lemmref[1]{\litlemmref{\ref{#1}}}
\newcommand\axioref[1]{\litaxioref{\ref{#1}}}
\newcommand\examref[1]{\litexamref{\ref{#1}}}
\newcommand\coexref[1]{\litcoexref{\ref{#1}}}
\newcommand\defiref[1]{\litdefiref{\ref{#1}}}
\newcommand\theoref[1]{\littheoref{\ref{#1}}}
\newcommand\itemref[1]{\lititemref{\ref{#1}}}
\newcommand\figuref[1]{\litfiguref{\ref{#1}}}
\newcommand\noteref[1]{\litnoteref{\ref{#1}}}
\newcommand\sectref[1]{\litsectref{\ref{#1}}}
\newcommand\nlbsectref[1]{\nolinebreak\sectref{#1}}
\newcommand\sectrefff[1]{\litsectref{\ref{#1}\,\ff\ \ignorespaces}}
\newcommand\Sectref[1]{\litsectref{\ref{#1}}}
\newcommand\itemrefs[2]{\lititemrefs{\ref{#1}}{\ref{#2}}}
\newcommand\requrefs[2]{\litrequrefs{\ref{#1}}{\ref{#2}}}
\newcommand\defirefs[2]{\litdefirefs{\ref{#1}}{\ref{#2}}}
\newcommand\lemmrefs[2]{\litlemmrefs{\ref{#1}}{\ref{#2}}}
\newcommand\axiorefs[2]{\litaxiorefs{\ref{#1}}{\ref{#2}}}
\newcommand\examrefs[2]{\litexamrefs{\ref{#1}}{\ref{#2}}}
\newcommand\coexrefs[2]{\litcoexrefs{\ref{#1}}{\ref{#2}}}
\newcommand\cororefs[2]{\litcororefs{\ref{#1}}{\ref{#2}}}
\newcommand\theorefs[2]{\littheorefs{\ref{#1}}{\ref{#2}}}
\newcommand\noterefs[2]{\litnoterefs{\ref{#1}}{\ref{#2}}}
\newcommand\sectrefs[2]{\litsectrefs{\ref{#1}}{\ref{#2}}}
\newcommand\sectfromtoref[2]{\litsectfromtoref{\ref{#1}}{\ref{#2}}}
\newcommand\notefromtoref[2]{\litnotefromtoref{\ref{#1}}{\ref{#2}}}
\newcommand\globalrequirementref[1]{\globalrequirement\,\ref{#1}}
\newcommand\itemrefss[3]{\lititemrefss{\ref{#1}}{\ref{#2}}{\ref{#3}}}
\newcommand\defirefss[3]{\litdefirefss{\ref{#1}}{\ref{#2}}{\ref{#3}}}
\newcommand\examrefss[3]{\litexamrefss{\ref{#1}}{\ref{#2}}{\ref{#3}}}
\newcommand\noterefss[3]{\litnoterefss{\ref{#1}}{\ref{#2}}{\ref{#3}}}
\newcommand\lemmrefss[3]{\litlemmrefss{\ref{#1}}{\ref{#2}}{\ref{#3}}}
\newcommand\axiorefss[3]{\litaxiorefss{\ref{#1}}{\ref{#2}}{\ref{#3}}}
\newcommand\cororefss[3]{\litcororefss{\ref{#1}}{\ref{#2}}{\ref{#3}}}
\newcommand\sectrefss[3]{\litsectrefss{\ref{#1}}{\ref{#2}}{\ref{#3}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%% here starts the \nth macro %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% It gets an integer or a character as argument and prints e.g. 
%%% \nth{1}    --->   1st
%%% \nth{11}   --->  11th
%%% \nth{21}   --->  21st
%%% \nth{-31}  ---> -31th
%%% \nth n     ---> nth
%%% \nth q     ---> qth
%%% \nth{nn}   ---> NONSENSE
%%% some more computation features provided
%%% uses count 0-5
%%% \mth      is like \nth but sets base  number in math mode
%%% \nonumbermth is like \mth, but does not work for numbers,
%%%              but for whole mathematical expressions
%%% \nonumbermst is like \nonumbermth, but puts ``st''
%%% \smallnth is like \nth but sets power text tiny
% \newcommand\nth[1]{#1\/\math{^{\hbox{\scriptsize th}}}}
% this was raising too much! And too stupid!
%\newcommand\nth[1]{\nthpositioner{#1}{\nthstring{#1}}}
%This was too big.
\newcommand\nthpositioner[2]
% do not put something around the #1! It may remove relevant font information.
{#1\raisebox{0.52ex}{\scriptsize\hspace{0.07em}#2}}
\newcommand\nth[1]{\nthtinypositioner{#1}{\nthstring{#1}}}
\newcommand\nthtinypositioner[2]{#1\raisebox{0.52ex}{\tiny\hspace{0.07em}#2}}
\newcommand\mth[1]{\mthpositioner{#1}{\nthstring{#1}}}
\newcommand\mthpositioner[2]
% do not put something around the #1! It may remove relevant font information.
{\math{#1}\raisebox{0.52ex}{\scriptsize\hspace{0.07em}#2}}
\newcommand\modulointocountzero[2]
{\count1=#1
\count2=#2
\count0=\count1
\divide  \count0 by \count2
\multiply\count0 by-\count2
\advance \count0 by \count1}
\newcommand\absolutevalueintocountzero[1]
{\count0=#1
\ifnum\count0<0\multiply\count0 by -1\fi}
\newcommand\nthstring[1]
{\def\myargone{#1}\ifcat a\myargone th\else\nthstringnochar{#1}\fi}
\newcommand\nthstringnochar[1]
{\absolutevalueintocountzero{#1}%
\modulointocountzero{\count0}{100} %we need the blank here!
\ifnum\count0>9\ifnum\count0<20 th\else\stupidnthstring\fi
                                  \else\stupidnthstring\fi}
\newcommand\stupidnthstring
{\modulointocountzero{\count0}{10}
\ifnum\count0=1 \hskip-0.2em st\else
\ifnum\count0=2 nd\else
\ifnum\count0=3 rd\else 
                th\fi\fi\fi}
\newcommand\nonumbermth[1]{\mthpositioner{#1}{th}}
\newcommand\nonumbermst[1]{\mthpositioner{#1}{st}}

\newcommand\writeascents
%writes and integer abc as a.bc
% 0   --> 0.00
% 123 --> 1.23
[1]{\count4=#1
\ifnum\count4<0 
-\multiply\count4 by -1\fi
\modulointocountzero{\count4}{10}
\divide\count4 by 10
\count3=\the\count0
\modulointocountzero{\count4}{10}
\divide\count4 by 10
\the\count4
.\the\count0
\the\count3
}

\newcommand\frenchnth[1]{\nthtinypositioner{#1}{\frenchnthstring{#1}}}
% this work correctly only for 1 and 2 by now!
\newcommand\frenchnthstring[1]
{\def\myargone{#1}\ifcat a\myargone th\else\frenchnthstringnochar{#1}\fi}
\newcommand\frenchnthstringnochar[1]
{\absolutevalueintocountzero{#1}%
\modulointocountzero{\count0}{100} %we need the blank here!
\ifnum\count0>9\ifnum\count0<20 th\else\frenchstupidnthstring\fi
                                  \else\frenchstupidnthstring\fi}
\newcommand\frenchstupidnthstring
{\modulointocountzero{\count0}{10}
\ifnum\count0=1 \hskip-0.2em re\else
\ifnum\count0=2 me\else
\ifnum\count0=3 rd\else 
                th\fi\fi\fi}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%% here ends the \nth macro %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Systems %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\COQ       {{\sc Coq}}
\newcommand\ACLTWO    {{\sc Acl2}}
\newcommand\ASCII     {{\sc Ascii}}
\newcommand\INTWOMATH {In2Math}
\newcommand\DAMIT     {DaMiT}
\newcommand\MATHWEB   {{\sc MathWeb}}
\newcommand\ACTIVEMATH{\mbox{\sc ActiveMath}}
\newcommand\AUTOMATH  {\mbox{\sc AutoMath}}
\newcommand\OANTS     {\math\Omegaoffont{\sc Ants}}
\newcommand\OPENMATH  {{\sc OpenMath}}
\newcommand\TPS       {{\sc TPS}}
\newcommand\RRL       {{\sc Rrl}}
\newcommand\SPIKE     {{\sc Spike}}
\newcommand\INKA      {{\sc Inka}}
\newcommand\NQTHM     {{\sc Nqthm}}
\newcommand\PROLOG    {{\sc Prolog}}
\newcommand\PERL      {{\sc Perl}}
\newcommand\OMEGA     {\math\Omegaoffont{\sc mega}} 
\newcommand\OYSTER    {{\sc Oyster}}
\newcommand\OYSTERCLAM{\OYSTER-\CLAM}
\newcommand\CLAM      {{\rm CL\kern-.36em\raise.39ex\hbox{\sc a}\kern-.15emM}}
\newcommand\LEOII     {\mbox{\sc Leo-II}}
\newcommand\LAMBDACLAM{{\sc \math\lambda\CLAM}}
\newcommand\LATEXML   {{\sc \LaTeX ML}}
\newcommand\ISAPLANNER{{\sc Isa\-Plan\-ner}}
\newcommand\LOUI      {{\sc L}\math\Omegaoffont{\sc UI}} 
\newcommand\CORE      {{\sc CoRe}}
\newcommand\C         {{\sc C}} 
\newcommand\COMMONLISP{{\sc Common Lisp}} 
\newcommand\JAVA      {{\sc Java}} 
\newcommand\HASKELL   {{\sc Haskell}} 
\newcommand\CURRY     {{\sc Curry}}
\newcommand\FORTRAN   {{\sc Fortran}} 
\newcommand\QUODLIBET {{\sc Quod\-Libet}} 
\newcommand\QML       {{\sc Qml}} 
\newcommand\TECTON    {{\sc Tec\-ton}} 
\newcommand\TEXMACS   {{\sc T\kern-.1667em\lower.5ex\hbox{E}\kern-.125emX\kern-.1em\lower.5ex\hbox{\textsc{m\kern-.05ema\kern-.125emc\kern-.05ems}}}}
\newcommand\XQUODLIBET{{\sc XQuod\-Libet}} 
\newcommand\EXPANDER  {{\sc Expander}} 
\newcommand\XEXPANDER {{\sc eXpander}} 
\newcommand\UNICOM    {{\sc Unicom}} 
\newcommand\KNUTHBENDIX{\knuth--\bendix}
\newcommand\PREX{\mbox{\itshape P\hspace{-2pt}.\hspace{1pt}rex\/}}
\newcommand\MBASE{{\sc MBase}}
\newcommand\ml{{\sc ml}}
\newcommand\MLshort{{\sc ML}}
\newcommand\NFshort{{\sc NF}}
\newcommand\MLlong{\quine'\es\ \nolinebreak\MLshort}
\newcommand\NFlong{\quine'\es\ \nolinebreak\NFshort}
\newcommand\ISABELLE{{\sc Isabelle}}
\newcommand\ISABELLEHOL{{\sc Isa\-belle/HOL}}
\newcommand\PVS{{\sc PVS}}
\newcommand\VAMPIRE{{\sc Vampire}}
\newcommand\VERIFUN{{\normalsize\math{\checkmark\!\!}}{\footnotesize\sc eriFun}}
\newcommand\VSE{{\sc VSE}}
\newcommand\XML{{\sc XML}}
\newcommand\WALDMEISTER{\index{Waldmeister}{\sc Wald\-Meister}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Institutions %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\DFKI{\mbox{DFKI}}
\newcommand\ags{AG Siekmann}
\newcommand\CMU{Carnegie Mellon \Univ}
\newcommand\MPII{\planckname\ \Inst\ f\ue r Informatik} 
\newcommand\MPIIenglish{\planckname\ \Inst\ for Informatics} 
\newcommand\UCBerkeley{\Univ\ of \California, \Berkeley}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Geographic Places %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\Aberdeen       {Aber\-deen}
\newcommand\Amsterdam      {Amster\-dam}
\newcommand\Augsburg       {Aug\esi burg}
\newcommand\Avignon        {Avignon}
\newcommand\California     {California}
\newcommand\Cambridge      {Cam\-bridge}
\newcommand\Chicago        {Chicago}
\newcommand\Cologne        {Cologne}
\newcommand\Berkeley       {Berkeley}
\newcommand\Berlin         {Ber\-lin}    
\newcommand\Bologna        {Bologna}
\newcommand\Boston         {Boston}
\newcommand\Breslau        {Bre\esi lau}
\newcommand\Buffalo        {Buffalo (NY)}    
\newcommand\DO             {Dort\-mund}
\newcommand\Dagstuhl       {Dag\-stuhl}
\newcommand\Darmstadt      {Darm\-stadt}
\newcommand\Diez           {Diez}
\newcommand\EB             {Edin\-burgh}
\newcommand\FFM            {Frank\-furt am Main}
\newcommand\Freiburg       {Freiburg (Breisgau)}
\newcommand\Genf           {Gen\`eve}
\newcommand\Genua          {Genova}
\newcommand\Glasgow        {Glasgow}
\newcommand\Goettingen     {G\oe ttingen}
\newcommand\Halle          {Halle an der Saale}
\newcommand\Hamburg        {Ham\-burg}
\newcommand\Harvard        {Har\-vard}
\newcommand\Hildesheim     {Hilde\esi heim}
\newcommand\Heidelberg     {Heidel\-berg}
\newcommand\Helsinki       {Helsingfor\es}
\newcommand\Innsbruck      {Inn\esi bruck}
\newcommand\Jena           {Jena}
\newcommand\KA             {Karl\esi ruhe}
\newcommand\KL             {Kaiser\esi lau\-tern}
\newcommand\KO             {Ko\-blenz}
\newcommand\Koenigsberg    {K\oe nig\esi berg}
\newcommand\Kopenhagen     {K\o ben\-havn}
\newcommand\Landau         {Lan\-dau}
\newcommand\Marburg        {Mar\-burg}
\newcommand\NewBrunswick   {New Brun\esi wick (NJ)}
\newcommand\NewYork        {New York}
\newcommand\LA             {Lo\es\ Angele\es}
\newcommand\Leipzig        {Leip\-zig}
\newcommand\London         {Lon\-don}
\newcommand\Mannheim       {Mann\-heim}
\newcommand\Massachusetts  {Massachusett\es}
\newcommand\Muenchen       {M\ue n\-chen}
\newcommand\Muenster       {M\ue nster}
\newcommand\Nancy          {Nancy}
\newcommand\Napoli         {Napoli}
\newcommand\Nuernberg      {N\ue rn\-berg}
\newcommand\Oslo           {Oslo}
\newcommand\Oxford         {Oxford}
\newcommand\Pontamousson   {Pont-\`a-Mousson (France)}
\newcommand\Princetonnostate{Princeton}
\newcommand\Princeton      {\Princetonnostate\ (NJ)}
\newcommand\Prag           {Prague}
\newcommand\Paris          {Pari\es}
\newcommand\SB             {Saar\-br\ue cken}
\newcommand\StAndrews      {St\,Andrews}
\newcommand\StPetersburg   {\St\ Peter\-burg}
\newcommand\SaratogaSprings{Sara\-toga Springs (NY)}
\newcommand\Stuttgart      {Stutt\-gart}
\newcommand\Stanford       {Stan\-ford}
\newcommand\Torino         {Torino}
\newcommand\Turkey         {Turkey}
\newcommand\Warszawa       {Warszawa}
\newcommand\WarszawaEnglish{Warsaw}
\newcommand\Washington     {Washington (DC)}
\newcommand\Wien           {Wien}
\newcommand\WI             {Wie\esi ba\-den}
\newcommand\Worms          {Worms}
\newcommand\Zuerich        {Z\ue rich}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ADDRESSES AND NAMES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\plzuniKL  {\mbox{D--67653}}
\newcommand\plzuniDO  {\mbox{D--44221}}
\newcommand\plzuniSB  {\mbox{D--66123}}
\newcommand\plzWIinnen{\mbox{D--65183}}
\newcommand\plzdiez   {\mbox{D--65582}}
\newcommand\plzdudweiler{\mbox{D--66125}}

\newcommand\uniEB       {University of \EB}
\newcommand\uniAberdeen {University of \Aberdeen}
\newcommand\uniGlasgow  {University of \Glasgow}
\newcommand\uniStAndrews{University of \StAndrews}
\newcommand\HeriotWatt{Heriot--Watt}
\newcommand\uniheriotwatt{\HeriotWatt\ University}
\newcommand\uniDO{\uni\ \DO}
\newcommand\uniKO{\uni\ \KO-\Landau}
\newcommand\uniKA{\uni\ \KA}
\newcommand\uniKL{\uni\ \KL}
\newcommand\uniSB{\uni\ des Saar\-lan\-de\es}
\newcommand\uniKLenglish{University of \KL}
\newcommand\uniSBenglish{Saar\-land University}
\newcommand\uniSBenglishshort{Saar\-land \Univ}

\newcommand\uniDOshort{\Univ\ \DO}
\newcommand\uniKLshort{\Univ\ \KL}
\newcommand\uniSBshort{Saar\-land \Univ}
\newcommand\uniEBshort{\Univ\ \EB}
\newcommand\uniKOshort{\Univ\ \KO-\Landau}
\newcommand\uniKAshort{\Univ\ \KA}

\newcommand\addressuniKL{\FBinf, \uniKL}
\newcommand\addressuniKLshort{\FBinfshort, \uniKLshort}
\newcommand\addressuniDOshort{\FBinfshort, \uniDOshort}
\newcommand\addressuniSBshort{\FRinfshort, \uniSBshort}
\newcommand\addressuniKLcomplete
{\FBinf, \uniKL, Postfach\,3049, \plzuniKL\,\KL, Germany}
\newcommand\addressuniDOcomplete
{Informatik, \uniDO, \plzuniDO\,\DO, Germany} 
\newcommand\addressuniSBcomplete
{\FRinf, \uniSB, \plzuniSB\,\SB, Germany} 
\newcommand\addressuniKLlongwithnl
{\FBinf,\\\uniKL,\\\plzuniKL\,\KL}
\newcommand\addressuniDOlongwithnl
{Informatik,\\\uniDO,\\\plzuniDO\,\DO} 
\newcommand\addressuniKLlongwithnlwithoutcomma
{\FBinf\\\uniKL\\\plzuniKL\,\KL}
\newcommand\addressuniDOlongwithnlwithoutcomma
{Informatik\\\uniDO\\\plzuniDO\,\DO} 
\newcommand\addressuniSBlongwithnlwithoutcomma
{\FRinf\\\uniSB\\\plzuniSB\,\SB} 
\def       \email        {{\tt wirth@logic.at}}
\newcommand\emailmh      {{\tt marianeh.rezaei@googlemail.com}}
% {{\tt marianeh\_80@yahoo.com}}
\newcommand\Institute
% {\planckname\ Institute for Informatics, \plzuniSB\,\SB, Germany}
{\Dept\ of \CS, \uniSBenglishshort, \plzuniSB\,\SB, Germany}
% {Brandenburger Str.\,42, \plzdiez\ \Diez, Germany}

\newcommand\SFB        {Collaborative Research Center}
\newcommand\oursfbshort{SFB\,378}
\newcommand\oursfblong {\SFB\ \oursfbshort}
\newcommand\oursfbname {Resource-Adaptive Cognitive Processes}
\newcommand\oldsfbshort{SFB\,314}
\newcommand\oldsfblong {\SFB\ \oldsfbshort}
\newcommand\oldsfbname {AI~---~Knowledge-Based Systems}

\newcommand\Myfocusofinterest{P\myfocusofinterestrest}
\newcommand\myfocusofinterest{p\myfocusofinterestrest}
\newcommand\myfocusofinterestrest
{ractice-relevant human-oriented interactive (co-) inductive 
theorem proving in first- and higher-order logics
with strong automation support,
as exemplified by our \QUODLIBET\ and \OMEGA\ systems}
\newcommand\myareasofexpertise{%
Logic%
, 
Theoretical Computer 
% \Sci%
Science%
, 
Formal Methods%
, 
\AI%
}
\newcommand\mysubfields{%
(Co-) Inductive Theorem Proving (automated/interactive)%
, 
Conditional Term Rewriting, Confluence Theorems%
, 
\hilbert's epsilon%
, 
Free-Variable Calculi%
, 
Proof Planning%
, 
\MASlong s%
,
Efficient Algorithms%
, 
Algebraic Specification%
, 
Hypertext Web Models%
,
History of Philosophy and Logic%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Citation commands %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% LECTURE NOTES

\newcommand\CSLILN[1]
{CSLI LN\,#1, CSLI Publications, \Stanford\ \Univ}

% SPRINGER LECTURE NOTES

% LNCS
\newcommand\LNCSvol[1]
{\mbox{LNCS}\,\ignorespaces#1}

% LNAI
\newcommand\LNAIvol[1]
{\mbox{LNAI}\,\ignorespaces#1}

% LNM
\newcommand\LNMvol[1]
{\mbox{LNM}\,\ignorespaces#1}


% Verlage---------------------------------------------------------------------
\newcommand\academicpress{Academic Press (\elsevier)}
\newcommand\ACM{ACM}
\newcommand\acmpress{\ACM\ Press}
\newcommand\addisonwesley{Addi\-son-Wes\-ley}
\newcommand\allenandunwin{\george\ Allen \& Unwin, \London}
\newcommand\birkhaeuser{Birkh\ae user (\springerverlag)}
\newcommand\cambridgeunipress{\Cambridge\ \Univ\ Press}
\newcommand\chicagounipress{\Univ\ \Chicago\ Press}
\newcommand\univcaliforinapress
{\Univ\ of \California\ Press, \Berkeley\ and \LA}
\newcommand\clarendonpress{Clarendon Press%, \Oxford
}
\newcommand\deGruyter{de\,Gruyter, \Berlin, \NewYork}
\newcommand\digitalpress{Digital Press (\elsevier)}
\newcommand\elsevier{Elsevier}
\newcommand\gauthiervillars{Gauthier-Villars, \Paris}
\newcommand\harvardunipress{\Harvard\ \Univ\ Press}
\newcommand\ieee{IEEE}
\newcommand\ieeepress{\ieee\ Press}
\newcommand\indianaunipress{Indiana \Univ\ Press}
\newcommand\infixverlag{Infix, 
Aka\-de\-mi\-sche Ver\-lags\-ge\-sell\-schaft Aka GmbH, 
Sankt Au\-gustin, \Berlin}
\newcommand\kluwer{Kluwer (\springerverlag)% Acad.\ \Publ
}
\newcommand\mcgrawhill{McGraw-Hill}
\newcommand\morgankaufmann{Morgan Kaufman (\elsevier)}
\newcommand\mitpress{MIT Press}
\newcommand\northholland{North-Holland (\elsevier)}
\newcommand\oxfordunipress{\Oxford\ \Univ\ Press}
\newcommand\pitman{Pitman \Publ, \London%
% This has been taken over by Financial Times Press and is hard to find.
% Thus, the place should be given explicitly!
}
\newcommand\PrenticeHall{Prentice--Hall, \Inc}
\newcommand\princetonunipress{\Princetonnostate\ \Univ\ Press}
\newcommand\DReidelpublishing{D. Reidel \Publ, Dordrecht}
\newcommand\sfischerverlagberlin{S. Fischer Ver\-lag, \Berlin}
\newcommand\sfischerverlagffm{S. Fischer Ver\-lag, \FFM}
\newcommand\springerverlag{Sprin\-ger}
\newcommand\teubner{Teub\-ner}
\newcommand\teubnerverlag{B. G. \teubner\ Ver\-lags\-ge\-sell\-schaft}
\newcommand\teubnerarchivzurmathematik[1]
{\teubner-Archiv zur Mathe\-ma\-tik, \Vol\,#1, \teubnerverlag, \Leipzig}
\newcommand\vannostrand{D. Van Nostrand}
\newcommand\wiley{\john\ Wiley \& Sons}
\newcommand\wissenschaftlichebuchgesellschaftdarmstadt
 {Wissen\-schaft\-liche Buch\-gesell\-schaft, \Darmstadt}

%Reports----------------------------------------------------------------------
\newcommand\sekireportname{SEKI-Report}
\newcommand\sekireportissn{1437--4447}
\newcommand\sekireportnoaddress[2]{\sekireportname\ \mbox{SR--#1--#2}}
\newcommand\sekireport   [2]{\sekireportnoaddress{#1}{#2}, \addressuniKLshort}
\newcommand\sekireportSB [2]{\sekireportnoaddress{#1}{#2}, \addressuniSBshort}
\newcommand\sekireportnew[2]{\sekireportnoaddress{#1}{#2}, ISSN\,1437-4447}

\newcommand\sekiworkingpapername{SEKI-Working-Paper}
\newcommand\sekiworkingpaperissn{1860--5931}
\newcommand\sekiworkingpapernoaddress[2]
{\sekiworkingpapername\ \mbox{SWP--#1--#2}}
\newcommand\sekiworkingpaper[2]{\sekiworkingpapernoaddress
{#1}{#2}, \addressuniKLshort}
\newcommand\sekiworkingpapernew[2]{\sekiworkingpapernoaddress
{#1}{#2}, ISSN\,1860-5931}

\newcommand\gruenereihe[2]{Report #2/#1, \addressuniDOshort}

\newcommand\mpireportnoaddress[2]{MPI--I--#1--2--#2}
\newcommand\mpireport[2]{\mpireportnoaddress{#1}{#2}, \MPII, \SB}

\newcommand\daireport
[1]{DAI Research Paper \Numero\,#1, \Dept\ \AI, \uniEBshort}

%Conferencen------------------------------------------------------------------
\newcommand\lncsconf[6]{\nth{#2}\,#1\,#3, #4, \PP{#5}{#6}, \springerverlag}

%AAAI
\newcommand\AAAI[4]
{\nth{#1} AAAI 19#2, \PP{#3}{#4}, \mitpress}
\newcommand\eighthAAAIninety{\AAAI{8}{90}}

%ALP1
\newcommand\fourthAlgLogPninetyfour
{\lncsconf{Algebraic and Logic Programming}{4}{1994}{\LNCSvol{850}}}

%ALP2
\newcommand\fourteenthAutLanPeightyseven
{\lncsconf{Automata, Languages and Programming}{14}{1987}{\LNCSvol{267}}}


%CAAP
\newcommand\CAAPname{\Int\ Colloquium on Trees in Algebra and Programming}
\newcommand\CAAPshort{CAAP}
\newcommand\ninthCAAPeightyfourtitle
{\Proc\ \nth 9 \CAAPname\ (\CAAPshort\,1984), Bordeaux}
%% Please use a separate bib entry!
%% \newcommand\ninthCAAPeightyfour[2]
%% {In: Bruno Courcelle (\ed): \ninthCAAPeightyfourtitle,
%%% \PP{#1}{#2}, \cambridgeunipress}
\newcommand\twentyfirstCAAPninetysix
{\lncsconf\CAAPshort{21}{1996}{\LNCSvol{1059}}}

%CADE
\newcommand\CADEname{\Int\ \Conf\ on Automated Deduction}
\newcommand\CADEshort{CADE}
\newcommand\thelocalCADE[3]{\nth{#1} \CADEname, #3, #2}
\newcommand\fifthCADEeighty           
{\lncsconf\CADEshort {5}{1980}{\LNCSvol{  87}}}
\newcommand\eighthCADEeightysix                  
{\lncsconf\CADEshort {8}{1986}{\LNCSvol{ 230}}}
\newcommand\theninthCADEeightyeight                
{\thelocalCADE       {9}{1988}{Argonne National Laboratory (IL)}}
\newcommand\ninthCADEeightyeight                
{\lncsconf\CADEshort {9}{1988}{\LNAIvol{ 310}}}
\newcommand\thetenthCADEninety                      
{\thelocalCADE      {10}{1990}{\KL}}
\newcommand\tenthCADEninety                      
{\lncsconf\CADEshort{10}{1990}{\LNAIvol{ 449}}}
\newcommand\theeleventhCADEninetytwo             
{\thelocalCADE  {11}{1992}{\SaratogaSprings}}
\newcommand\eleventhCADEninetytwo                
{\lncsconf\CADEshort{11}{1992}{\LNAIvol{ 607}}}
\newcommand\thetwelvethCADEninetyfour            
{\thelocalCADE  {12}{1994}{Nancy}}
\newcommand\twelvethCADEninetyfour               
{\lncsconf\CADEshort{12}{1994}{\LNAIvol{ 814}}}
\newcommand\thethirteenthCADEninetysix           
{\thelocalCADE  {13}{1996}{\NewBrunswick}}
\newcommand\thirteenthCADEninetysix              
{\lncsconf\CADEshort{13}{1996}{\LNAIvol{1104}}}
\newcommand\thesixteenthCADEninetynine              
{\thelocalCADE  {16}{1999}{Trento, Italy}}
\newcommand\sixteenthCADEninetynine              
{\lncsconf\CADEshort{16}{1999}{\LNAIvol{1632}}}
\newcommand\eightteenthCADEtwo                   
{\lncsconf\CADEshort{18}{2002}{\LNAIvol{2392}}}
\newcommand\theeightteenthCADEtwo                   
{\thelocalCADE  {18}{2002}{\Kopenhagen}}
\newcommand\nineteenthCADEthree                   
{\lncsconf\CADEshort{19}{2003}{\LNAIvol{2741}}}
\newcommand\thenineteenthCADEthree                   
{\thelocalCADE  {19}{2003}{Miami Beach (FL)}}
\newcommand\thetwentiethCADEfive
{\thelocalCADE  {20}{2005}{Tallinn}}
\newcommand\twentiethCADEfive
{\lncsconf\CADEshort{20}{2005}{\LNAIvol{3632}}}

%CALCULEMUS

%CCL
\newcommand\firstCCL{\nth 1 Workshop on 
Construction of Computational Logics, Val d'Ajol (France), 1992}

%CLP
\newcommand\eighthCLPtitle
{\Proc\ \nth{8} \Int\ \Conf\ on Logic Programming}
\newcommand\twelvethCLPtitle
{\Proc\ \nth{12} \Int\ \Conf\ on Logic Programming}
%% Please use a new bib entry instead!
%% \newcommand\eighthCLP  [2]{\eighthCLPtitle,   1991, \PP{#1}{#2}, \mitpress}
%% \newcommand\twelvethCLP[2]{\twelvethCLPtitle, 1995, \PP{#1}{#2}, \mitpress}

%CSL
\newcommand\CSLname{\Conf\ of the European Association for \CS\ Logic}

%CTRS
\newcommand\CTRSname{\Int\ Workshop on Conditional Term Rewriting Systems}
\newcommand\CTRSshort{CTRS}
\newcommand\theCTRS[3]{\nth{#1} \CTRSname, #3, #2}
\newcommand\firstCTRSeightyseven   {\lncsconf\CTRSshort{1}{1987}{\LNCSvol{308}}}
\newcommand\thefirstCTRSninetytwo         {\theCTRS{1}{1987}
{Orsay (France)}}
\newcommand\secondCTRSninety       {\lncsconf\CTRSshort{2}{1990}{\LNCSvol{516}}}
\newcommand\thirdCTRSninetytwo     {\lncsconf\CTRSshort{3}{1992}{\LNCSvol{656}}}
\newcommand\thethirdCTRSninetytwo         {\theCTRS{3}{1992}{\Pontamousson}}
\newcommand\fourthCTRSninetyfour   {\lncsconf\CTRSshort{4}{1994}{\LNCSvol{968}}}
\newcommand\thefourthCTRSninetyfour       {\theCTRS{4}{1994}{Jerusalem}}

%ECAI
\newcommand\ECAIname{European \Conf\ on \AI}
\newcommand\ECAI[5]
{{\em\nth{#1} \ECAIname\ (ECAI\,#2)}, \PP{#4}{#5}, #3}
\newcommand\eighthECAIeightyeight{Y. Kodratoff (\ed). \ECAI{8}{1988}{\pitman}}
\newcommand\ninthECAIninety{\ECAI{9}{1990}{\pitman}}
\newcommand\ninthECAIninetyfour{A. Cohn (\ed). \ECAI{11}{1994}{\wiley}}

%FTP
\newcommand\FTPname{\Int\ Workshop on First-Order Theorem Proving}
\newcommand\FTPshort{FTP}

%ICALP
\newcommand\thirteenthICALPeightysix{\lncsconf{ICALP}{13}{1986}{\LNCSvol{226}}}

%IJCAI
\newcommand\IJCAIname{\Int\ Joint \Conf\ on \AI}
\newcommand\IJCAI    {IJCAI}
\newcommand\eleventhIJCAIeightnine
[2]{In: N. S. Sridharan (\ed). 
       {\em \Proc\ \nth{11} \IJCAIname\ (\IJCAI)}, \PP{#1}{#2},
       \morgankaufmann}
\newcommand\thirteenthIJCAIninetythree
[2]{In: Ruzena Bajcsy (\ed). 
       {\em \Proc\ \nth{13} \IJCAIname\ (\IJCAI)}, \PP{#1}{#2},
       \morgankaufmann}
\newcommand\seventeenthIJCAIone
[2]{In: \nebelname\ (\ed). 
       {\em \Proc\ \nth{17} \IJCAIname\ (\IJCAI)}, \PP{#1}{#2},
       \morgankaufmann}

%IJCAR
\newcommand\IJCARname{\Int\ Joint \Conf\ on Automated Reasoning}
\newcommand\firstIJCARone{\lncsconf{IJCAR}{1}{2001}{\LNAIvol{2083}}}

%LFCS
\newcommand\LFCSname{\Int\ Symposium on Logical Foundations of \CS}
\newcommand\LFCSshort{LFCS}
\newcommand\thirdLFCSninetyfour
{\lncsconf\LFCSshort{3}{1994}{\LNCSvol{813}}}

%LICS
\newcommand\LICSname{\ieee\ Symposium on Logic In \CS}
\newcommand\LICS[3]
{#1 \LICSname, \PP{#2}{#3}, \ieeepress}
\newcommand\firstLICSeightysix  {\LICS{\nth 1}}
\newcommand\thirdLICSeightyeight{\LICS{\nth 3}}

%LPAR
\newcommand\LPAR{LPAR}
\newcommand\LPARname{\Int\ \Conf\ on Logic for Programming, \AI, and Reasoning}
\newcommand\thirdLPARninetytwo  {\lncsconf{LPAR} {3}{1992}{\LNAIvol {624}}}
\newcommand\fifthLPARninetyfour {\lncsconf{LPAR} {5}{1994}{\LNAIvol {822}}}
\newcommand\eleventhLPARzerofour{\lncsconf{LPAR}{11}{2004}{\LNAIvol{3452}}}
\newcommand\twelfthLPARzerofive {\lncsconf{LPAR}{12}{2005}{\LNAIvol{3835}}}

%MKM
\newcommand\MKMshort{MKM}
\newcommand\MKMname{\Int\ \Conf\ on Mathematical Knowledge Management}
\newcommand\theforthMKMfive{\nth 4 \MKMname\ (\MKMshort), Bremen, 2005}
\newcommand\fourthMKMfive{\lncsconf{MKM}{4}{2005}{\LNAIvol{3863}}}

%RTA
\newcommand\RTAname
{\Int\ \Conf\ on Rewriting Techniques and Applications}
\newcommand\theRTA[3]
{\nth{#1} \RTAname, #3, #2}
\newcommand\thirdRTAeightynine       {\lncsconf{RTA}{ 3}{1989}{\LNCSvol{ 355}}}
\newcommand\fourthRTAninetyone       {\lncsconf{RTA}{ 4}{1991}{\LNCSvol{ 488}}}
\newcommand\thesixthRTAninetyfive           {\theRTA{ 6}{1995}{\KL}}
\newcommand\sixthRTAninetyfive       {\lncsconf{RTA}{ 6}{1995}{\LNCSvol{ 914}}}
\newcommand\theseventhRTAninetysix          {\theRTA{ 7}{1996}{\NewBrunswick}}
\newcommand\seventhRTAninetysix      {\lncsconf{RTA}{ 7}{1996}{\LNCSvol{1103}}}
\newcommand\eighthRTAninetyseven     {\lncsconf{RTA}{ 8}{1997}{\LNCSvol{1232}}}
\newcommand\tenthRTAninetynine       {\lncsconf{RTA}{10}{1999}{\LNCSvol{1631}}}

%STACS
\newcommand\STACSname{\Int\ Symposium on Theoretical Aspects of \CS}
\newcommand\STACSshort{STACS}
\newcommand\eleventhSTACSninetyfour{\lncsconf{STACS}{11}{1994}{\LNCSvol{775}}}

%TABLEAUX
\newcommand\TABLEAUname
{\Int\ \Conf\ on Tableaus and Related Methods}
\newcommand\TABLEAUshort{TAB\-LEAUX}
\newcommand\theTABLEAU[3]
{\nth{#1} \TABLEAUname, #3, #2}
\newcommand\thefourthTABLEAUninetyfive{\theTABLEAU{5}{1995}{\St\ Goar (Germany)}}
\newcommand\fourthTABLEAUninetyfive
{\lncsconf\TABLEAUshort{4} {1995}{\LNAIvol{ 918}}}
\newcommand\thesixthTABLEAUninetyseven{\theTABLEAU{6}{1997}{\Pontamousson}}
\newcommand\sixthTABLEAUninetyseven
{\lncsconf\TABLEAUshort{6} {1997}{\LNAIvol{1227}}}
\newcommand\eighthTABLEAUninetynine
{\lncsconf\TABLEAUshort{8} {1999}{\LNAIvol{1617}}}
\newcommand\theeighthTABLEAUninetynine    
{\theTABLEAU{8} {1999}{\SaratogaSprings}}
\newcommand\ninthTABLEAUzero       
{\lncsconf\TABLEAUshort{9} {2000}{\LNAIvol{1847}}}
\newcommand\theeleventhTABLEAUtwo  
{\theTABLEAU{11}{2002}{\Kopenhagen}}
\newcommand\eleventhTABLEAUtwo     
{\lncsconf\TABLEAUshort{11}{2002}{\LNAIvol{2381}}}
\newcommand\thefourteenthTABLEAUfive{\theTABLEAU{14}{2005}{\KO}}
\newcommand\fourteenthTABLEAUfive
{\lncsconf\TABLEAUshort{14}{2005}{\LNAIvol{3702}}}


%TAPSOFT
\newcommand\TAPSOFTninetythree[2]
{TAPSOFT 1993, \LNCSvol{668}, \PP{#1}{#2}, \springerverlag}

%TPHOLs
\newcommand\TPHOLshort{TPHOLs}
\newcommand\TPHOLname{\Int\ \Conf\ on Theorem Proving in Higher-Order Logics}
\newcommand\theninthTPHOLninetysix{\nth 9 \TPHOLname\ (\TPHOLshort), Turku (Finland), 1996}
\newcommand\TPHOLninetysix[2]
{\theninthTPHOLninetysix, \LNCSvol{1125}, \PP{#1}{#2}, \springerverlag}


%UNIF
\newcommand\UNIFname{\Int\ Workshop on Unificiation}
\newcommand\UNIFshort{UNIF}

%Newspapers-------------------------------------------------------------------

\newcommand\newspaperreference[5]
{\def\nameofjournalpress{#2}#1, #4 #5, #3\if?\nameofjournalpress
\else, #2\fi}

\newcommand\nytimes{\newspaperreference{The \NewYork\ Times}?}

%Journals---------------------------------------------------------------------

\newcommand\dateinjournal[1]{}

\newcommand\journalreference[6]
{\def\nameofjournalpress{#2}#1\nolinebreak\hskip.2em%
\dateinjournal{(#3) }{\mbox{\bf #4}}, \PP{#5}{#6}\if?\nameofjournalpress
\else, #2\fi}

\newcommand\journalreferenceprintyear[6]
{\def\nameofjournalpress{#2}#1 
{(#3) }{\bf #4}, \PP{#5}{#6}\if?\nameofjournalpress
\else, #2\fi}

\newcommand\journalreferenceprintyearaspartofnumber[6]
{\def\nameofjournalpress{#2}#1 
{#4/#3}, \PP{#5}{#6}\if?\nameofjournalpress
\else, #2\fi}

\newcommand\AARname{Association for Automated Reasoning}
\newcommand\AARshort{AAR}

\newcommand\AbhandlungenmathHamburgname
{Abhandlungen au\es\ dem mathematischen Seminar der \Univ\ Hamburg}
\newcommand\AbhandlungenmathHamburg
{\journalreference
{\AbhandlungenmathHamburgname}?}

\newcommand\actacybernetica
{\journalreference{Acta Cybernetica}{Szeged}}

\newcommand\actamathematicaprintyear
{\journalreference{Acta Mathematica}?}

\newcommand\americanmathematicalmonthly
{\journalreference{American Mathematical Monthly}?}

\newcommand\americanjmath
{\journalreference{American J. of \Math}?}

\newcommand\americanscientistname
{American Scientist}

\newcommand\americanscientistprintyear
{\journalreferenceprintyear{\americanscientistname}?}

\newcommand\annalesecolesuperieur
{\journalreference{Annales Scientifiques d l'\EcoleNormaleSuperieure}?}

\newcommand\annalesuniversiteparis
{\journalreference{Annales de l'Universit\'e de \Paris}?}

\newcommand\annalsofmathematics
{\journalreference{Annals of Mathematics}?}

\newcommand\archivehistoryexactsciences
{\journalreference{Archive for History of Exact Sciences}\springerverlag}

\newcommand\artificialintelligence
{\journalreference{\AI}?}
\newcommand\artificialintelligenceprintyear
{\journalreferenceprintyear{\AI}?}

\newcommand\artificialintelligencetools
{\Int\ J. \AI\ Tools}

\newcommand\artificialintelligencetoolsprintyear
{\journalreferenceprintyear{\artificialintelligencetools}?}

\newcommand\AttiAccadTorinoname{Atti della Reale Accademia delle Scienze di \Torino\ ---  Classe di Scienze Morali, Storiche e Filologiche e Classe di Scienze Fisiche, Matematiche e Naturali}
\newcommand\AttiAccadTorino
{\journalreference{\AttiAccadTorinoname}?}

\newcommand\AttiAccadTorinoFisicheMatematicheNaturali
{\journalreference{Atti della Reale Accademia delle Scienze di \Torino\ ---
Classe di Scienze Fisiche, Matematiche e Naturali}?}

\newcommand\EATCSname{European Assoc.\ for Theoretical \CS}
\newcommand\EATCSshort{EATCS}
\newcommand\bulleatcs
{\journalreference{\Bull\ \EATCSshort}?}

\newcommand\AMSname{American \Math\ \Soc}
\newcommand\AMSshort{AMS}
\newcommand\bullamsname
{\Bull\ \AMSname}
\newcommand\bullams
{\journalreference{\bullamsname}?}

\newcommand\noticesamsname{Notices of the \AMSname}
\newcommand\transamsname{Transactions of the \AMSname}

\newcommand\cahierssemhistmath
{\journalreference{Cahiers du s\'eminaire d'histoire des math\'ematiques}?}

\newcommand\comptesrendusname
{Comptes rendus hebdomadaires des s\'eances de l'Acad\'emie des Sciences 
(\Paris)}

\newcommand\comptesrendus
{\journalreference{\comptesrendusname}?}

\newcommand\computationallinguisticsname{Computational Linguistic\es}
\newcommand\computationallinguistics
{\journalreference{\computationallinguisticsname}?}

\newcommand\commacm
{\journalreference{\Comm\ \ACM}\acmpress}

\newcommand\dmvmitteilungen
{\journalreferenceprintyearaspartofnumber{DMV-Mitteilungen}?}

\newcommand\ENTCSname{Electronic Notes in Theoretical \CS}
\newcommand\ENTCS
{\journalreference\ENTCSname\elsevier}

\newcommand\erkenntisannalen{Erkenntnis (Annalen der Philosophie (und Philosophischen Kritik))}

\newcommand\forschungenname
{Forschungen zur Logik und zur Grundlegung der exakten Wissenschaften}

\newcommand\forschungen
{\journalreference
{\forschungenname}
\Leipzig}

\newcommand\fundamentainformaticaename
{Fundamenta Informaticae}

\newcommand\fundamentainformaticae
{\journalreference{\fundamentainformaticaename}?}

\newcommand\ieicetrans
{\journalreference{IEICE Transactions}?}

\newcommand\informationandcomputation
{\journalreference{Information and Computation}\academicpress}

\newcommand\informationandcontrol
{\journalreference{Information and Control}?}

\newcommand\historiamathematica
{\journalreference{Historia Mathematica}?}

\newcommand\historyandphilosophyoflogicname
{History and Philosophy of Logic}
\newcommand\historyandphilosophyoflogic
{\journalreference
{\historyandphilosophyoflogicname}{Taylor \& Francis, \London}}

\newcommand\aaeccname
{J. Applicable Algebra in Engineering, Communication and Computing (AAECC)}
\newcommand\aaecc
{\journalreference\aaeccname\springerverlag}
\newcommand\aaeccprintyear
{\journalreferenceprintyear\aaeccname\springerverlag}

\newcommand\ieeetransse
{\journalreference{\ieee\ Transactions on Software Engineering}\ieeepress}

\newcommand\jacm
{\journalreference{J. \ACM}\acmpress}

\newcommand\jalname{J. Applied Logic}
\newcommand\jal
{\journalreference\jalname\elsevier}
\newcommand\jalprintyear
{\journalreferenceprintyear\jalname\elsevier}

\newcommand\jarname
{J. Automated Reasoning}
\newcommand\jar
{\journalreference\jarname\kluwer}
\newcommand\jarprintyear
{\journalreferenceprintyear\jarname\kluwer}

\newcommand\janclname{J. Applied Non-Classical Logics}
\newcommand\jancl{\journalreference\janclname?}

\newcommand\jcssname{J. Computer and System \Sci}
\newcommand\jcss
{\journalreference{\jcssname}\academicpress}

\newcommand\jlc
{\journalreference{J. Logic Computat.}\oxfordunipress}


\newcommand\jmathpuresapplname
{J.  de \Math\ Pures et Appliqu\'ees (J. \liouville)}


\newcommand\jmathpuresappl
{\journalreference{\jmathpuresapplname}?}

\newcommand\jphillogicname{J. Philosophical Logic}
\newcommand\jphillogic
{\journalreference{\jphillogicname}\kluwer}


\newcommand\jreineundangewandtemathematikname
{J.\ f\ue r die reine und angewandte Mathematik (\crelle sches J.)}

\newcommand\jreineundangewandtemathematik
{\journalreference{\jreineundangewandtemathematikname}?}


\newcommand\jscname
{J. Symbolic Computation}
\newcommand\jsc
{\journalreference{\jscname}\academicpress}
\newcommand\jscshort
{\journalreference{\jscname}?}
\newcommand\jscprintyear
%{\journalreferenceprintyear{\jscname}?}
{\journalreferenceprintyear{\jscname}\academicpress}

\newcommand\jslname{J. Symbolic Logic}
\newcommand\jsl
{\journalreference{\jslname}?}

\newcommand\leinseignementmathematiquename
{L'Enseignement Math\'e\-matique}
\newcommand\leinseignementmathematique
{\journalreference{\leinseignementmathematiquename}?}

\newcommand\linguisticinquiryname{Linguistic Inquiry}
\newcommand\linguisticinquiry
{\journalreference{\linguisticinquiryname}\mitpress}

\newcommand\linguisticsandphilosophyname{Linguistics and Philosophy}
\newcommand\linguisticsandphilosophy
{\journalreference{\linguisticsandphilosophyname}?}

\newcommand\ljigplname{Logic J. of the IGPL}
\newcommand\ljigpl
{\journalreference\ljigplname\oxfordunipress}
\newcommand\ljigplprintyear
{\journalreferenceprintyear\ljigplname\oxfordunipress}

\newcommand\mathematicallogicquarterlyname{\Math\ Logic \Quart}
\newcommand\mathematicallogicquarterly
{\journalreference{\mathematicallogicquarterlyname}?}

\newcommand\mathematischezeitschrift
{\journalreference{Mathematische Zeitschrift}?}

\newcommand\mindname{Mind}

\newcommand\mind{\journalreference{\mindname}?}

\newcommand\MathematischeAnnalen{Mathe\-ma\-ti\-sche Annalen}
\newcommand\mathematischeannalen
{\journalreference{\MathematischeAnnalen}?}

\newcommand\mitteilungenmathgeshamburgprintyear
{\journalreferenceprintyear
{Mitteilungen der Mathematischen Gesellschaft in Hamburg}?}

\newcommand\modernlogic
{\journalreference{Modern Logic}?}

\newcommand\monatsheftempname
{Monat\esi hefte f\ue r Mathematik und Physik}

\newcommand\monatsheftemp
{\journalreference{\monatsheftempname}?}

\newcommand\NordiskMatematiskTidskrift
{\journalreference{Nordisk Matematisk Tidskrift}?}

\newcommand\notredamename{Notre Dame J. of Formal Logic}
\newcommand\notredame
{\journalreference{\notredamename}?}

\newcommand\philosphiamathname{Philosophia Mathematica (III)}
\newcommand\philosphiamath
{\journalreference{\philosphiamathname}?}

\newcommand\physis
{\journalreference{Physis}?}

\newcommand\cambridgephilsoc
{\journalreference{\Proc\ \Cambridge\ Philosophical \Soc}?}

\newcommand\revuemetaphysiquemorale
{\journalreference{Revue de M\'etaphysique et de Morale}?}

\newcommand\sciencejournalname
{Science}

\newcommand\sciencejournalprintyear
{\journalreferenceprintyear{\sciencejournalname}?}

\newcommand\skriftername
{Skrifter, Norske Videnskaps-Akademi i Oslo 
(=  Videnskapsselskapet i Kristiania), 
Matema\-tisk-Natur\-viden\-skapelig Klasse}

\newcommand\skrifterpublisher
{J. Dybwad, \Oslo}

\newcommand\skrifter[4]
{\journalreference{\skriftername}
{\skrifterpublisher}{#1}{#1/#2}{#3}{#4}}

\newcommand\WarsawScientificSocietyIII
{Towarzystwa Naukowego Warszaw\-skiego, Wydzia\l\ III}

\newcommand\sprawozdaniazposiedzenname
{Sprawozdania z posiedze\'n \WarsawScientificSocietyIII\ (Comptes Rendus S\'eances Soci\'et\'e des Sciences et Lettres Varsovie, Cl.\,III)}

\newcommand\sprawozdaniazposiedzen
{\journalreference{\sprawozdaniazposiedzenname}?}

\newcommand\tcsname{Theoretical \CS}
\newcommand\tcsjournal
%{\journalreference\tcsname ?}
{\journalreference\tcsname\elsevier}
\newcommand\tcsjournalprintyear
%{\journalreference\tcsname ?}
{\journalreferenceprintyear\tcsname\elsevier}

\newcommand\themathematicsteacher
{\journalreference{The Mathematics Teacher}{ISSN\,0025-5769}}

\newcommand
\vierteljahresschriftfuerwissenschaftlichephilosophiename
{Vier\-tel\-jahr\esi schrift f\ue r wissenschaftliche Philosophie}

\newcommand\vierteljahresschriftfuerwissenschaftlichephilosophie
{\journalreference
{\vierteljahresschriftfuerwissenschaftlichephilosophiename}?}

\newcommand\ZLGname{Zeitschrift f\ue r \mathe\ Logik und Grundlagen der \Math}
\newcommand\ZLG
{\journalreference{\ZLGname}?}


==> pdf.tex <==
%&latex
\newcommand\SEKImasterusepackages{
\usepackage{times}
\input headernamesrest
\newcommand\SEKIedition{{\small Searchable Online Edition}\\}
}
\input body


==> specialfonts.tex <==
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Characters and Punctuation signs %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\underscore{\underline~}
\let\aefranz\ae
\let\oefranz\oe
%\newcommand\aefranz{\char"1A}%This does not work any more 
%\newcommand\oefranz{\char"1B}%as latex 2e confuses font tables!
\newcommand\ttbackslash  {{\tt\char'134}}
\newcommand\ttdoublequote{{\tt\char'042}}

\mathchardef\Gammaoffont="7000
\mathchardef\Gamma="0100
\mathchardef\Deltaoffont="7001
\mathchardef\Delta="0101
\mathchardef\Thetaoffont="7002
\mathchardef\Theta="0102
\mathchardef\Lambdaoffont="7003
\mathchardef\Lambda="0103
\mathchardef\Xioffont="7004
\mathchardef\Xi="0104
\mathchardef\Pioffont="7005
\mathchardef\Pi="0105
\mathchardef\Sigmaoffont="7006
\mathchardef\Sigma="0106
\mathchardef\Upsilonoffont="7007
\mathchardef\Upsilon="0107
\mathchardef\Phioffont="7008
\mathchardef\Phi="0108
\mathchardef\Psioffont="7009
\mathchardef\Psi="0109
\mathchardef\Omegaoffont="700A
\mathchardef\Omega="010A
\mathchardef\itype="017B

\catcode`\@=11

\gdef\allowhyphens{\penalty\@M \hskip\z@skip}

\gdef\set@low@box#1{\setbox\tw@\hbox{,}\setbox\z@\hbox{#1}\dimen\z@\ht\z@
     \advance\dimen\z@ -\ht\tw@
     \setbox\z@\hbox{\lower\dimen\z@ \box\z@}\ht\z@\ht\tw@ \dp\z@\dp\tw@ }
%    (this lowers the german double left quotes to the same level as the comma.)
\gdef\set@low@boxsingle#1{\setbox\tw@\hbox{\rm,}\setbox\z@\hbox{#1}\dimen\z@\ht\z@
     \advance\dimen\z@ -\ht\tw@
     \setbox\z@\hbox{\lower\dimen\z@ \box\z@}\ht\z@\ht\tw@ \dp\z@\dp\tw@ }
%    (this lowers the german single left quotes to the same level as the comma.)

\gdef\@glqq{%
\ifhmode\edef\@SF{\spacefactor\the\spacefactor}%
\else\let\@SF\empty
\fi
\CheckFamily\font\fraknomath\ifSameFamily ``\relax
\else\CheckFamily\font\swab\ifSameFamily ``\relax
\else\leavevmode\set@low@box{''}\box\z@\kern-.04em\allowhyphens\@SF\relax
\fi\fi}
\gdef\glqq{\protect\@glqq\kern+.07em}
\gdef\@grqq{%
\ifhmode\edef\@SF{\spacefactor\the\spacefactor}%
\else\let\@SF\empty 
\fi 
\CheckFamily\font\fraknomath\ifSameFamily ''\relax
\else\CheckFamily\font\swab\ifSameFamily ''\relax
\else\kern+.07em``\kern.07em\@SF\relax
\fi\fi}
\gdef\grqq{\protect\@grqq}
\gdef\@glq{{\ifhmode \edef\@SF{\spacefactor\the\spacefactor}\else
     \let\@SF\empty \fi \leavevmode
     \set@low@boxsingle{'\/}\box\z@\kern-.04em\allowhyphens\@SF\relax}}
\gdef\glq{\protect\@glq\kern+.07em}
\gdef\@grq{\ifhmode \edef\@SF{\spacefactor\the\spacefactor}\else
     \let\@SF\empty \fi \kern-.0125em`\kern.07em\@SF\relax}
\gdef\grq{\protect\@grq}

\catcode`\@=12

% Use the following two signs like ``bla bla\closequotecomma
% Do not use them like             ``bla bla\closequotecomma\
% because this produces an extra space. This cannot be
% avoided because otherwise the end-of-sentence extra-space does 
% not work prperly.
\newcommand\closequotecommanospace{''\nolinebreak\hskip-0.23em,}
\newcommand\closequotecomma      {\closequotecommanospace\         \,}
\newcommand\closequotecommaextraspace{\closequotecommanospace\   \ \,}
\newcommand\closequotefullstop   {\closequotefullstopnospace\      \,}
\newcommand\closequotefullstopextraspace   
                                 {\closequotefullstopnospace\    \ \,}
\newcommand\closequotefullstopextraextraspace   
                                 {\closequotefullstopnospace\  \ \ \,}
\newcommand\closequotefullstopcloseparentheses   
                                 {\closequotefullstopnospace)        }
\newcommand\closequotefullstopcloseparenthesesextraspace
                                 {\closequotefullstopnospace)    \ \,}
\newcommand\closequotefullstopnospace
                                 {''\nolinebreak\hskip-0.20em\@.}
\newcommand\closequotecolonnospace{''\nolinebreak\hskip-0.10em:}
\newcommand\closequotecolon      {\closequotecolonnospace\ \,}
\newcommand\closequotecolonextraspace{\closequotecolonnospace\ \ \,}
\newcommand\closequotesemicolon  {''\nolinebreak\hskip-0.06em;     \,}
\newcommand\closequotesemicolonnospace{''\nolinebreak\hskip-0.06em;}
\newcommand\closequotesemicolonextraspace  {''\nolinebreak\hskip-0.10em; \ \,}
\newcommand\closesinglequotecomma{'\nolinebreak\hskip-0.20em,      \,}
\newcommand\closesinglequotecommaextraspace{'\nolinebreak\hskip-0.20em, \ \,}
\newcommand\closesinglequotefullstopnospace{'\nolinebreak\hskip-0.20em\@.}
\newcommand\closesinglequotefullstop{\closesinglequotefullstopnospace\ \,}
\newcommand\closesinglequotefullstopextraspace
{\closesinglequotefullstopnospace\ \ \,}
\newcommand\grqqcomma             {\grqq\nolinebreak\hskip-0.25em,  \,}
\newcommand\grqqcommaextraspace   {\grqq\nolinebreak\hskip-0.25em,  \, \ }
\newcommand\grqqsemicolon         {\grqq\nolinebreak\hskip-0.15em;  \,}
\newcommand\grqcomma              {\grq\nolinebreak\hskip-0.25em,   \,}
\newcommand\grqfullstop           {\grq\nolinebreak\hskip-0.25em\@. \,}
\newcommand\grqsemicolon          {\grq\nolinebreak\hskip-0.15em; \,}
\newcommand\grqqfullstop          {\grqq\nolinebreak\hskip-0.25em\@. \,}
\newcommand\grqqfullstopextraspace{\grqq\nolinebreak\hskip-0.25em\@. \ \ \,}
\newcommand\grqqfullstopnospace   {\grqq\nolinebreak\hskip-0.25em\@.}
\newcommand\commanospace          {,\nolinebreak\hskip-0.23em}
\newcommand\fullstopnospace       {\@.\nolinebreak\hskip-0.23em}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% here starts oldgerman.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Alte deutsche Schrifttypen werden verfuegbar gemacht
% Dies sind die Schrifttypen
% (goth) gothisch
% (frak) Frankfurter Fraktur
% (swab) Schwabacher
% (init) Initialen
% font kann goth,frak,swab oder init sein.

% Jeden der Fonts gibt es in der normalen Textgroesse und den naechsten 4
% Vergroesserungen
% Aufruf mit 
% \font ... text ... 
% \Font ... text ...
% \FOnt ... text ... 
% \FONt ... text ... 
% \FONT ... text ...

% Zusaetzlich gibt es die fonts noch in Groessen fuer Indizes
% als \scriptfont \scriptscriptfont und \scriptscriptscriptfont
% Als Vergroesserungsstufen wurden mag 0.912, 0.833, 0.760 (entsprechend
% 1.2 ^ -0.5, -1, -1.5) gewaehlt.


% fuer Gebrauch im Mathemodus gibt es die Kommandos mfont, mFont, etc
% Diese erhalten ein Argument, dieses wird in einer mbox in diesem
% Font gesetzt.
% font kann goth,frak oder swab sein.
% entsprechen zu oben gibt es auch die Kommandos \mscriptscriptscriptfont,
% \mscriptscriptfont und \mscriptfont.

\makeatletter
\if \@ptsize 0
   \newfont{\scriptscriptscriptgoth}{ygoth scaled 760}
   \newfont{\scriptscriptgoth}{ygoth scaled 833}
   \newfont{\scriptgoth}{ygoth scaled 912}
   \newfont{\gothnomath}{ygoth}
   \newfont{\Goth}{ygoth scaled \magstephalf}
   \newfont{\GOth}{ygoth scaled \magstep1}
   \newfont{\GOTh}{ygoth scaled \magstep2}
   \newfont{\GOTH}{ygoth scaled \magstep3}

   \newfont{\scriptscriptscriptswab}{yswab scaled 760}
   \newfont{\scriptscriptswab}{yswab scaled 833}
   \newfont{\scriptswab}{yswab scaled 912}
   \newfont{\swab}{yswab}
   \newfont{\Swab}{yswab scaled \magstephalf}
   \newfont{\SWab}{yswab scaled \magstep1}
   \newfont{\SWAb}{yswab scaled \magstep2}
   \newfont{\SWAB}{yswab scaled \magstep3}

   \newfont{\scriptscriptscriptfrak}{yfrak scaled 760}
   \newfont{\scriptscriptfrak}{yfrak scaled 833}
   \newfont{\scriptfrak}{yfrak scaled 912}
   \newfont{\fraknomath}{yfrak}
   \newfont{\Frak}{yfrak scaled \magstephalf}
   \newfont{\FRak}{yfrak scaled \magstep1}
   \newfont{\FRAk}{yfrak scaled \magstep2}
   \newfont{\FRAK}{yfrak scaled \magstep3}

   \newfont{\init}{yinit}
   \newfont{\Init}{yinit scaled \magstephalf}
   \newfont{\INit}{yinit scaled \magstep1}
   \newfont{\INIt}{yinit scaled \magstep2}
   \newfont{\INIT}{yinit scaled \magstep3}
\fi
\if \@ptsize 1
   \newfont{\scriptscriptscriptgoth}{ygoth scaled 833}
   \newfont{\scriptscriptgoth}{ygoth scaled 912}
   \newfont{\scriptgoth}{ygoth}
   \newfont{\gothnomath}{ygoth scaled \magstephalf}
   \newfont{\Goth}{ygoth scaled \magstep1}
   \newfont{\GOth}{ygoth scaled \magstep2}
   \newfont{\GOTh}{ygoth scaled \magstep3}
   \newfont{\GOTH}{ygoth scaled \magstep4}

   \newfont{\scriptscriptscriptswab}{yswab scaled 833}
   \newfont{\scriptscriptswab}{yswab scaled 912}
   \newfont{\scriptswab}{yswab}
   \newfont{\swab}{yswab scaled \magstephalf}
   \newfont{\Swab}{yswab scaled \magstep1}
   \newfont{\SWab}{yswab scaled \magstep2}
   \newfont{\SWAb}{yswab scaled \magstep3}
   \newfont{\SWAB}{yswab scaled \magstep4}

   \newfont{\scriptscriptscriptfrak}{yfrak scaled 833}
   \newfont{\scriptscriptfrak}{yfrak scaled 912}
   \newfont{\scriptfrak}{yfrak}
   \newfont{\fraknomath}{yfrak scaled \magstephalf}
   \newfont{\Frak}{yfrak scaled \magstep1}
   \newfont{\FRak}{yfrak scaled \magstep2}
   \newfont{\FRAk}{yfrak scaled \magstep3}
   \newfont{\FRAK}{yfrak scaled \magstep4}

   \newfont{\init}{yinit scaled \magstephalf}
   \newfont{\Init}{yinit scaled \magstep1}
   \newfont{\INit}{yinit scaled \magstep2}
   \newfont{\INIt}{yinit scaled \magstep3}
   \newfont{\INIT}{yinit scaled \magstep4}
\fi
\if \@ptsize 2
   \newfont{\scriptscriptscriptgoth}{ygoth scaled 912}
   \newfont{\scriptscriptgoth}{ygoth}
   \newfont{\scriptgoth}{ygoth scaled \magstephalf}
   \newfont{\gothnomath}{ygoth scaled \magstep1}
   \newfont{\Goth}{ygoth scaled \magstep2}
   \newfont{\GOth}{ygoth scaled \magstep3}
   \newfont{\GOTh}{ygoth scaled \magstep4}
   \newfont{\GOTH}{ygoth scaled \magstep5}

   \newfont{\scriptscriptscriptswab}{yswab scaled 912}
   \newfont{\scriptscriptswab}{yswab}
   \newfont{\scriptswab}{yswab scaled \magstephalf}
   \newfont{\swab}{yswab scaled \magstep1}
   \newfont{\Swab}{yswab scaled \magstep2}
   \newfont{\SWab}{yswab scaled \magstep3}
   \newfont{\SWAb}{yswab scaled \magstep4}
   \newfont{\SWAB}{yswab scaled \magstep5}

   \newfont{\scriptscriptscriptfrak}{yfrak scaled 912}
   \newfont{\scriptscriptfrak}{yfrak}
   \newfont{\scriptfrak}{yfrak scaled \magstephalf}
   \newfont{\fraknomath}{yfrak scaled \magstep1}
   \newfont{\Frak}{yfrak scaled \magstep2}
   \newfont{\FRak}{yfrak scaled \magstep3}
   \newfont{\FRAk}{yfrak scaled \magstep4}
   \newfont{\FRAK}{yfrak scaled \magstep5}

   \newfont{\init}{yinit scaled \magstep1}
   \newfont{\Init}{yinit scaled \magstep2}
   \newfont{\INit}{yinit scaled \magstep3}
   \newfont{\INIt}{yinit scaled \magstep4}
   \newfont{\INIT}{yinit scaled \magstep5}
\fi
\newcommand{\mscriptscriptscriptgoth}[1]{\mbox{\scriptscriptscriptgoth#1}}
\newcommand{\mscriptscriptgoth}[1]{\mbox{\scriptscriptgoth#1}}
\newcommand{\mscriptgoth}[1]{\mbox{\scriptgoth#1}}
\newcommand{\mgoth}[1]{\mbox{\gothnomath#1}}
\newcommand{\mGoth}[1]{\mbox{\Goth#1}}
\newcommand{\mGOth}[1]{\mbox{\GOth#1}}
\newcommand{\mGOTh}[1]{\mbox{\GOTh#1}}
\newcommand{\mGOTH}[1]{\mbox{\GOTH#1}}

\newcommand{\mscriptscriptscriptswab}[1]{\mbox{\scriptscriptscriptswab#1}}
\newcommand{\mscriptscriptswab}[1]{\mbox{\scriptscriptswab#1}}
\newcommand{\mscriptswab}[1]{\mbox{\scriptswab#1}}
\newcommand{\mswab}[1]{\mbox{\swab#1}}
\newcommand{\mSwab}[1]{\mbox{\Swab#1}}
\newcommand{\mSWab}[1]{\mbox{\Swab#1}}
\newcommand{\mSWAb}[1]{\mbox{\Swab#1}}
\newcommand{\mSWAB}[1]{\mbox{\SWAB#1}}

\newcommand{\mscriptscriptscriptfrak}[1]{\mbox{\scriptscriptscriptfrak#1}}
\newcommand{\mscriptscriptfrak}[1]{\mbox{\scriptscriptfrak#1}}
\newcommand{\mscriptfrak}[1]{\mbox{\scriptfrak#1}}
\newcommand{\mfrak}[1]{\mbox{\fraknomath#1}}
\newcommand{\mFrak}[1]{\mbox{\Frak#1}}
\newcommand{\mFRak}[1]{\mbox{\Frak#1}}
\newcommand{\mFRAk}[1]{\mbox{\Frak#1}}
\newcommand{\mFRAK}[1]{\mbox{\FRAK#1}}
\makeatother
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% this is the end of oldgerman.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newif\ifSameFamily
\def\CheckFamily#1#2{\GetFamilyName{#1}\ArgOne
        \GetFamilyName{#2}\ArgTwo
        \ifx\ArgOne\ArgTwo\SameFamilytrue\else\SameFamilyfalse\fi}
\def\GetFamilyName#1{\edef\Tempa{#1}\def\Tempb{#1}\ifx\Tempa\Tempb
        \edef\Tempa{\fontname#1}\fi
        \edef\Tempa{\Tempa\space}%
        \expandafter\iGetFamilyName\Tempa\\}
\def\iGetFamilyName#1 #2\\#3{\def#3{#1}}
\def\DefFontName#1#2{{\escapechar-1\expandafter\expandafter\expandafter
        \iDefFontName\expandafter{\csname#2\endcsname}%
        \xdef#1{\expandafter\string\Tempa}}}
\def\iDefFontName{\def\Tempa}

%The usage is: \CheckFamily<font1><font2>\ifSameFamily ... \else ... \fi
%where <font1> and <font2> are either \font or font-id like
%\tenrm.  For example;
%
%        \CheckFamily\font\mymightyfont\ifSameFamily ... \else ... \fi
%
%will do what you want providing \mymightyfont has been
%loaded.  Otherwise, you must define font name beforehand by
%\DefFontName like;
%
%        \DefFontName\mymightyfont{mmf10}
%
%where "mmf10" is the family name of \mymightyfont.  This
%trick is required because \fontname produces a string of
%\catcode=12 (other) characters.
%
%Please note that;
%
%        \def\ifSame#1#2{\CheckFamily#1#2\ifSameFamily}
%                :
%        \ifSame\font\mymightyfont ... \else ... \fi
%
%will cause some trouble if "\ifSame ... \fi" is in the
%true/false part of another \ifXXX.  That is, when ourter
%\ifXXX causes "\ifSame" to be skipped, TeX won't think
%\ifSame is a kind of \if and will confuse \if-\fi
%construction.

\newcommand\unprotectedae
{\CheckFamily\font\fraknomath\ifSameFamily *a\else
 \CheckFamily\font\swab\ifSameFamily\char'212\else\"a\fi\fi}
\newcommand\unprotectedoe
{\CheckFamily\font\fraknomath\ifSameFamily 
*o\else\CheckFamily\font\swab\ifSameFamily\char'232\else\"o\fi\fi}
\newcommand\unprotectedue
{\CheckFamily\font\fraknomath\ifSameFamily 
*u\else\CheckFamily\font\swab\ifSameFamily\char'237\else\"u\fi\fi}
\newcommand\unprotectedAe
{\CheckFamily\font\fraknomath\ifSameFamily 
Ae\else\CheckFamily\font\swab\ifSameFamily Ae\else\"A\fi\fi}
\newcommand\unprotectedOe
{\CheckFamily\font\fraknomath\ifSameFamily 
Oe\else\CheckFamily\font\swab\ifSameFamily Oe\else\"O\fi\fi}
\newcommand\unprotectedUe
{\CheckFamily\font\fraknomath\ifSameFamily 
Ue\else\CheckFamily\font\swab\ifSameFamily Ue\else\"U\fi\fi}
\DefFontName\eccclarge{eccc1200}
\DefFontName\eccc{eccc1000}
\DefFontName\ecccsmall{eccc0900}
\DefFontName\ecccfootnotesize{eccc0800}
\newcommand\unprotectedsz
{\CheckFamily\font\fraknomath\ifSameFamily\char'032\else
 \CheckFamily\font\swab\ifSameFamily\char'032\else
 \CheckFamily\font\eccclarge\ifSameFamily sz\else
 \CheckFamily\font\eccc\ifSameFamily sz\else
 \CheckFamily\font\ecccsmall\ifSameFamily sz\else
 \CheckFamily\font\ecccfootnotesize\ifSameFamily sz\else
 \ss\fi\fi\fi\fi\fi\fi}
\newcommand\unprotectedes
{\CheckFamily\font\fraknomath\ifSameFamily\char'215\else
\CheckFamily\font\swab\ifSameFamily\char'215\else  
s\fi\fi}
% \newcommand\unprotectedses
% {\CheckFamily\font\fraknomath\ifSameFamily\char'032\else
% \CheckFamily\font\swab\ifSameFamily\char'032\else ss\fi\fi}
\newcommand\unprotectedses
{\CheckFamily\font\fraknomath\ifSameFamily 
s\nolinebreak\hskip-.055em\char'215\else
\CheckFamily\font\swab\ifSameFamily s\char'215\else ss\fi\fi}
\newcommand\unprotectedesi
{\CheckFamily\font\fraknomath\ifSameFamily\char'215\else
\CheckFamily\font\swab\ifSameFamily\char'215\else  
\mbox{s\hskip.05em}\fi\fi
\-\ignorespaces}
\newcommand\unprotectedesid
{\CheckFamily\font\fraknomath\ifSameFamily\char'215\-\hskip.055em d\else
\CheckFamily\font\swab\ifSameFamily\char'215\-d\else  
\mbox{s\hskip.055em}\-d\fi\fi
\ignorespaces}
\newcommand\unprotectedefi
{\CheckFamily\font\fraknomath\ifSameFamily f\else
\CheckFamily\font\swab\ifSameFamily f\else  
\mbox{f\hskip.055em}\fi\fi
\-\ignorespaces}
\newcommand\unprotectedsesi
{\CheckFamily\font\fraknomath\ifSameFamily 
s\nolinebreak\hskip-.055em\char'215\else
\CheckFamily\font\swab\ifSameFamily s\char'215\else\mbox{ss\hskip.045em}\fi\fi
\-\ignorespaces}
\newcommand\unprotectedmyparagraphsymbol
{\CheckFamily\font\fraknomath\ifSameFamily 
\char'244\else\CheckFamily\font\swab\ifSameFamily
\char'244\else\S\fi\fi}
\newcommand\unprotectedzwithdot
{\CheckFamily\font\fraknomath\ifSameFamily 
\accent'137z\else\CheckFamily\font\swab\ifSameFamily z\else\.z\fi\fi}
\newcommand\unprotectedewithtrema
{\-\CheckFamily\font\fraknomath\ifSameFamily 
 "e\else\CheckFamily\font\swab\ifSameFamily "e\else\"e\fi\fi}
\newcommand\unprotectediwithtrema
{\-\CheckFamily\font\fraknomath\ifSameFamily 
 "\i\else\CheckFamily\font\swab\ifSameFamily "\i\else\"\i\fi\fi}

\renewcommand\ae{\protect\unprotectedae}
\renewcommand\oe{\protect\unprotectedoe}
\newcommand\ue  {\protect\unprotectedue}
\newcommand\Ae  {\protect\unprotectedAe}
\newcommand\Oe  {\protect\unprotectedOe}
\newcommand\Ue  {\protect\unprotectedUe}
\newcommand\sz  {\protect\unprotectedsz}
\newcommand\es  {\protect\unprotectedes}
\newcommand\ses {\protect\unprotectedses}
\newcommand\esi {\protect\unprotectedesi}  %wortinterne Version
\newcommand\esid{\protect\unprotectedesid}  %wortinterne Version
\newcommand\efi {\protect\unprotectedefi}  %wortinterne Version
\newcommand\sesi{\protect\unprotectedsesi} %wortinterne Version
\newcommand\fdi {\discretionary{f-} {d}{f\mbox {\hskip.09em}d}} 
\newcommand\ffi {\discretionary{f-} {f}{f\mbox {\hskip.09em}f}} 
\newcommand\ffli{\discretionary{ff-}{l}{ff\mbox{\hskip.09em}l}} 
\newcommand\fgi {\discretionary{f-} {g}{f\mbox {\hskip.07em}g}} 
\newcommand\fki {\discretionary{f-} {k}{f\mbox {\hskip.11em}k}} 
\newcommand\fli {\discretionary{f-} {l}{f\mbox {\hskip.09em}l}} 
\newcommand\fsi {\discretionary{f-} {s}{f\mbox {\hskip.09em}s}} 
\newcommand\lli {\discretionary{l-} {l}{l\mbox {\hskip.07em}l}} 
\newcommand\tzi {\discretionary{t-} {z}{t\mbox {\hskip.03em}z}} 
\newcommand\myparagraphsymbol{\protect\unprotectedmyparagraphsymbol}
\newcommand\zwithdot{\protect\unprotectedzwithdot}
\newcommand\ewithtrema{\protect\unprotectedewithtrema}
\newcommand\iwithtrema{\protect\unprotectediwithtrema}
% \ses\ stands for ss in the form of s ending-s (\es)
% In Fraktur and Schwabacher it prints as s\es, otherwise as ss.
% Duden recommends s\es in Fraktur and Biblia Germanica does it, too.
% \sz\ may be more convenient, however. 


